Tightening Time-Energy Uncertainty Relations

The uncertainty principle is a cornerstone of modern physics, and its implications have a fundamental impact on theoretical and applied quantum mechanics. The aim of this thesis is to study and apply the uncertainty relations between time and energy, which are interpreted operationally as the speed limit of quantum evolution. A geometric approach is used to derive improved bounds for the evolution of isolated and open systems and obtain a constructive approach for efficient and fast quantum driving. These results are applied to set the limits for the rate of information transfer and processing, and the power of nanomachines.

==> Backmatter/back_inset.tex <==
\newpage\leavevmode\thispagestyle{empty}\newpage
\newpage\leavevmode\thispagestyle{empty}\newpage

==> Backmatter/back_page.tex <==
\thispagestyle{empty}
\tikz[remember picture,overlay] \node[opacity=1,inner sep=0pt] at (current page.center){\includegraphics[width=\paperwidth,height=\paperheight]{Figures/back_page.pdf}};


==> Frontmatter/first_page.tex <==
\begin{titlepage}
	\newgeometry{left=2cm,right=2cm}
	\center 
	
	%------------------------------------------------
	%	Headings
	%------------------------------------------------
	
	\includegraphics[width=0.8\textwidth]{Figures/monash_university_logo.png}\vspace{0.28\textheight}
	
	%------------------------------------------------
	%	Title
	%------------------------------------------------
	
	{\thetitle}\vspace{20pt}% Title of your document
	
	%------------------------------------------------
	%	Author(s)
	%------------------------------------------------
	
    {\Large FRANCESCO CAMPAIOLI}\\
	\vspace{5pt}
	{\large School of Physics and Astronomy\\\vspace{5pt}
	Monash University}
	
	%------------------------------------------------
	%	Date
	%------------------------------------------------
	\vspace{0.25\textheight}
	%------------------------------------------------
	%	Logo
	%------------------------------------------------
	
	{\small A thesis submitted for the degree of\\
	\textit{Doctor of Philosophy}\\
	November 2019}

	 
	%----------------------------------------------------------------------------------------
	
	\vfill % Push the date up 1/4 of the remaining page
	\restoregeometry
\end{titlepage}

==> Frontmatter/front_inset.tex <==
\newpage\leavevmode\thispagestyle{empty}\newpage

==> Frontmatter/title_page.tex <==
\thispagestyle{empty}
\tikz[remember picture,overlay] \node[opacity=1,inner sep=0pt] at (current page.center){\includegraphics[width=\paperwidth,height=\paperheight]{Figures/front_page.pdf}};


==> lib2.tex <==
@article{Campaioli2019,
       author = {{Campaioli}, Francesco and {Sloan}, William and {Modi}, Kavan and
         {Pollock}, Felix Alexander},
        title = "{An algorithm for solving unconstrained unitary quantum brachistochrone problems}",
      journal = {arXiv e-prints},
     keywords = {Quantum Physics},
         year = "2019",
        month = "Jun",
          eid = {arXiv:1906.02934},
        pages = {arXiv:1906.02934},
archivePrefix = {arXiv},
       eprint = {1906.02934},
 primaryClass = {quant-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190602934C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@phdthesis{Binder2016,
author = {Binder, Felix C},
school = {University of Oxford},
title = {{Work, Heat, and Power of Quantum Processes}},
url = {https://ora.ox.ac.uk/objects/uuid:279871ea-3b2e-4baf-975c-1bd42b4961c3},
year = {2016}
}

@article{Campaioli2018b,
abstract = {Starting from a geometric perspective, we derive a quantum speed limit for arbitrary open quantum evolution, which could be Markovian or non-Markovian, providing a fundamental bound on the time taken for the most general quantum dynamics. Our methods rely on measuring angles and distances between (mixed) states represented as generalized Bloch vectors. We study the properties of our bound and present its form for closed and open evolution, with the latter in both Lindblad form and in terms of a memory kernel. Our speed limit is provably robust under composition and mixing, features that largely improve the effectiveness of quantum speed limits for open evolution of mixed states. We also demonstrate that our bound is easier to compute and measure than other quantum speed limits for open evolution, and that it is tighter than the previous bounds for almost all open processes. Finally, we discuss the usefulness of quantum speed limits and their impact in current research, giving particular attention to quantum optimal control.},
archivePrefix = {arXiv},
arxivId = {1806.08742},
author = {Campaioli, Francesco and Pollock, Felix A. and Modi, Kavan},
eprint = {1806.08742},
file = {::},
month = {jun},
title = {{Tight, robust, and feasible quantum speed limits for open dynamics}},
url = {http://arxiv.org/abs/1806.08742},
year = {2018}
}
@article{Petz2010,
abstract = {The subject of this paper is a mathematical transition from the Fisher information of classical statistics to the matrix formalism of quantum theory. If the monotonicity is the main requirement, then there are several quantum versions parametrized by a function. In physical applications the minimal is the most popular. There is a one-to-one correspondence between Fisher informations (called also monotone metrics) and abstract covariances. The skew information and the chi-square-divergence are treated here as particular cases.},
archivePrefix = {arXiv},
arxivId = {1008.2417},
author = {Petz, Denes and Ghinea, Catalin},
eprint = {1008.2417},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Petz, Ghinea - 2010 - Introduction to quantum Fisher information.pdf:pdf},
month = {aug},
title = {{Introduction to quantum Fisher information}},
url = {http://arxiv.org/abs/1008.2417},
year = {2010}
}
@article{Michalet2005,
author = {Michalet, X. and Pinaud, F. F. and Bentolila, L. A. and Tsay, J. M. and Doose, S. and Li, J. J. and Sundaresan, G. and Wu, A. M. and Gambhir, S. S. and Weiss, S.},
journal = {Science (80-. ).},
number = {5709},
title = {{Quantum Dots for Live Cells, in Vivo Imaging, and Diagnostics}},
volume = {307},
year = {2005}
}
@article{Aerts2016,
abstract = {An extended Bloch representation of quantum mechanics was recently derived to offer a possible (hidden-measurements) solution to the measurement problem. In this article we use this representation to investigate the geometry of superposition and entangled states, explaining interference effects and entanglement correlations in terms of the different orientations a state-vector can take within the generalized Bloch sphere. We also introduce a tensorial determination of the generators of SU(N), which we show to be particularly suitable for the description of multipartite systems, from the viewpoint of the sub-entities. We then use it to show that non-product states admit a general description where sub-entities can remain in well-defined states, even when entangled. This means that the completed version of quantum mechanics provided by the extended Bloch representation, where density operators are also considered to be representative of genuine states (providing a complete description), not only offers a pl...},
author = {Aerts, Diederik and {Sassoli de Bianchi}, Massimiliano},
doi = {10.1063/1.4973356},
issn = {0022-2488},
journal = {J. Math. Phys.},
keywords = {SU(N) theory,quantum entanglement},
month = {dec},
number = {12},
pages = {122110},
publisher = { AIP Publishing LLC  },
title = {{The extended Bloch representation of quantum mechanics: Explaining superposition, interference, and entanglement}},
url = {http://aip.scitation.org/doi/10.1063/1.4973356},
volume = {57},
year = {2016}
}
@article{Zheng2016,
author = {Zheng, Yuanjian and Campbell, Steve and {De Chiara}, Gabriele and Poletti, Dario},
doi = {10.1103/PhysRevA.94.042132},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zheng et al. - 2016 - Cost of counterdiabatic driving and work output.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {oct},
number = {4},
pages = {042132},
publisher = {American Physical Society},
title = {{Cost of counterdiabatic driving and work output}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.94.042132},
volume = {94},
year = {2016}
}
@book{InstitutionofEngineeringandTechnology.2007,
abstract = {This study presents a survey on quantum control theory and applications from a control systems perspective. Some of the basic concepts and main developments (including open-loop control and closed-loop control) in quantum control theory are reviewed. In the area of open-loop quantum control, the paper surveys the notion of controllability for quantum systems and presents several control design strategies including optimal control, Lyapunov-based methodologies, variable structure control and quantum incoherent control. In the area of closed-loop quantum control, this study reviews closed-loop learning control and several important issues related to quantum feedback control including quantum filtering, feedback stabilisation, linear-quadratic-Gaussian control and robust quantum control.},
author = {{Institution of Engineering and Technology.}, D. and Petersen, I.R.},
booktitle = {IET Control Theory {\&} Appl.},
issn = {1751-8652},
keywords = {Lyapunov based methodologies,closed-loop control,control design,control systems,controllability,feedback stabilisation,linear-quadratic-Gaussian control,open-loop control,optimal control,quantum control theory,quantum feedback control,quantum filtering,quantum incoherent control,robust quantum control,variable structure control},
month = {dec},
number = {12},
pages = {2651--2671},
publisher = {Institution of Engineering and Technology},
title = {{IET control theory {\&} applications}},
url = {http://digital-library.theiet.org/content/journals/10.1049/iet-cta.2009.0508},
volume = {4},
year = {2007}
}
@article{Zander2007,
author = {Zander, C and Plastino, a R and Plastino, A and Casas, M},
doi = {10.1088/1751-8113/40/11/020},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zander et al. - 2007 - Entanglement and the speed of evolution of multi-partite quantum systems.pdf:pdf},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {mar},
number = {11},
pages = {2861--2872},
publisher = {IOP Publishing},
title = {{Entanglement and the speed of evolution of multi-partite quantum systems}},
url = {http://stacks.iop.org/1751-8121/40/i=11/a=020?key=crossref.a7e222c8936a9c8eab84a36b94f41c47},
volume = {40},
year = {2007}
}
@article{Reich2012,
abstract = {The non-linear optimization method developed by A. Konnov and V. Krotov [Autom. Remote Cont. (Engl. Transl.) 60, 1427 (1999)] has been used previously to extend the capabilities of optimal control theory from the linear to the non-linear Schr{\"{o}}dinger equation [S. E. Sklarz and D. J. Tannor, Phys. Rev. A 66, 053619 (2002)]10.1103/PhysRevA.66.053619. Here we show that based on the Konnov-Krotov method, monotonically convergent algorithms are obtained for a large class of quantum control problems. It includes, in addition to nonlinear equations of motion, control problems that are characterized by non-unitary time evolution, nonlinear dependencies of the Hamiltonian on the control, time-dependent targets, and optimization functionals that depend to higher than second order on the time-evolving states. We furthermore show that the nonlinear (second order) contribution can be estimated either analytically or numerically, yielding readily applicable optimization algorithms. We demonstrate monotonic convergence f...},
author = {Reich, Daniel M. and Ndong, Mamadou and Koch, Christiane P.},
doi = {10.1063/1.3691827},
issn = {0021-9606},
journal = {J. Chem. Phys.},
keywords = {Schrodinger equation,convergence of numerical methods,optical control,optimisation,polynomials,quantum optics},
month = {mar},
number = {10},
pages = {104103},
publisher = {American Institute of Physics},
title = {{Monotonically convergent optimization in quantum control using Krotov's method}},
url = {http://aip.scitation.org/doi/10.1063/1.3691827},
volume = {136},
year = {2012}
}
@article{Mirkin2016,
author = {Mirkin, Nicol{\'{a}}s and Toscano, Fabricio and Wisniacki, Diego A.},
doi = {10.1103/PhysRevA.94.052125},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Mirkin, Toscano, Wisniacki - 2016 - Quantum-speed-limit bounds in an open quantum evolution.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {nov},
number = {5},
pages = {052125},
publisher = {American Physical Society},
title = {{Quantum-speed-limit bounds in an open quantum evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.94.052125},
volume = {94},
year = {2016}
}
@article{Levitin2009,
abstract = {How fast a quantum state can evolve has attracted considerable attention in connection with quantum measurement and information processing. A lower bound on the orthogonalization time, based on the energy spread $\Delta$E, was found by Mandelstam and Tamm. Another bound, based on the average energy E, was established by Margolus and Levitin. The bounds coincide and can be attained by certain initial states if $\Delta$E=E. Yet, the problem remained open when $\Delta$E≠E. We consider the unified bound that involves both $\Delta$E and E. We prove that there exist no initial states that saturate the bound if $\Delta$E≠E. However, the bound remains tight: for any values of $\Delta$E and E, there exists a one-parameter family of initial states that can approach the bound arbitrarily close when the parameter approaches its limit. These results establish the fundamental limit of the operation rate of any information processing system.},
author = {Levitin, Lev B. and Toffoli, Tommaso},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Levitin, Toffoli - Unknown - Fundamental Limit on the Rate of Quantum Dynamics The Unified Bound Is Tight.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Levitin, Toffoli - 2009 - Fundamental Limit on the Rate of Quantum Dynamics The Unified Bound Is Tight.pdf:pdf},
isbn = {0031-9007},
issn = {00319007},
journal = {Phys. Rev. Lett.},
keywords = {Levitin2009},
month = {oct},
number = {16},
pages = {160502},
pmid = {19905679},
publisher = {American Physical Society},
title = {{Fundamental limit on the rate of quantum dynamics: The unified bound is tight}},
url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.103.160502},
volume = {103},
year = {2009}
}
@article{Berrada2018,
abstract = {In this paper, the behavior of the quantum speed up with detuning for an open two-level system embedded in a reservoir at zero temperature within the Janes-Cummings model is studied. We consider two examples of spectral densities in the framework of non-Markovian environments: a high-Q cavity is slightly off-resonant with the transition frequency of the qubit and a two-level system coupled to an anisotropic photonic band gap crystal environment without Markovian or Born approximation. Generally, it is found that there exist a sudden transition from no speedup to speedup at certain critical detuning value, and the physical parameters do not affect the decoherence process for long driving times. Interestingly, we find that the control of the speed of the quantum evolution can be benefit from the combination of the detuning and spectral width density in the first case, while the acceleration of the quantum evolution occurs as the qubit transition frequency is detuned inside the gap for the anisotropic dispersion model. Finally, we clarify how the excited populations and non-Markovianity can be influenced by the detuning to realize the quantum speed limit.},
author = {Berrada, K.},
doi = {10.1016/J.PHYSE.2017.08.020},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Berrada - 2018 - Quantum speedup in structured environments.pdf:pdf},
issn = {1386-9477},
journal = {Phys. E Low-dimensional Syst. Nanostructures},
month = {jan},
pages = {6--10},
publisher = {North-Holland},
title = {{Quantum speedup in structured environments}},
url = {https://www.sciencedirect.com/science/article/pii/S1386947717308846},
volume = {95},
year = {2018}
}
@article{Gessner2018,
author = {Gessner, Manuel and Smerzi, Augusto},
doi = {10.1103/PhysRevA.97.022109},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {feb},
number = {2},
pages = {022109},
publisher = {American Physical Society},
title = {{Statistical speed of quantum states: Generalized quantum Fisher information and Schatten speed}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.97.022109},
volume = {97},
year = {2018}
}
@article{Horikawa2013,
abstract = {Visual imagery during sleep has long been a topic of persistent speculation, but its private nature has hampered objective analysis. Here we present a neural decoding approach in which machine-learning models predict the contents of visual imagery during the sleep-onset period, given measured brain activity, by discovering links between human functional magnetic resonance imaging patterns and verbal reports with the assistance of lexical and image databases. Decoding models trained on stimulus-induced brain activity in visual cortical areas showed accurate classification, detection, and identification of contents. Our findings demonstrate that specific visual experience during sleep is represented by brain activity patterns shared by stimulus perception, providing a means to uncover subjective contents of dreaming using objective neural measurement.},
author = {Horikawa, T and Tamaki, M and Miyawaki, Y and Kamitani, Y},
doi = {10.1126/science.1234330},
issn = {1095-9203},
journal = {Science},
month = {may},
number = {6132},
pages = {639--42},
pmid = {23558170},
publisher = {American Association for the Advancement of Science},
title = {{Neural decoding of visual imagery during sleep.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/23558170},
volume = {340},
year = {2013}
}
@article{Luo2005,
author = {Luo, Shunlong and Zhang, Zhengmin},
doi = {10.1007/s11005-004-5095-4},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Luo, Zhang - 2005 - On Decaying Rate of Quantum States.pdf:pdf},
issn = {0377-9017},
journal = {Lett. Math. Phys.},
month = {jan},
number = {1},
pages = {1--11},
publisher = {Kluwer Academic Publishers},
title = {{On Decaying Rate of Quantum States}},
url = {http://link.springer.com/10.1007/s11005-004-5095-4},
volume = {71},
year = {2005}
}
@article{Lopez2008,
author = {L{\'{o}}pez, C. E. and Romero, G. and Lastra, F. and Solano, E. and Retamal, J. C.},
doi = {10.1103/PhysRevLett.101.080503},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {aug},
number = {8},
pages = {080503},
publisher = {American Physical Society},
title = {{Sudden Birth versus Sudden Death of Entanglement in Multipartite Systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.080503},
volume = {101},
year = {2008}
}
@article{Pollock2017,
abstract = {Memory effects in open quantum dynamics are often incorporated in the equation of motion through a superoperator known as the memory kernel, which encodes how past states affect future dynamics. However, the usual prescription for determining the memory kernel requires information about the underlying system-environment dynamics. Here, by deriving the transfer tensor method from first principles, we show how a memory kernel master equation, for any quantum process, can be entirely expressed in terms of a family of completely positive dynamical maps. These can be reconstructed through quantum process tomography on the system alone, either experimentally or numerically, and the resulting equation of motion is equivalent to a generalised Nakajima-Zwanzig equation. For experimental settings, we give a full prescription for the reconstruction procedure, rendering the memory kernel operational. When simulation of an open system is the goal, we show how our procedure yields a considerable advantage for numerically calculating dynamics, even when the system is arbitrarily periodically (or transiently) driven or initially correlated with its environment. Namely, we show that the long time dynamics can be efficiently obtained from a set of reconstructed maps over a much shorter time.},
author = {Pollock, Felix A. and Modi, Kavan},
doi = {10.22331/q-2018-07-11-76},
issn = {2521-327X},
journal = {Quantum},
month = {apr},
pages = {76},
publisher = {Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften},
title = {{Tomographically reconstructed master equations for any open quantum dynamics}},
url = {https://quantum-journal.org/papers/q-2018-07-11-76/ http://dx.doi.org/10.22331/q-2018-07-11-76},
volume = {2},
year = {2017}
}
@article{Deffner2010,
author = {Deffner, Sebastian and Lutz, Eric},
doi = {10.1103/PhysRevLett.105.170402},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Deffner, Lutz - 2010 - Generalized Clausius Inequality for Nonequilibrium Quantum Processes.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {oct},
number = {17},
pages = {170402},
publisher = {American Physical Society},
title = {{Generalized Clausius Inequality for Nonequilibrium Quantum Processes}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.170402},
volume = {105},
year = {2010}
}
@article{Batle2005,
author = {Batle, J. and Casas, M. and Plastino, A. and Plastino, A. R.},
doi = {10.1103/PhysRevA.72.032337},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Batle et al. - 2005 - Connection between entanglement and the speed of quantum evolution.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {032337},
publisher = {American Physical Society},
title = {{Connection between entanglement and the speed of quantum evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.72.032337},
volume = {72},
year = {2005}
}
@book{Nielsen2000,
abstract = {This is an introduction to the main ideas and techniques of the field of quantum computation and quantum information. It asks the question: what are the ultimate physical limits to computation and communication? Fundamental Concepts -- Introduction and overview -- Introduction to quantum mechanics -- Introduction to computer science -- Quantum Computation -- Quantum circuits -- The quantum Fourier transform and its applications -- Quantum search algorithms -- Quantum computers: physical realisation -- Quantum Information -- Quantum noise, open quantum systems, and quantum operations -- Distance measurement for quantum information -- Quantum error-correction -- Entropy and information -- Quantum information theory -- Notes on basic probability theory -- Group theory -- Approximating quantum gates: the Solovay-Kitaev theorem -- Number theory -- Public-key cryptography and the RSA cryptosystem -- Proof of Lieb's theorem.},
author = {Nielsen, Michael A. and Chuang, Isaac L.},
isbn = {0521635039},
pages = {676},
publisher = {Cambridge University Press},
title = {{Quantum computation and quantum information}},
url = {https://books.google.com.au/books/about/Quantum{\_}Computation{\_}and{\_}Quantum{\_}Informat.html?id=65FqEKQOfP8C{\&}redir{\_}esc=y},
year = {2000}
}
@article{Gurvits2002,
author = {Gurvits, Leonid and Barnum, Howard},
doi = {10.1103/PhysRevA.66.062311},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {dec},
number = {6},
pages = {062311},
publisher = {American Physical Society},
title = {{Largest separable balls around the maximally mixed bipartite quantum state}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.66.062311},
volume = {66},
year = {2002}
}
@article{Bukov2018,
abstract = {We analyze state preparation within a restricted space of local control parameters between adiabatically connected states of control Hamiltonians. We formulate a conjecture that the time integral of energy fluctuations over the protocol duration is bounded from below by the geodesic length set by the quantum geometric tensor. The conjecture implies a geometric lower bound for the quantum speed limit (QSL). We prove the conjecture for arbitrary sufficiently slow protocols using adiabatic perturbation theory, and show that the bound is saturated by geodesic protocols, which keep the energy variance constant along the trajectory. Our conjecture implies that any optimal unit-fidelity protocol, even those which drive the system far from equilibrium, are fundamentally constrained by the quantum geometry of adiabatic evolution. When the control space includes all possible couplings, spanning the full Hilbert space, we recover the well-known Mandelstam-Tamm bound. However, using only accessible local controls to anneal in complex models such as glasses, or target individual excited states in quantum chaotic systems, the geometric bound for the QSL can be exponentially large in the system size due to a diverging geodesic length. We validate our conjecture both analytically by constructing counter-diabatic and fast-forward protocols for a three-level system, and numerically in non-integrable spin chains using optimal control.},
archivePrefix = {arXiv},
arxivId = {1804.05399},
author = {Bukov, Marin and Sels, Dries and Polkovnikov, Anatoli},
eprint = {1804.05399},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bukov, Sels, Polkovnikov - 2018 - The Geometric Speed Limit of Accessible Quantum State Preparation.pdf:pdf},
month = {apr},
title = {{The Geometric Speed Limit of Accessible Quantum State Preparation}},
url = {http://arxiv.org/abs/1804.05399},
year = {2018}
}
@article{Marvian,
abstract = {We introduce state-independent, nonperturbative Hamiltonian quantum speed limits for population leakage and fidelity loss, for a gapped open system interacting with a reservoir. These results hold in the presence of initial correlations between the system and the reservoir, under the sole assumption that their interaction and its commutator with the reservoir Hamiltonian are norm bounded. The reservoir need not be thermal and can be time dependent. We study the significance of energy mismatch between the system and the local degrees of freedom of the reservoir that directly interact with the system. We demonstrate that, in general, by increasing the system gap we may reduce this energy mismatch, and, consequently, drive the system and the reservoir into resonance; this can accelerate fidelity loss, irrespective of the thermal properties or state of the reservoir. This implies that quantum error suppression strategies based on increasing the gap are not uniformly beneficial. Our speed limits also yield an elementary lower bound on the relaxation time of spin systems. DOI: 10.1103/PhysRevLett.115.210402 PACS numbers: 03.67.Ac, 03.65.Yz, 03.67.Lx, 03.67.Pp Quantum speed limits (QSLs) answer the fundamental question of how fast a quantum system can evolve, and have numerous applications in, e.g., quantum computation, con-trol, and metrology. Traditionally, they characterize the minimum amount of time required for a quantum state of a closed quantum system to evolve to an orthogonal state. Mandelstam and Tamm (MT) [1] first showed that this time is lower bounded by the inverse of the standard deviation of the Hamiltonian. Margolus and Levitin (ML) [2] gave a different bound involving the inverse of the mean of the Hamiltonian, and the two bounds were subsequently unified [3]. These results led to numerous applications and exten-sions that go beyond the traditional QSLs and consider, e.g., the minimum time for optimal control or for implementing a unitary gate in quantum computation [4–20]. In this Letter, we are concerned with QSLs for open quantum systems [21], a question that has attracted signifi-cant recent attention [22–25]. While earlier work focused on generalizing the MT or ML bounds to the open-system setting, here we present state-independent, nonperturbative Hamiltonian QSL bounds for population leakage and fidelity loss, for a gapped open system interacting with a reservoir. The assumptions behind the results we present here are also different and independent from those behind previous such bounds. First, we make the (often natural) assumption that the system's initial state is restricted to an energy sector that is separated from the rest of the spectrum by a nonzero gap $\Delta$E, e.g., the ground subspace in various quantum information processing applications. Second, our bounds are independent of the state of the system or reservoir and, in particular, remain valid in the presence of initial correlations between the system and the reservoir. Third, our bounds are obtained purely at the Hamiltonian level. Thus, unlike most other open-system QSL bounds [22–25], we do not assume that the system's evolution is governed by a master equation or a completely positive channel. Our key result is given in Eqs. (6) and (7) below, and comprises fundamental QSL bounds on decoherence and leakage times, expressed in terms of $\Delta$E and the bounded norms of the interaction Hamiltonian and its commutator with the reservoir Hamiltonian, without assuming that the reservoir Hamiltonian is norm bounded. Note that applying the traditional closed system QSL bounds to the system and reservoir together in general yields bounds that are rather loose and independent of the gap $\Delta$E [26]. Given the very general assumptions behind our QSLs, they have a wide range of applicability similar to the previously known QSLs, including relaxation in many-body spin systems and limitations of control via a remote controller. The primary application on which we focus is quantum error suppression, where the goal is to slow down the loss of fidelity relative to some desired system state, e.g., in the context of quantum information processing tasks [27,28]. A common strategy to achieve fidelity enhance-ments is to use or generate energy gaps (e.g., [29–35]). Therefore, after deriving our QSLs, we study the depend-ence of the speed of decoherence and leakage on $\Delta$E. This enables us to find a general lower bound on the time scale for leakage. As expected, we find that in the $\Delta$E → ∞ limit the probability of leakage at any finite time goes to zero; moreover, if the error detection condition [36] holds, then in this limit the state retains its fidelity and remains},
author = {Marvian, Iman and Lidar, Daniel A},
doi = {10.1103/PhysRevLett.115.210402},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Marvian, Lidar - Unknown - Quantum Speed Limits for Leakage and Decoherence.pdf:pdf},
title = {{Quantum Speed Limits for Leakage and Decoherence}}
}
@article{Facchi2010,
abstract = {The tomographic picture of quantum mechanics has brought the description of quantum states closer to that of classical probability and statistics. On the other hand, the geometrical formulation of quantum mechanics introduces a metric tensor and a symplectic tensor (Hermitian tensor) on the space of pure states. By putting these two aspects together, we show that the Fisher information metric, both classical and quantum, can be described by means of the Hermitian tensor on the manifold of pure states.},
author = {Facchi, Paolo and Kulkarni, Ravi and Man'ko, V.I. and Marmo, Giuseppe and Sudarshan, E.C.G. and Ventriglia, Franco},
doi = {10.1016/J.PHYSLETA.2010.10.005},
issn = {0375-9601},
journal = {Phys. Lett. A},
month = {nov},
number = {48},
pages = {4801--4803},
publisher = {North-Holland},
title = {{Classical and quantum Fisher information in the geometrical formulation of quantum mechanics}},
url = {https://www.sciencedirect.com/science/article/pii/S0375960110013204?via{\%}3Dihub},
volume = {374},
year = {2010}
}
@article{Engl,
abstract = {We predict a generic signature of quantum interference in many-body bosonic systems resulting in a coherent enhancement of the average return probability in Fock space. This enhancement is robust with respect to variations of external parameters even though it represents a dynamical manifestation of the delicate superposition principle in Fock space. It is a genuine quantum many-body effect that lies beyond the reach of any mean-field approach. Using a semiclassical approach based on interfering paths in Fock space, we calculate the magnitude of the backscattering peak and its dependence on gauge fields that break time-reversal invariance. We confirm our predictions by comparing them to exact quantum evolution probabilities in Bose-Hubbard models, and discuss their relevance in the context of many-body thermalization.},
archivePrefix = {arXiv},
arxivId = {1306.3169},
author = {Engl, Thomas and Dujardin, Julien and Arg??elles, Arturo and Schlagheck, Peter and Richter, Klaus and Urbina, Juan Diego},
doi = {10.1103/PhysRevLett.112.140403},
eprint = {1306.3169},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Engl et al. - Unknown - Coherent Backscattering in Fock Space A Signature of Quantum Many-Body Interference in Interacting Bosonic Syste.pdf:pdf},
isbn = {0031-9007 1079-7114},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {14},
title = {{Coherent backscattering in fock space: A signature of quantum many-body interference in interacting bosonic systems}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.112.140403},
volume = {112},
year = {2014}
}
@article{Vandersypen2005,
author = {Vandersypen, L. M. K. and Chuang, I. L.},
doi = {10.1103/RevModPhys.76.1037},
issn = {0034-6861},
journal = {Rev. Mod. Phys.},
month = {jan},
number = {4},
pages = {1037--1069},
publisher = {American Physical Society},
title = {{NMR techniques for quantum control and computation}},
url = {https://link.aps.org/doi/10.1103/RevModPhys.76.1037},
volume = {76},
year = {2005}
}
@article{Fischer2019,
archivePrefix = {arXiv},
arxivId = {1901.05756},
author = {Fischer, Jonas and Basilewitsch, Daniel and Koch, Christiane P. and Sugny, Dominique},
eprint = {1901.05756},
file = {::},
month = {jan},
title = {{Time-optimal purification of a qubit in contact with a structured environment}},
url = {https://arxiv.org/abs/1901.05756},
year = {2019}
}
@article{Le2017,
abstract = {Recently, it has been shown that energy can be deposited on a collection of quantum systems at a rate that scales super-extensively. Some of these schemes for `quantum batteries' rely on the use of global many-body interactions that take the batteries through a correlated short cut in state space. Here, we extend the notion of a quantum battery from a collection of a priori isolated systems to a many-body quantum system with intrinsic interactions. Specifically, we consider a one-dimensional spin chain with physically realistic two-body interactions. We find that the spin-spin interactions can yield an advantage in charging power over the non-interacting case, and we demonstrate that this advantage can grow super-extensively when the interactions are long ranged. However, we show that, unlike in previous work, this advantage is a mean-field interaction effect that does not involve correlations and that relies on the interactions being intrinsic to the battery.},
archivePrefix = {arXiv},
arxivId = {1712.03559},
author = {Le, Thao P. and Levinsen, Jesper and Modi, Kavan and Parish, Meera M. and Pollock, Felix A.},
doi = {10.1103/PhysRevA.97.022106},
eprint = {1712.03559},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Le et al. - 2017 - Spin-chain model of a many-body quantum battery.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Le et al. - 2018 - Spin-chain model of a many-body quantum battery.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {feb},
number = {2},
pages = {022106},
publisher = {American Physical Society},
title = {{Spin-chain model of a many-body quantum battery}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.97.022106 http://arxiv.org/abs/1712.03559},
volume = {97},
year = {2017}
}
@article{Yang2017,
author = {Yang, Fan and Koll{\'{a}}r, Alicia J. and Taylor, Stephen F. and Turner, Richard W. and Lev, Benjamin L.},
doi = {10.1103/PhysRevApplied.7.034026},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Yang et al. - 2017 - Scanning Quantum Cryogenic Atom Microscope.pdf:pdf},
issn = {2331-7019},
journal = {Phys. Rev. Appl.},
month = {mar},
number = {3},
pages = {034026},
publisher = {American Physical Society},
title = {{Scanning Quantum Cryogenic Atom Microscope}},
url = {https://link.aps.org/doi/10.1103/PhysRevApplied.7.034026},
volume = {7},
year = {2017}
}
@article{Saha2017,
abstract = {With special attention to the role of information theory in physical sciences we present analytical results for the coordinate-and momentum-space Fisher information of some important one-dimensional quantum systems which differ in spacing of their energy levels. The studies envisaged allow us to relate the coordinate-space information (r I) with the familiar energy levels of the quantum system. The corresponding momentum-space information (g I) does not obey such a simple relationship with the energy spectrum. Our results for the product (r g I I) depend quadratically on the principal quantum number n and satisfy an appropriate uncertainty relation derived by Dehesa et al (2007 J. Phys. A: Math. Theor. 40 1845)},
author = {Saha, Aparna and Talukdar, B and Chatterjee, Supriya and Bakal, S and Kim, Y S and Noz, M E and Saha, Aparna and Talukdar, B and Chatterjee, Supriya},
doi = {10.1088/1361-6404/aa51a0},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bakal et al. - 2017 - On the realization of quantum Fisher information.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Saha, Talukdar, Chatterjee - 2017 - On the realization of quantum Fisher information.pdf:pdf},
issn = {0143-0807},
keywords = {1D quantum systems,Fisher information,energy eigenvalues,physical realization,relation},
month = {mar},
number = {2},
pages = {025103},
publisher = {IOP Publishing},
title = {{On the realization of quantum Fisher information}},
url = {http://iopscience.iop.org/0143-0807/38/2/025103 http://stacks.iop.org/0143-0807/38/i=2/a=025103?key=crossref.a5406b4069741334ef63450bb7f08ac6},
volume = {38},
year = {2017}
}
@article{Scully2003,
author = {Scully, Marlan O. and Zubairy, M. Suhail and Agarwal, Girish S. and Walther, Herbert},
doi = {10.1126/science.1078955},
journal = {Science (80-. ).},
number = {5608},
pages = {862--864},
title = {{Extracting Work from a Single Heat Bath via Vanishing Quantum Coherence}},
volume = {299},
year = {2003}
}
@article{Zwierz2012,
author = {Zwierz, Marcin},
doi = {10.1103/PhysRevA.86.016101},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zwierz - 2012 - Comment on “Geometric derivation of the quantum speed limit”.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jul},
number = {1},
pages = {016101},
publisher = {American Physical Society},
title = {{Comment on “Geometric derivation of the quantum speed limit”}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.86.016101},
volume = {86},
year = {2012}
}
@article{Carlini2006,
author = {Carlini, Alberto and Hosoya, Akio and Koike, Tatsuhiko and Okudaira, Yosuke},
doi = {10.1103/PhysRevLett.96.060503},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Carlini et al. - 2006 - Time-Optimal Quantum Evolution.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {6},
pages = {060503},
publisher = {American Physical Society},
title = {{Time-Optimal Quantum Evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.060503},
volume = {96},
year = {2006}
}
@article{Duncan2018,
archivePrefix = {arXiv},
arxivId = {1811.10336},
author = {Duncan, Cody B. and Kirchgae{\ss}er, Patrick},
eprint = {1811.10336},
file = {::},
month = {nov},
title = {{Kinematic strangeness production in cluster hadronization}},
url = {https://arxiv.org/abs/1811.10336},
year = {2018}
}
@article{Jurcevic2014,
abstract = {The key to explaining a wide range of quantum phe-nomena is understanding how entanglement propagates around many-body systems. Furthermore, the controlled distribution of entanglement is of fundamental impor-tance for quantum communication and computation. In many situations, quasiparticles are the carriers of infor-mation around a quantum system and are expected to dis-tribute entanglement in a fashion determined by the sys-tem interactions [1]. Here we report on the observation of magnon quasiparticle dynamics in a one-dimensional many-body quantum system of trapped ions representing an Ising spin model [2, 3]. Using the ability to tune the effective interaction range [4–6], and to prepare and mea-sure the quantum state at the individual particle level, we observe new quasiparticle phenomena. For the first time, we reveal the entanglement distributed by quasiparticles around a many-body system. Second, for long-range in-teractions we observe the divergence of quasiparticle ve-locity and breakdown of the light-cone picture [7–10] that is valid for short-range interactions. Our results will al-low experimental studies of a wide range of phenomena, such as quantum transport [11, 12], thermalisation [13], localisation [14] and entanglement growth [15], and rep-resent a first step towards a new quantum-optical regime with on-demand quasiparticles with tunable non-linear in-teractions. Quasiparticles, such as magnons, phonons, and anyons, are elementary excitations in the collective behaviour of an un-derlying many-body quantum system. While precise control is already possible in the laboratory for systems of individual atoms, ions, or photons, it remains a challenge to extend this to quasiparticles. In systems with nearest-neighbour interac-tions, quasiparticles are expected to distribute entanglement within light-like-cones defined by a strict quantum informa-tion speed limit, enforced not by relativity but by the finite interaction range itself [7, 16, 17]. These results, known as Lieb-Robinson bounds, have allowed various important theo-rems to be proven about systems with nearest-neighbour in-teractions, including restrictions on ground-state correlations [18, 19] and the time to create states for topological quan-tum computation [16]. Recently, wavefronts of correlations have been observed in bosonic atoms in optical lattices with nearest-neighbour interactions [20, 21], and an outstanding challenge is to observe the entanglement dynamics.},
author = {Jurcevic, P and Lanyon, B P and Hauke, P and Hempel, C and Zoller, P and Blatt, R and Roos, C F},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Jurcevic et al. - 2014 - Observation of entanglement propagation in a quantum many-body system.pdf:pdf},
title = {{Observation of entanglement propagation in a quantum many-body system}},
year = {2014}
}
@article{Perarnau-Llobet,
abstract = {We derive general limitations concerning efficiency and power of heat engines strongly coupled to thermal baths. We build this framework on the insight that quantum systems strongly coupled to many-body systems will equilibrate to the reduced state of a global thermal state, deviating from the local thermal state of the system as it occurs in the weak-coupling limit. Taking this observation as the starting point of our analysis, we first provide strong-coupling corrections to the second law in three of its different readings: As a statement of maximal extractable work, on heat dissipation, and bound to the Carnot efficiency. The corrections identified become relevant for small quantum systems and always vanish in first order in the interaction strength. We then move to the question of power of heat engines, obtaining a bound on the power enhancement due to strong coupling. To exemplify our results, we discuss the implications on the paradigmatic situation of non-Markovian quantum Brownian motion.},
author = {Perarnau-Llobet, M and Wilming, H and Riera, A and Gallego, R and Eisert, J},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Perarnau-Llobet et al. - Unknown - Fundamental corrections to work and power in the strong coupling regime.pdf:pdf},
title = {{Fundamental corrections to work and power in the strong coupling regime}},
url = {https://arxiv.org/pdf/1704.05864.pdf}
}
@article{Davie2013,
abstract = {{\textless}p{\textgreater} We give a new bound {\textless}italic{\textgreater}$\omega${\textless}/italic{\textgreater} {\&}lt; 2.37369 for the exponent of complexity of matrix multiplication, giving a small improvement on the previous bound obtained by Coppersmith and Winograd. The proof involves an extension of the method used by these authors. We have attempted to make the exposition self-contained. {\textless}/p{\textgreater}},
author = {Davie, A. M. and Stothers, A. J.},
doi = {10.1017/S0308210511001648},
issn = {0308-2105},
journal = {Proc. R. Soc. Edinburgh Sect. A Math.},
month = {apr},
number = {02},
pages = {351--369},
title = {{Improved bound for complexity of matrix multiplication}},
url = {http://www.journals.cambridge.org/abstract{\_}S0308210511001648},
volume = {143},
year = {2013}
}
@article{Zhang2019,
abstract = {Reinforcement learning has been widely used in many problems including quantum control of qubits. However, such problems can, at the same time, be solved by traditional, non-machine-learning based methods such as stochastic gradient descendent and Krotov algorithms, and it remains unclear which one is most suitable when the control has specific constraints. In this work we perform a comparative study on the efficacy of two reinforcement learning algorithms, Q-learning and deep Q-learning, as well as stochastic gradient descendent and Krotov algorithms, in the problem of preparing a desired quantum state. We found that overall, the deep Q-learning outperforms others when the problem is discretized, e.g. allowing discrete values of control. The Q-learning and deep Q-learning can also adaptively reduce the complexity of the control sequence, shortening the operation time and improving the fidelity. Our comparison provides insights on the suitability of reinforcement learning in quantum control problems.},
archivePrefix = {arXiv},
arxivId = {1902.02157},
author = {Zhang, Xiao-Ming and Wei, Zezhu and Asad, Raza and Yang, Xu-Chen and Wang, Xin},
eprint = {1902.02157},
file = {::},
month = {feb},
title = {{When reinforcement learning stands out in quantum control? A comparative study on state preparation}},
url = {http://arxiv.org/abs/1902.02157},
year = {2019}
}
@book{AmericanMathematicalSociety.1989,
author = {{American Mathematical Society.}, Fumio and {United States. National Bureau of Standards.}, Yoshihiro and {Institute for Numerical Analysis (U.S.)}},
booktitle = {Pacific J. Math.},
issn = {0030-8730},
month = {jun},
number = {2},
pages = {259--294},
publisher = {Pacific Journal of Mathematics, etc.]},
title = {{Pacific journal of mathematics.}},
url = {https://msp.org/pjm/1989/138-2/p06.xhtml},
volume = {138},
year = {1989}
}
@article{Lohmayer2006,
abstract = {We provide a complete analysis of mixed three-qubit states composed of a Greenberger-Horne-Zeilinger state and a W state orthogonal to the former. We present optimal decompositions and convex roofs for the three-tangle. Further, we provide an analytical method to decide whether or not an arbitrary rank-2 state of three qubits has vanishing three-tangle. These results highlight intriguing differences compared to the properties of two-qubit mixed states, and may serve as a quantitative reference for future studies of entanglement in multipartite mixed states. By studying the Coffman-Kundu-Wootters inequality we find that, while the amounts of inequivalent entanglement types strictly add up for pure states, this "monogamy" can be lifted for mixed states by virtue of vanishing tangle measures.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0606071},
author = {Lohmayer, Robert and Osterloh, Andreas and Siewert, Jens and Uhlmann, Armin},
doi = {10.1103/PhysRevLett.97.260502},
eprint = {0606071},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Lohmayer et al. - 2006 - Entangled Three-Qubit States without Concurrence and Three-Tangle.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Lohmayer et al. - 2006 - Entangled Three-Qubit States without Concurrence and Three-Tangle(2).pdf:pdf},
isbn = {0031-9007 1079-7114},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {26},
pages = {260502},
pmid = {17280411},
primaryClass = {quant-ph},
publisher = {American Physical Society},
title = {{Entangled Three-Qubit States without Concurrence and Three-Tangle}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.97.260502},
volume = {97},
year = {2006}
}
@article{Pendry1983,
author = {Pendry, J B},
doi = {10.1088/0305-4470/16/10/012},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Unknown - 1983 - Quantum limits to the flow of information and entropy.pdf:pdf},
issn = {0305-4470},
journal = {J. Phys. A. Math. Gen.},
number = {10},
pages = {2161},
publisher = {IOP Publishing},
title = {{Quantum limits to the flow of information and entropy}},
url = {http://iopscience.iop.org/article/10.1088/0305-4470/16/10/012/meta},
volume = {16},
year = {1983}
}
@incollection{Mandelstam1945,
address = {Berlin, Heidelberg},
author = {Mandelstam, L. and Tamm, I.},
booktitle = {Sel. Pap.},
doi = {10.1007/978-3-642-74626-0_8},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Mandelstam, Tamm - 1991 - The Uncertainty Relation Between Energy and Time in Non-relativistic Quantum Mechanics.pdf:pdf},
pages = {115--123},
publisher = {Springer Berlin Heidelberg},
title = {{The Uncertainty Relation Between Energy and Time in Non-relativistic Quantum Mechanics}},
year = {1945}
}
@article{Campbell2017,
author = {Campbell, Steve and Deffner, Sebastian},
doi = {10.1103/PhysRevLett.118.100601},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campbell, Deffner - 2017 - Trade-Off Between Speed and Cost in Shortcuts to Adiabaticity.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campbell, Deffner - 2017 - Trade-Off Between Speed and Cost in Shortcuts to Adiabaticity(3).pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {10},
pages = {100601},
publisher = {American Physical Society},
title = {{Trade-Off Between Speed and Cost in Shortcuts to Adiabaticity}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.100601},
volume = {118},
year = {2017}
}
@article{Dietz2006,
author = {Dietz, Klaus},
doi = {10.1088/0305-4470/39/6/016},
file = {::},
issn = {0305-4470},
journal = {J. Phys. A. Math. Gen.},
month = {feb},
number = {6},
pages = {1433--1447},
publisher = {IOP Publishing},
title = {{Generalized Bloch spheres for {\textless}i{\textgreater}m{\textless}/i{\textgreater} -qubit states}},
url = {http://stacks.iop.org/0305-4470/39/i=6/a=016?key=crossref.bbc17b8062dce976ef743a2988fcf9f0},
volume = {39},
year = {2006}
}
@article{Benatti2010,
abstract = {The usual notion of separability has to be reconsidered when applied to states describing identical particles. A definition of separability not related to any a priori Hilbert space tensor product structure is needed: this can be given in terms of commuting subalgebras of observables. Accordingly, the results concerning the use of the quantum Fisher information in quantum metrology are generalized and physically reinterpreted.},
author = {Benatti, F. and Floreanini, R. and Marzolino, U.},
doi = {10.1016/j.aop.2010.01.005},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Benatti, Floreanini, Marzolino - 2010 - Sub-shot-noise quantum metrology with entangled identical particles.pdf:pdf},
issn = {00034916},
journal = {Ann. Phys. (N. Y).},
number = {4},
pages = {924--935},
title = {{Sub-shot-noise quantum metrology with entangled identical particles}},
volume = {325},
year = {2010}
}
@article{Basilewitsch2017,
author = {Basilewitsch, Daniel and Schmidt, Rebecca and Sugny, Dominique and Maniscalco, Sabrina and Koch, Christiane P},
doi = {10.1088/1367-2630/aa96f8},
issn = {1367-2630},
journal = {New J. Phys.},
month = {nov},
number = {11},
pages = {113042},
publisher = {IOP Publishing},
title = {{Beating the limits with initial correlations}},
url = {http://stacks.iop.org/1367-2630/19/i=11/a=113042?key=crossref.0453294715cb89bce6263c03f5addf0b},
volume = {19},
year = {2017}
}
@article{Nagata2009,
author = {Nagata, Koji},
doi = {10.1007/s10773-009-0139-2},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Nagata - 2009 - Necessary and Sufficient Condition for Greenberger-Horne-Zeilinger Diagonal States to Be Full N-partite Entangled.pdf:pdf},
issn = {0020-7748},
journal = {Int. J. Theor. Phys.},
month = {dec},
number = {12},
pages = {3358--3364},
publisher = {Springer US},
title = {{Necessary and Sufficient Condition for Greenberger-Horne-Zeilinger Diagonal States to Be Full N-partite Entangled}},
url = {http://link.springer.com/10.1007/s10773-009-0139-2},
volume = {48},
year = {2009}
}
@article{DelCampo2012,
author = {del Campo, Adolfo and Rams, Marek M. and Zurek, Wojciech H.},
doi = {10.1103/PhysRevLett.109.115703},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/del Campo, Rams, Zurek - 2012 - Assisted Finite-Rate Adiabatic Passage Across a Quantum Critical Point Exact Solution for the Quantum Is.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {sep},
number = {11},
pages = {115703},
publisher = {American Physical Society},
title = {{Assisted Finite-Rate Adiabatic Passage Across a Quantum Critical Point: Exact Solution for the Quantum Ising Model}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.115703},
volume = {109},
year = {2012}
}
@article{Bath2007,
author = {Bath, Jonathan and Turberfield, Andrew J.},
doi = {10.1038/nnano.2007.104},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bath, Turberfield - 2007 - DNA nanomachines.pdf:pdf},
issn = {1748-3387},
month = {may},
number = {5},
pages = {275--284},
publisher = {Nature Publishing Group},
title = {{DNA nanomachines}},
url = {http://www.nature.com/doifinder/10.1038/nnano.2007.104 https://www.nature.com/articles/nnano.2007.104.pdf},
volume = {2},
year = {2007}
}
@article{Gray2005,
abstract = {In the Mandelstam–Tamm version of the time-energy uncertainty principle $\Delta$t denotes the infimum of time intervals that elapse before the change in the mean of any observable has the same magnitude as its standard deviation. We clarify this interpretation, and show that the infimum is achieved for certain observables and thus that this famous inequality is actually an equality.},
author = {Gray, John E. and Vogt, Andrew},
doi = {10.1063/1.1897164},
issn = {0022-2488},
journal = {J. Math. Phys.},
keywords = {indeterminancy,mathematical analysis},
month = {may},
number = {5},
pages = {052108},
publisher = {American Institute of Physics},
title = {{Mathematical analysis of the Mandelstam–Tamm time-energy uncertainty principle}},
url = {http://aip.scitation.org/doi/10.1063/1.1897164},
volume = {46},
year = {2005}
}
@article{Peirce1988,
abstract = {The optimal control of the path to a specified 6nal state of a quantum-mechanical system is inves-tigated. The problem is formulated as a minimization problem over appropriate function spaces, and the well-posedness of this problem is is established by proving the existence of an optimal solu-tion. A I.agrange-multiplier technique is used to reduce the problem to an equivalent optimization problem and to derive necessary conditions for a minimum. These necessary conditions form the basis for a gradient iterative procedure to search for a minimum. A numerical scheme based on 6nite di8'erences is used to reduce the in6nite-dimensional minimization problem to an approximate finite-dimensional problem. Numerical examples are provided for 6nal-state control of a diatomic molecule represented by a Morse potential. {\%}ithia the context of this optimal control formulation, numerical results are given for the optimal pulsing strategy to demonstrate the feasibility of wave-packet control and 6nally to achieve a speci6ed dissociative wave packet at a given time. The op-timal external optical Aelds generally have a high degree of structure, including an early time period of wave-packet phase adjustment followed by a period of extensive energy deposition to achieve the imposed objective. Constraints on the form of the molecular dipole (e.g. , a linear dipole) are shown to limit the accessibility (i.e. , controllability) of certain types of molecular wave-packet objectives. The nontrivial structure of the optimal pulse strategies emphasizes the ultimate usefulness of an optimal-control approach to the steering of quantum systems to desired objectives.},
author = {Peirce, Anthony P and Dahleh, Mohammed A and Rabitz, Herschel},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Peirce, Dahleh, Rabitz - 1988 - Optimal control of quantum-mechanical systems Existence, numerical approximation, and appbcations.pdf:pdf},
number = {15},
title = {{Optimal control of quantum-mechanical systems: Existence, numerical approximation, and appbcations}},
volume = {37},
year = {1988}
}
@article{Souza2011,
abstract = {Error correction in quantum computing can be implemented using transversal gates, which in turn rely on the availability of so-called magic states. The authors experimentally show that it is possible to improve the fidelity of these states by distilling five of them into one.},
author = {Souza, Alexandre M. and Zhang, Jingfu and Ryan, Colm A. and Laflamme, Raymond},
doi = {10.1038/ncomms1166},
file = {::},
issn = {2041-1723},
journal = {Nat. Commun.},
keywords = {Atomic and molecular physics,Quantum information,Theoretical physics},
month = {sep},
number = {1},
pages = {169},
publisher = {Nature Publishing Group},
title = {{Experimental magic state distillation for fault-tolerant quantum computing}},
url = {http://www.nature.com/articles/ncomms1166},
volume = {2},
year = {2011}
}
@article{Pusz1978,
author = {Pusz, W. and Woronowicz, S. L.},
doi = {10.1007/BF01614224},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pusz, Woronowicz - 1978 - Passive states and KMS states for general quantum systems.pdf:pdf},
issn = {0010-3616},
journal = {Commun. Math. Phys.},
month = {oct},
number = {3},
pages = {273--290},
publisher = {Springer-Verlag},
title = {{Passive states and KMS states for general quantum systems}},
url = {http://link.springer.com/10.1007/BF01614224},
volume = {58},
year = {1978}
}
@article{Zhang2016,
abstract = {Important properties of a quantum system are not directly measurable, but they can be disclosed by how fast the system changes under controlled perturbations. In particular, asymmetry and entanglement can be verified by reconstructing the state of a quantum system. Yet, this usually requires experimental and computational resources which increase exponentially with the system size. Here we show how to detect metrologically useful asymmetry and entanglement by a limited number of measurements. This is achieved by studying how they affect the speed of evolution of a system under a unitary transformation. We show that the speed of multiqubit systems can be evaluated by measuring a set of local observables, providing exponential advantage with respect to state tomography. Indeed, the presented method requires neither the knowledge of the state and the parameter-encoding Hamiltonian nor global measurements performed on all the constituent subsystems. We implement the detection scheme in an all-optical experiment.},
archivePrefix = {arXiv},
arxivId = {1611.02004},
author = {Zhang, Chao and Yadin, Benjamin and Hou, Zhi-Bo and Cao, Huan and Liu, Bi-Heng and Huang, Yun-Feng and Maity, Reevu and Vedral, Vlatko and Li, Chuan-Feng and Guo, Guang-Can and Girolami, Davide},
doi = {10.1103/PhysRevA.96.042327},
eprint = {1611.02004},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zhang et al. - 2017 - Detecting metrologically useful asymmetry and entanglement by a few local measurements.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zhang et al. - 2016 - Detecting metrologically useful asymmetry and entanglement by a few local measurements.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {nov},
number = {4},
pages = {042327},
publisher = {American Physical Society},
title = {{Detecting metrologically useful asymmetry and entanglement by a few local measurements}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.96.042327 http://arxiv.org/abs/1611.02004 http://dx.doi.org/10.1103/PhysRevA.96.042327},
volume = {96},
year = {2016}
}
@article{Hwang2003,
author = {Hwang, Won-Young},
doi = {10.1103/PhysRevLett.91.057901},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hwang - 2003 - Quantum Key Distribution with High Loss Toward Global Secure Communication.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
number = {5},
pages = {057901},
publisher = {American Physical Society},
title = {{Quantum Key Distribution with High Loss: Toward Global Secure Communication}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.91.057901},
volume = {91},
year = {2003}
}
@article{Wang2009,
author = {Wang, Xiaoting and Schirmer, S. G.},
doi = {10.1103/PhysRevA.79.052326},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wang, Schirmer - 2009 - Contractivity of the Hilbert-Schmidt distance under open-system dynamics.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {may},
number = {5},
pages = {052326},
publisher = {American Physical Society},
title = {{Contractivity of the Hilbert-Schmidt distance under open-system dynamics}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.79.052326},
volume = {79},
year = {2009}
}
@article{Aharonov1961,
abstract = {Because time does not appear in Schr{\"{o}}dinger's equation as an operator but only as a parameter, the time-energy uncertainty relation must be formulated in a special way. This problem has in fact been studied by many authors and we give a summary of their treatments. We then criticize the main conclusion of these treatments; viz., that in a measurement of energy carried out in a time interval, $\Delta$t, there must be a minimum uncertainty in the transfer of energy to the observed system, given by $\Delta$(E′-E){\textgreater}{\~{}}h/$\Delta$t. We show that this conclusion is erroneous in two respects. First, it is not consistent with the general principles of the quantum theory, which require that all uncertainty relations be expressible in terms of the mathematical formalism, i.e., by means of operators, wave functions, etc. Secondly, the examples of measurement processes that were used to derive the above uncertainty relation are not general enough. We then develop a systematic presentation of our own point of view, with regard to the role of time in the quantum theory, and give a concrete example of a measurement process not satisfying the above uncertainty relation.},
author = {Aharonov, Y. and Bohm, D.},
doi = {10.1103/PhysRev.122.1649},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Aharonov, Bohm - 1961 - Time in the Quantum Theory and the Uncertainty Relation for Time and Energy.pdf:pdf},
isbn = {9780874216561},
issn = {0031899X},
journal = {Phys. Rev.},
month = {jun},
number = {5},
pages = {1649--1658},
pmid = {25052830},
publisher = {American Physical Society},
title = {{Time in the quantum theory and the uncertainty relation for time and energy}},
url = {https://link.aps.org/doi/10.1103/PhysRev.122.1649},
volume = {122},
year = {1961}
}
@book{Breuer2002,
author = {Breuer, Heinz-Peter and Petruccione, F. (Francesco)},
isbn = {9780199213900},
pages = {625},
publisher = {Oxford University Press},
title = {{The theory of open quantum systems}},
year = {2002}
}
@article{Islam2011,
abstract = {A quantum simulator can follow the evolution of a prescribed model, whose behaviour may be difficult to determine. Here, the emergence of magnetism is simulated by implementing a quantum Ising model, providing a benchmark for simulations in larger systems.},
author = {Islam, R. and Edwards, E.E. and Kim, K. and Korenblit, S. and Noh, C. and Carmichael, H. and Lin, G.-D. and Duan, L.-M. and {Joseph Wang}, C.-C. and Freericks, J.K. and Monroe, C.},
doi = {10.1038/ncomms1374},
file = {::},
issn = {2041-1723},
journal = {Nat. Commun.},
keywords = {Atomic and molecular interactions with photons,Condensed,Quantum information,matter physics},
month = {sep},
number = {1},
pages = {377},
publisher = {Nature Publishing Group},
title = {{Onset of a quantum phase transition with a trapped ion quantum simulator}},
url = {http://www.nature.com/articles/ncomms1374},
volume = {2},
year = {2011}
}
@article{Alicki1979,
author = {Alicki, R},
doi = {10.1088/0305-4470/12/5/007},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Alicki - 1979 - The quantum open system as a model of the heat engine.pdf:pdf},
journal = {J. Phys. A. Math. Gen.},
month = {may},
number = {5},
pages = {L103--L107},
publisher = {IOP Publishing},
title = {{The quantum open system as a model of the heat engine}},
url = {http://stacks.iop.org/0305-4470/12/i=5/a=007?key=crossref.98fc4bbe6a0bb0341479c8ece6f35991},
volume = {12},
year = {1979}
}
@article{Bruning2012,
abstract = {This article gives a brief overview of some recent progress in the characterization and parametrization of density matrices of finite dimensional systems. We discuss in some detail the Bloch-vector and Jarlskog parametrizations and mention briefly the coset parametrization. As applications of the Bloch parametrization we discuss the trace invariants for the case of time dependent Hamiltonians and in some detail the dynamics of three-level systems. Furthermore, the Bloch vector of two-qubit systems as well as the use of the polarization operator basis is indicated. As the main application of the Jarlskog parametrization we construct density matrices for composite systems. In addition, some recent related articles are mentioned without further discussion.},
author = {Br{\"{u}}ning, E. and M{\"{a}}kel{\"{a}}, H. and Messina, A. and Petruccione, F.},
doi = {10.1080/09500340.2011.632097},
issn = {0950-0340},
journal = {J. Mod. Opt.},
keywords = {Bloch vector,Jarlskog parametrization,density matrix parametrization,finite-dimensional density matrix,quantum optics (inc. quantum information)},
month = {jan},
number = {1},
pages = {1--20},
publisher = { Taylor {\&} Francis Group },
title = {{Parametrizations of density matrices}},
url = {http://www.tandfonline.com/doi/abs/10.1080/09500340.2011.632097},
volume = {59},
year = {2012}
}
@article{Robertson1929,
author = {Robertson, H. P.},
doi = {10.1103/PhysRev.34.163},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Robertson - 1929 - The Uncertainty Principle.pdf:pdf},
journal = {Phys. Rev.},
number = {1},
pages = {163--164},
publisher = {American Physical Society},
title = {{The Uncertainty Principle}},
url = {http://link.aps.org/doi/10.1103/PhysRev.34.163},
volume = {34},
year = {1929}
}
@incollection{Uhlmann1992a,
address = {Dordrecht},
author = {Uhlmann, Armin},
booktitle = {Groups Relat. Top.},
doi = {10.1007/978-94-011-2801-8_23},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uhlmann - 1992 - The Metric of Bures and the Geometric Phase.pdf:pdf},
number = {1991},
pages = {267--274},
publisher = {Springer Netherlands},
title = {{The Metric of Bures and the Geometric Phase}},
url = {http://www.springerlink.com/index/10.1007/978-94-011-2801-8{\_}23},
year = {1992}
}
@article{Miyake2003,
abstract = {We find that multidimensional determinants "hyperdeterminants", related to entanglement measures (the so-called concurrence or 3-tangle for the 2 or 3 qubits, respectively), are derived from a duality between entangled states and separable states. By means of the hyperdeterminant and its singularities, the single copy of multipartite pure entangled states is classified into an onion structure of every closed subset, similar to that by the local rank in the bipartite case. This reveals how inequivalent multipartite entangled classes are partially ordered under local actions. In particular, the generic entangled class of the maximal dimension, distinguished as the nonzero hyperdeterminant, does not include the maximally entangled states in Bell's inequalities in general (e.g., in the {\$}n \backslashgeq 4{\$} qubits), contrary to the widely known bipartite or 3-qubit cases. It suggests that not only are they never locally interconvertible with the majority of multipartite entangled states, but they would have no grounds for the canonical n-partite entangled states. Our classification is also useful for the mixed states.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0206111},
author = {Miyake, Akimasa},
doi = {10.1103/PhysRevA.67.012108},
eprint = {0206111},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Miyake - Unknown - Classification of multipartite entangled states by multidimensional determinants.pdf:pdf},
isbn = {1050-2947},
issn = {1050-2947},
journal = {Phys. Rev. A},
number = {1},
pages = {012108},
primaryClass = {quant-ph},
title = {{Classification of multipartite entangled states by multidimensional determinants}},
url = {http://arxiv.org/abs/quant-ph/0206111{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRevA.67.012108},
volume = {67},
year = {2003}
}
@article{Zhang,
abstract = {We investigate theoretically a quantum optomechanical realization of a heat engine. In a generic optomechanical arrangement the optomechanical coupling between the cavity field and the oscillating end mirror results in polariton normal mode excitations whose character depends on the pump detuning and the coupling strength. By varying that detuning it is possible to transform their character from phononlike to photonlike, so that they are predominantly coupled to the thermal reservoir of phonons or photons, respectively. We exploit the fact that the effective temperatures of these two reservoirs are different to produce an Otto cycle along one of the polariton branches. We discuss the basic properties of the system in two different regimes: in the optical domain it is possible to extract work from the thermal energy of a mechanical resonator at finite temperature, while in the microwave range one can in principle exploit the cycle to extract work from the blackbody radiation background coupled to an ultracold atomic ensemble. DOI: 10.1103/PhysRevLett.112.150602 PACS numbers: 05.70.-a, 07.10.Cm, 42.50.Lc, 42.50.Wk Heat engines operating in the quantum regime have attracted much recent attention due to their potential to investigate the quantum limit of classical thermodynamical concepts such as the Carnot efficiency limit—and perhaps overcome that limit, to better understand thermalization in the deep quantum regime, and, on a more applied side, in the quest for the realization of nanoengines of increasingly small size [1–5]. Microscopic scale heat engines have been realized in micro-electro-mechanical systems [6,7], but reaching the quantum regime remains a challenge due to thermal noise in the mechanical elements. Theoretical proposals for quantum heat engines have been advanced involving single ions [8], ultracold bosonic atoms [9], and quantum dots [10], but so far their experimental realization has remained elusive. This Letter proposes and analyzes theoretically a quan-tum heat engine based on a cavity optomechanical setup. This system presents several attractive features: first, it is a truly mechanical system; second, it has the potential to operate deep in the quantum regime using existing, state-of-the-art equipment; third, it is conceptually extremely simple; and fourth, it offers, in principle at least, the potential to extract work from the 2.7 K blackbody radiation back-ground. Finally, when combined with progress in quantum optics toward the realization of squeezed reservoirs [11], it may provide a route to testing the Carnot efficiency limit in the quantum regime. The key element of a heat engine is a medium that may be used to extract work and that exchanges heat with thermal reservoirs at two different temperatures. Cavity optome-chanics provides a conceptually simple way to realize that goal: The radiation pressure force permits the exchange of energy between cavity photons and mechanical phonons, and crucially the cavity and mechanical damping couple the system to both a cold and a hot reservoir. Cavity optomechanics has witnessed spectacular developments in the last decade (see, e.g., Refs [12–14] for recent reviews), and can operate deep in the quantum regime [15–17]. Also, quantum entanglement and squeezed states of photons and phonons have been demonstrated in these systems [18,19]. We consider a standard optomechanical setup with a cavity mode at frequency $\omega$ c coupled to a mechanical resonator at frequency $\omega$ m —for example, the harmonically bound end mirror of a Fabry-P{\'{e}}rot resonator, with single-photon coupling strength g. The resonator is driven by an optical pump field with strength $\alpha$ in and frequency $\omega$ p . In addition, the intracavity field and mechanical oscillator suffer damping of rates $\kappa$ and $\gamma$. We assume that the intracavity field is strong enough that it can be described as the sum of a large mean field $\alpha$ and small quantum fluctuations. In a frame rotating at $\omega$ p the Hamiltonian of the entire system can then be linearized as},
author = {Zhang, Keye and Bariani, Francesco and Meystre, Pierre},
doi = {10.1103/PhysRevLett.112.150602},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zhang, Bariani, Meystre - Unknown - Quantum Optomechanical Heat Engine.pdf:pdf},
title = {{Quantum Optomechanical Heat Engine}}
}
@article{Haah2017,
abstract = {{\textless}p{\textgreater} We present an infinite family of protocols to distill magic states for {\textless}math{\textgreater} {\textless}mi{\textgreater}T{\textless}/mi{\textgreater} {\textless}/math{\textgreater} -gates that has a low space overhead and uses an asymptotic number of input magic states to achieve a given target error that is conjectured to be optimal. The space overhead, defined as the ratio between the physical qubits to the number of output magic states, is asymptotically constant, while both the number of input magic states used per output state and the {\textless}math{\textgreater} {\textless}mi{\textgreater}T{\textless}/mi{\textgreater} {\textless}/math{\textgreater} -gate depth of the circuit scale linearly in the logarithm of the target error {\textless}math{\textgreater} {\textless}mi{\textgreater}$\delta${\textless}/mi{\textgreater} {\textless}/math{\textgreater} (up to {\textless}math{\textgreater} {\textless}mi{\textgreater}log{\textless}/mi{\textgreater} {\textless}mo{\textgreater}⁡{\textless}/mo{\textgreater} {\textless}mi{\textgreater}log{\textless}/mi{\textgreater} {\textless}mo{\textgreater}⁡{\textless}/mo{\textgreater} {\textless}mn{\textgreater}1{\textless}/mn{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mo{\textgreater}/{\textless}/mo{\textgreater} {\textless}/mrow{\textgreater} {\textless}mi{\textgreater}$\delta${\textless}/mi{\textgreater} {\textless}/math{\textgreater} ). Unlike other distillation protocols, this protocol achieves this performance without concatenation and the input magic states are injected at various steps in the circuit rather than all at the start of the circuit. The protocol can be modified to distill magic states for other gates at the third level of the Clifford hierarchy, with the same asymptotic performance. The protocol relies on the construction of weakly self-dual CSS codes with many logical qubits and large distance, allowing us to implement control-SWAPs on multiple qubits. We call this code the "inner code". The control-SWAPs are then used to measure properties of the magic state and detect errors, using another code that we call the "outer code". Alternatively, we use weakly-self dual CSS codes which implement controlled Hadamards for the inner code, reducing circuit depth. We present several specific small examples of this protocol. {\textless}/p{\textgreater}},
archivePrefix = {arXiv},
arxivId = {1703.07847},
author = {Haah, Jeongwan and Hastings, Matthew B. and Poulin, D. and Wecker, D.},
doi = {10.22331/q-2017-10-03-31},
eprint = {1703.07847},
issn = {2521-327X},
journal = {Quantum},
month = {oct},
pages = {31},
publisher = {Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften},
title = {{Magic state distillation with low space overhead and optimal asymptotic input count}},
url = {https://quantum-journal.org/papers/q-2017-10-03-31/ http://arxiv.org/abs/1703.07847 http://dx.doi.org/10.22331/q-2017-10-03-31},
volume = {1},
year = {2017}
}
@article{Gawron2010,
abstract = {Numerical range of a Hermitian operator X is defined as the set of all possible expectation values of this observable among a normalized quantum state. We analyze a modification of this definition in which the expectation value is taken among a certain subset of the set of all quantum states. One considers, for instance, the set of real states, the set of product states, separable states, or the set of maximally entangled states. We show exemplary applications of these algebraic tools in the theory of quantum information: analysis of k-positive maps and entanglement witnesses, as well as study of the minimal output entropy of a quantum channel. Product numerical range of a unitary operator is used to solve the problem of local distinguishability of a family of two unitary gates.},
author = {Gawron, Piotr and Pucha{\l}a, Zbigniew and Miszczak, Jaros{\l}aw Adam and Skowronek, {\L}ukasz and {\.{Z}}yczkowski, Karol},
doi = {10.1063/1.3496901},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gawron et al. - 2010 - Restricted numerical range A versatile tool in the theory of quantum information.pdf:pdf},
issn = {0022-2488},
journal = {J. Math. Phys.},
keywords = {Hermitian matrices,entropy,quantum entanglement,quantum gates},
month = {oct},
number = {10},
pages = {102204},
publisher = {American Institute of Physics},
title = {{Restricted numerical range: A versatile tool in the theory of quantum information}},
url = {http://aip.scitation.org/doi/10.1063/1.3496901},
volume = {51},
year = {2010}
}
@article{Batle2006,
author = {Batle, J. and Casas, M. and Plastino, A. and Plastino, A. R.},
doi = {10.1103/PhysRevA.73.049904},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Batle et al. - 2006 - Erratum Connection between entanglement and the speed of quantum evolution Phys. Rev. A b72b , 032337 (2005).pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {apr},
number = {4},
pages = {049904},
publisher = {American Physical Society},
title = {{Erratum: Connection between entanglement and the speed of quantum evolution [Phys. Rev. A {\textless}b{\textgreater}72{\textless}/b{\textgreater} , 032337 (2005)]}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.73.049904},
volume = {73},
year = {2006}
}
@article{Bechmann-Pasquinucci2000,
author = {Bechmann-Pasquinucci, H. and Tittel, W.},
doi = {10.1103/PhysRevA.61.062308},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bechmann-Pasquinucci, Tittel - 2000 - Quantum cryptography using larger alphabets.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
number = {6},
pages = {062308},
publisher = {American Physical Society},
title = {{Quantum cryptography using larger alphabets}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.61.062308},
volume = {61},
year = {2000}
}
@article{Reich2013,
abstract = {We derive an algebraic framework which identifies the minimal information required to assess how well a quantum device implements a desired quantum operation. Our approach is based on characterizing only the unitary part of an open system's evolution. We show that a reduced set of input states is sufficient to estimate the average fidelity of a quantum gate, avoiding a sampling over the full Liouville space. Surprisingly, the minimal set consists of only two input states, independent of the Hilbert space dimension. The minimal set is, however, impractical for device characterization since one of the states is a totally mixed thermal state and extracting bounds for the average fidelity is impossible. We therefore present two further reduced sets of input states that allow, respectively, for numerical and analytical bounds on the average fidelity.},
archivePrefix = {arXiv},
arxivId = {1305.3222},
author = {Reich, Daniel M and Gualdi, Giulia and Koch, Christiane P},
doi = {10.1103/PhysRevA.88.042309},
eprint = {1305.3222},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Reich, Gualdi, Koch - 2013 - Minimum number of input states required for quantum gate characterization.pdf:pdf},
issn = {10502947},
journal = {Phys. Rev. A - At. Mol. Opt. Phys.},
number = {4},
title = {{Minimum number of input states required for quantum gate characterization}},
url = {https://journals.aps.org/pra/pdf/10.1103/PhysRevA.88.042309},
volume = {88},
year = {2013}
}
@article{Rodriguez-Rosario2011,
author = {Rodr{\'{i}}guez-Rosario, C{\'{e}}sar A. and Kimura, Gen and Imai, Hideki and Aspuru-Guzik, Al{\'{a}}n},
doi = {10.1103/PhysRevLett.106.050403},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Rodr{\'{i}}guez-Rosario et al. - 2011 - Sufficient and Necessary Condition for Zero Quantum Entropy Rates under any Coupling to the Environme.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {5},
pages = {050403},
publisher = {American Physical Society},
title = {{Sufficient and Necessary Condition for Zero Quantum Entropy Rates under any Coupling to the Environment}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.050403},
volume = {106},
year = {2011}
}
@article{Valenti2015,
author = {Valenti, D. and Magazz{\`{u}}, L. and Caldara, P. and Spagnolo, B.},
doi = {10.1103/PhysRevB.91.235412},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Valenti et al. - 2015 - Stabilization of quantum metastable states by dissipation.pdf:pdf},
issn = {1098-0121},
journal = {Phys. Rev. B},
month = {jun},
number = {23},
pages = {235412},
publisher = {American Physical Society},
title = {{Stabilization of quantum metastable states by dissipation}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.91.235412},
volume = {91},
year = {2015}
}
@article{Ashhab2012,
abstract = {We use analytical and numerical calculations in order to obtain speed limits for various unitary quantum operations in multi-qubit systems. The operations that we consider include single-, two- and three-qubit gates, as well as quantum state transfer in a chain of qubits. We find in particular that simple methods for implementing two-qubit gates generally provide the fastest possible implementations of these gates. We also find that the three-qubit Toffoli gate time varies greatly depending on the system's geometry, taking only slightly longer than a two-qubit CNOT gate for a triangle geometry. The speed limit for quantum state transfer across a qubit chain is set by the maximum spin wave speed in the chain.},
author = {Ashhab, S and {De Groot}, P C and Nori, Franco},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ashhab, De Groot, Nori - 2012 - Speed limits for quantum gates in multiqubit systems.pdf:pdf},
journal = {Phys. Rev. A},
number = {5},
title = {{Speed limits for quantum gates in multiqubit systems}},
url = {https://doi.org/10.1103/PhysRevA.85.052327},
volume = {85},
year = {2012}
}
@article{Toth2013,
author = {T{\'{o}}th, G{\'{e}}za and Petz, D{\'{e}}nes},
doi = {10.1103/PhysRevA.87.032324},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {mar},
number = {3},
pages = {032324},
publisher = {American Physical Society},
title = {{Extremal properties of the variance and the quantum Fisher information}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.87.032324},
volume = {87},
year = {2013}
}
@article{Andrews2007,
author = {Andrews, Mark},
doi = {10.1103/PhysRevA.75.062112},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Andrews - 2007 - Bounds to unitary evolution.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jun},
number = {6},
pages = {062112},
publisher = {American Physical Society},
title = {{Bounds to unitary evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.75.062112},
volume = {75},
year = {2007}
}
@article{Fleming1973,
author = {Fleming, G. N.},
doi = {10.1007/BF02819419},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Fleming - 1973 - A unitarity bound on the evolution of nonstationary states.pdf:pdf},
issn = {0369-3546},
journal = {Nuovo Cim. A},
month = {jul},
number = {2},
pages = {232--240},
publisher = {Societ{\`{a}} Italiana di Fisica},
title = {{A unitarity bound on the evolution of nonstationary states}},
url = {http://link.springer.com/10.1007/BF02819419},
volume = {16},
year = {1973}
}
@article{Kimura2003,
abstract = {We determine the set of the Bloch vectors for N-level systems, generalizing the familiar Bloch ball in 2-level systems. An origin of the structural difference from the Bloch ball in 2-level systems is clarified.},
author = {Kimura, Gen},
doi = {10.1016/S0375-9601(03)00941-1},
issn = {0375-9601},
journal = {Phys. Lett. A},
month = {aug},
number = {5-6},
pages = {339--349},
publisher = {North-Holland},
title = {{The Bloch vector for N-level systems}},
url = {https://www.sciencedirect.com/science/article/pii/S0375960103009411 https://www-sciencedirect-com.ezproxy.lib.monash.edu.au/science/article/pii/S0375960103009411},
volume = {314},
year = {2003}
}
@article{Piani2012,
author = {Piani, M.},
doi = {10.1103/PhysRevA.86.034101},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {034101},
publisher = {American Physical Society},
title = {{Problem with geometric discord}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.86.034101},
volume = {86},
year = {2012}
}
@article{Lendi1998a,
author = {Lendi, K. and Farhadmotamed, F. and van Wonderen, A. J.},
doi = {10.1023/A:1023004929346},
file = {::},
issn = {00224715},
journal = {J. Stat. Phys.},
number = {5/6},
pages = {1115--1135},
publisher = {Kluwer Academic Publishers-Plenum Publishers},
title = {{Regularization of Quantum Relative Entropy in Finite Dimensions and Application to Entropy Production}},
url = {http://link.springer.com/10.1023/A:1023004929346},
volume = {92},
year = {1998}
}
@article{Jennewein2000,
author = {Jennewein, Thomas and Simon, Christoph and Weihs, Gregor and Weinfurter, Harald and Zeilinger, Anton},
doi = {10.1103/PhysRevLett.84.4729},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Jennewein et al. - 2000 - Quantum Cryptography with Entangled Photons.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
number = {20},
pages = {4729--4732},
publisher = {American Physical Society},
title = {{Quantum Cryptography with Entangled Photons}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.84.4729},
volume = {84},
year = {2000}
}
@article{Fruchtman2016,
author = {Fruchtman, Amir and G{\'{o}}mez-Bombarelli, Rafael and Lovett, Brendon W. and Gauger, Erik M.},
doi = {10.1103/PhysRevLett.117.203603},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {nov},
number = {20},
pages = {203603},
publisher = {American Physical Society},
title = {{Photocell Optimization Using Dark State Protection}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.203603},
volume = {117},
year = {2016}
}
@article{Santos2016,
author = {Santos, Alan C. and Silva, Raphael D. and Sarandy, Marcelo S.},
doi = {10.1103/PhysRevA.93.012311},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {jan},
number = {1},
pages = {012311},
publisher = {American Physical Society},
title = {{Shortcut to adiabatic gate teleportation}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.93.012311},
volume = {93},
year = {2016}
}
@article{Caneva2009,
abstract = {Optimal control theory is a promising candidate for a drastic improvement of the performance of quantum information tasks. We explore its ultimate limit in paradigmatic cases, and demonstrate that it coincides with the maximum speed limit allowed by quantum evolution.},
author = {Caneva, T. and Murphy, M. and Calarco, T. and Fazio, R. and Montangero, S. and Giovannetti, V. and Santoro, G. E.},
doi = {10.1103/PhysRevLett.103.240501},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Caneva et al. - 2009 - Optimal Control at the Quantum Speed Limit(2).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Caneva et al. - 2009 - Optimal Control at the Quantum Speed Limit(4).pdf:pdf},
isbn = {0031-9007},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {24},
pages = {240501},
pmid = {20366188},
publisher = {American Physical Society},
title = {{Optimal Control at the Quantum Speed Limit}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.240501 https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.103.240501},
volume = {103},
year = {2009}
}
@article{Amatriain2009,
abstract = {{\textless}p{\textgreater}The AlloSphere is a spherical space in which immersive, virtual environments allow users to explore large-scale data sets through multimodal, interactive media.{\textless}/p{\textgreater}},
author = {Amatriain, Xavier and Kuchera-Morin, JoAnn and Hollerer, Tobias and Pope, Stephen Travis},
doi = {10.1109/MMUL.2009.35},
issn = {1070-986X},
journal = {IEEE Multimed.},
keywords = {3D audio,Immersive environments,human–computer interaction,scientific visualization,spherical displays,stereographic displays},
month = {apr},
number = {2},
pages = {64--75},
publisher = {IEEE Computer Society},
title = {{The AlloSphere: Immersive Multimedia for Scientific Discovery and Artistic Exploration}},
url = {http://ieeexplore.ieee.org/document/5167290/},
volume = {16},
year = {2009}
}
@article{Fubini1904,
author = {Fubini, Guido},
journal = {Atti Istit. Veneto},
pages = {502--513},
title = {{Sulle metriche definite da una forma Hermitiana}},
volume = {63},
year = {1904}
}
@article{Schafer2018,
abstract = {Fast and high-fidelity two-qubit logic gates are demonstrated by using amplitude-shaped laser pulses to ensure that the gate operation is insensitive to the optical phase of the pulses.},
author = {Sch{\"{a}}fer, V. M. and Ballance, C. J. and Thirumalai, K. and Stephenson, L. J. and Ballance, T. G. and Steane, A. M. and Lucas, D. M.},
doi = {10.1038/nature25737},
issn = {0028-0836},
journal = {Nature},
keywords = {Atomic and molecular interactions with photons,Quantum information,Qubits},
month = {feb},
number = {7694},
pages = {75--78},
publisher = {Nature Publishing Group},
title = {{Fast quantum logic gates with trapped-ion qubits}},
url = {http://www.nature.com/doifinder/10.1038/nature25737},
volume = {555},
year = {2018}
}
@article{Figueroa-Romero2018,
abstract = {It is common, when dealing with quantum processes involving a subsystem of a much larger composite closed system, to treat them as effectively memory-less (Markovian). While open systems theory tells us that non-Markovian processes should be the norm, the ubiquity of Markovian processes is undeniable. Here, without resorting to the Born-Markov assumption of weak coupling or making any approximations, we formally prove that typical processes are exponentially close to Markovian ones when the subsystem is sufficiently small compared to the remainder of the composite. We also show that, for a fixed global system size, it may not be possible to neglect non-Markovian effects when the process is allowed to continue for long enough. However, detecting non-Markovianity for such processes would usually require non-trivial entangling resources. Our results have foundational importance, as they give birth to Markov processes from composite closed dynamics.},
archivePrefix = {arXiv},
arxivId = {1802.10344},
author = {Figueroa-Romero, Pedro and Modi, Kavan and Pollock, Felix A.},
eprint = {1802.10344},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Figueroa-Romero, Modi, Pollock - 2018 - Almost Markovian processes from closed dynamics.pdf:pdf},
month = {feb},
title = {{Almost Markovian processes from closed dynamics}},
url = {http://arxiv.org/abs/1802.10344},
year = {2018}
}
@article{Dillenschneider2009,
author = {Dillenschneider, R. and Lutz, E. and {Nielsen M. A.}, Chuang I. L. and {Bennett C. H.}, DiVincenzo D. P., Fuchs C. A., Mor T., Rains E., Shor P. W., Smolin J. A. and Wootters W. K. and H., Ollivier H. and Zurek W. and {Horodecki M.}, Horodecki K., Horodecki P., Horodecki R., Oppenheim J., Sen(De) A. and Sen U. and {Datta A.}, Shaji A. and Caves C. M. and {Lanyon B. P.}, Barbieri M., Almeida M. P. and White A. G. and {Oppenheim J.}, Horodecki M., Horodecki P. and Horodecki R. and H., Zurek W. and {Horodecki M.}, Horodecki P., Horodecki R., Oppenheim J., Sen(De) A., Sen U. and Synak-Radtke B. and {Alicki R.}, Horedecki M., Horodecki P. and Horodecki R. and {Scully M. O.}, Zubairy M. S., Agarwal G. S. and Walther H. and A., Nielsen M. and {Arnesen M. C.}, Bose S. and Vedral V. and F., Kamta G. L. and Starace A. and {Amico L.}, Fazio R., Osterloh A. and Vedral V. and {Ghosh S.}, Rosenbaum T. F., Aeppli G. and Coppersmith S. N. and E., V{\'{e}}rtesi T. and Bene and {Rappoport T. G.}, Ghivelder L., Fernandes J. C., Guimar{\~{a}}es R. B. and Continentin M. A. and C., Zheng S. B. and Guo G. and {Osnaghi S.}, Bertet P., Auffeves A., Maioli P., Brune M., Raimond J. M. and Haroche S. and X., Wang and P., Schleich W. and {Cohen-Tannoudji C.}, Dupont-Roc J., Grynberg G. and B., Callen H. and V., Henderson L. and Vedral and {Hamieh S.}, Kobes R. and Zaraket H. and {B{\"{o}}hm H. R.}, Gigan S., Langer G., Hertzberg J. B., Blaser F., B{\"{a}}uerle D., Schwab K. C., Zeilinger A. and Aspelmeyer M.},
doi = {10.1209/0295-5075/88/50003},
issn = {0295-5075},
journal = {EPL (Europhysics Lett.},
month = {dec},
number = {5},
pages = {50003},
publisher = {IOP Publishing},
title = {{Energetics of quantum correlations}},
url = {http://stacks.iop.org/0295-5075/88/i=5/a=50003?key=crossref.0f74780de28c56609d21b31aa4af9056},
volume = {88},
year = {2009}
}
@article{Astafiev2004,
author = {Astafiev, O. and Pashkin, Yu. and Nakamura, Y. and Yamamoto, T. and Tsai, J.},
doi = {10.1103/PhysRevLett.93.267007},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Astafiev et al. - 2004 - Quantum Noise in the Josephson Charge Qubit.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {26},
pages = {267007},
publisher = {American Physical Society},
title = {{Quantum Noise in the Josephson Charge Qubit}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.93.267007},
volume = {93},
year = {2004}
}
@article{Brouzos2015,
abstract = {We extend the concept of quantum speed limit – the minimal time needed to perform a driven evolution – to complex interacting many-body systems. We investigate a prototypical many-body system, a bosonic Josephson junction, at increasing levels of complexity: (a) within the two-mode approximation corresponding to a nonlinear two-level system, (b) at the mean-field level by solving the nonlinear Gross-Pitaevskii equation in a double well potential, and (c) at an exact many-body level by solving the time-dependent many-body Schr{\"{o}}dinger equation. We propose a control protocol to transfer atoms from the ground state of a well to the ground state of the neighbouring well. Furthermore, we show that the detrimental effects of the inter-particle repulsion can be eliminated by means of a compensating control pulse, yielding, quite surprisingly, an enhancement of the transfer speed because of the particle interaction – in contrast to the self-trapping scenario. Finally, we perform numerical optimisations of both the nonlinear and the (exact) many-body quantum dynamics in order to further enhance the transfer efficiency close to the quantum speed limit. PACS numbers: 02.30.Yy, 03.75.Kk, 03.75.Lm, 05.60.Gg},
author = {Brouzos, Ioannis and Streltsov, Alexej I and Negretti, Antonio and Said, Ressa S and Caneva, Tommaso and Montangero, Simone and Calarco, Tommaso},
doi = {10.1103/PhysRevA.92.062110},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Brouzos et al. - 2015 - Quantum Speed Limit and Optimal Control of Many-Boson Dynamics.pdf:pdf},
journal = {Phys. Rev. A},
pages = {062110},
title = {{Quantum Speed Limit and Optimal Control of Many-Boson Dynamics}},
volume = {92},
year = {2015}
}
@article{Zhou2016,
abstract = {We consider the quantum measurements on a finite quantum system in coherence-vector representation. In this representation, all the density operators of an N-level (N 2) quantum system constitute a convex set M (N) embedded in an (N 2 − 1)-dimensional Euclidean space R N 2 −1 , and we find that an orthogonal measurement is an (N − 1)-dimensional projector operator on R N 2 −1 . The states unchanged by an orthogonal measurement form an (N − 1)-dimensional simplex, and in the case when N is prime or power of prime, the space of the density operator is a direct sum of (N + 1) such simplices. The mathematical description of quantum measurement is plain in this representation, and this may have further applications in quantum information processing. quantum measurement, coherence-vector representation, geometry PACS number(s): 03.65.Ca, 03.65.Ta, 03.65.-w Citation: T. Zhou, Quantum measurement in coherence-vector representation, Sci.},
author = {Zhou, Tao},
doi = {10.1007/s11433-016-5789-5},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zhou - 2016 - Quantum measurement in coherence-vector representation.pdf:pdf},
journal = {Artic. . Sci. CHINA Physics, Mech. Astron. China-Phys. Mech. Astron},
number = {59},
pages = {640301--640301},
title = {{Quantum measurement in coherence-vector representation}},
url = {https://link-springer-com.ezproxy.lib.monash.edu.au/content/pdf/10.1007{\%}2Fs11433-016-5789-5.pdf},
volume = {59},
year = {2016}
}
@article{Wang2013,
author = {Wang, Xiaoting and Vinjanampathy, Sai and Strauch, Frederick W. and Jacobs, Kurt},
doi = {10.1103/PhysRevLett.110.157207},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wang et al. - 2013 - Absolute Dynamical Limit to Cooling Weakly Coupled Quantum Systems.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {apr},
number = {15},
pages = {157207},
publisher = {American Physical Society},
title = {{Absolute Dynamical Limit to Cooling Weakly Coupled Quantum Systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.157207},
volume = {110},
year = {2013}
}
@article{Braunstein1994,
author = {Braunstein, Samuel L. and Caves, Carlton M.},
doi = {10.1103/PhysRevLett.72.3439},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Braunstein, Caves - 1994 - Statistical distance and the geometry of quantum states.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {may},
number = {22},
pages = {3439--3443},
publisher = {American Physical Society},
title = {{Statistical distance and the geometry of quantum states}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.3439},
volume = {72},
year = {1994}
}
@article{Wigley2016,
abstract = {Fast machine-learning online optimization of ultra-cold-atom experiments},
author = {Wigley, P. B. and Everitt, P. J. and van den Hengel, A. and Bastian, J. W. and Sooriyabandara, M. A. and McDonald, G. D. and Hardman, K. S. and Quinlivan, C. D. and Manju, P. and Kuhn, C. C. N. and Petersen, I. R. and Luiten, A. N. and Hope, J. J. and Robins, N. P. and Hush, M. R.},
doi = {10.1038/srep25890},
file = {::},
issn = {2045-2322},
journal = {Sci. Rep.},
keywords = {Computational science,Matter waves and particle beams},
month = {sep},
number = {1},
pages = {25890},
publisher = {Nature Publishing Group},
title = {{Fast machine-learning online optimization of ultra-cold-atom experiments}},
url = {http://www.nature.com/articles/srep25890},
volume = {6},
year = {2016}
}
@article{Russell2017,
abstract = {We study the maximum speed of quantum computation and how it is affected by limitations on physical resources. We show how the resulting concepts generalize to a broader class of physical models of computation within dynamical systems and introduce a specific algebraic structure representing these speed limits. We derive a family of quantum speed limit results in resource-constrained quantum systems with pure states and a finite dimensional state space, by using a geometric method based on right invariant action functionals on SU(N). We show that when the action functional is bi-invariant, the minimum time for implementing any quantum gate using a potentially time-dependent Hamiltonian is equal to the minimum time when using a constant Hamiltonian, thus constant Hamiltonians are time optimal for these constraints. We give an explicit formula for the time in these cases, in terms of the resource constraint. We show how our method produces a rich family of speed limit results, of which the generalized Margo...},
author = {Russell, Benjamin and Stepney, Susan},
doi = {10.1142/S0129054117500204},
issn = {0129-0541},
journal = {Int. J. Found. Comput. Sci.},
keywords = {Quantum speed limit,quantum computation},
month = {jun},
number = {04},
pages = {321--333},
publisher = { World Scientific Publishing Company },
title = {{The Geometry of Speed Limiting Resources in Physical Models of Computation}},
url = {http://www.worldscientific.com/doi/abs/10.1142/S0129054117500204},
volume = {28},
year = {2017}
}
@article{Uzdin2015,
abstract = {Quantum heat engines (QHE) are thermal machines where the working substance is a quantum object. In the extreme case, the working medium can be a single particle or a few-level quantum system. The study of QHE has shown a remarkable similarity with macroscopic thermodynamical results, thus raising the issue of what is quantum in quantum thermodynamics. Our main result is the thermodynamical equivalence of all engine types in the quantum regime of small action with respect to Planck's constant. They have the same power, the same heat, and the same efficiency, and they even have the same relaxation rates and relaxation modes. Furthermore, it is shown that QHE have quantum-thermodynamic signature; i.e., thermodynamic measurements can confirm the presence of quantum effects in the device. We identify generic coherent and stochastic work extraction mechanisms and show that coherence enables power outputs that greatly exceed the power of stochastic (dephased) engines.},
author = {Uzdin, Raam and Levy, Amikam and Kosloff, Ronnie},
doi = {10.1103/PhysRevX.5.031044},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uzdin, Levy, Kosloff - Unknown - Equivalence of Quantum Heat Machines, and Quantum-Thermodynamic Signatures.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uzdin, Levy, Kosloff - 2015 - Equivalence of Quantum Heat Machines, and Quantum-Thermodynamic Signatures.pdf:pdf},
issn = {2160-3308},
journal = {Phys. Rev. X},
keywords = {Quantum Physics,Subject Areas},
month = {sep},
number = {3},
pages = {031044},
publisher = {American Physical Society},
title = {{Equivalence of Quantum Heat Machines, and Quantum-Thermodynamic Signatures}},
url = {http://link.aps.org/doi/10.1103/PhysRevX.5.031044},
volume = {5},
year = {2015}
}
@article{Hamma2012,
abstract = {Most states in the Hilbert space are maximally entangled. This fact has proven useful to investigate—among other things—the foundations of statistical mechanics. Unfortunately, most states in the Hilbert space of a quantum many-body system are not physically accessible. We define physical ensembles of states acting on random factorized states by a circuit of length k of random and independent unitaries with local support. We study the typicality of entanglement by means of the purity of the reduced state. We find that for a time k=O(1), the typical purity obeys the area law. Thus, the upper bounds for area law are actually saturated, on average, with a variance that goes to zero for large systems. Similarly, we prove that by means of local evolution a subsystem of linear dimensions L is typically entangled with a volume law when the time scales with the size of the subsystem. Moreover, we show that for large values of k the reduced state becomes very close to the completely mixed state.},
archivePrefix = {arXiv},
arxivId = {1109.4391v1},
author = {Hamma, Alioscia and Santra, Siddhartha and Zanardi, Paolo},
doi = {10.1103/PhysRevLett.109.040502},
eprint = {1109.4391v1},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hamma, Santra, Zanardi - Unknown - Quantum entanglement in random physical states.pdf:pdf},
issn = {00319007},
journal = {Phys. Rev. Lett.},
number = {4},
pmid = {23006070},
title = {{Quantum entanglement in random physical states}},
volume = {109},
year = {2012}
}
@article{Campbell2017a,
abstract = {We assess precision thermometry for an arbitrary single quantum system. For a {\$}d{\$}-dimensional harmonic system we show that the gap sets a single temperature that can be optimally estimated. Furthermore, we establish a simple linear relationship between the gap and this temperature, and show that the precision exhibits a quadratic relationship. We extend our analysis to explore systems with arbitrary spectra, showing that exploiting anharmonicity and degeneracy can greatly enhance the precision of thermometry. Finally, we critically assess the dynamical features of two thermometry protocols for a two level system. By calculating the quantum speed limit we find that, despite the gap fixing a preferred temperature to probe, there is no evidence of this emerging in the dynamical features.},
archivePrefix = {arXiv},
arxivId = {1709.09672},
author = {Campbell, Steve and Genoni, Marco G. and Deffner, Sebastian},
eprint = {1709.09672},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campbell, Genoni, Deffner - 2017 - Precision thermometry and the quantum speed limit.pdf:pdf},
month = {sep},
title = {{Precision thermometry and the quantum speed limit}},
url = {http://arxiv.org/abs/1709.09672},
year = {2017}
}
@article{Bender2006,
abstract = {Given an initial quantum state |psi{\_}I{\textgreater} and a final quantum state |psi{\_}F{\textgreater} in a Hilbert space, there exist Hamiltonians H under which |psi{\_}I{\textgreater} evolves into |psi{\_}F{\textgreater}. Consider the following quantum brachistochrone problem: Subject to the constraint that the difference between the largest and smallest eigenvalues of H is held fixed, which H achieves this transformation in the least time tau? For Hermitian Hamiltonians tau has a nonzero lower bound. However, among non-Hermitian PT-symmetric Hamiltonians satisfying the same energy constraint, tau can be made arbitrarily small without violating the time-energy uncertainty principle. This is because for such Hamiltonians the path from |psi{\_}I{\textgreater} to |psi{\_}F{\textgreater} can be made short. The mechanism described here is similar to that in general relativity in which the distance between two space-time points can be made small if they are connected by a wormhole. This result may have applications in quantum computing.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0609032},
author = {Bender, Carl M. and Brody, Dorje C. and Jones, Hugh F. and Meister, Bernhard K.},
doi = {10.1103/PhysRevLett.98.040403},
eprint = {0609032},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bender et al. - 2006 - Faster than Hermitian Quantum Mechanics.pdf:pdf},
month = {sep},
primaryClass = {quant-ph},
title = {{Faster than Hermitian Quantum Mechanics}},
url = {http://arxiv.org/abs/quant-ph/0609032 http://dx.doi.org/10.1103/PhysRevLett.98.040403},
year = {2006}
}
@article{Zueco2009,
author = {Zueco, David and Reuther, Georg M. and Kohler, Sigmund and H{\"{a}}nggi, Peter},
doi = {10.1103/PhysRevA.80.033846},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {033846},
publisher = {American Physical Society},
title = {{Qubit-oscillator dynamics in the dispersive regime: Analytical theory beyond the rotating-wave approximation}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.80.033846},
volume = {80},
year = {2009}
}
@article{Baird1963,
abstract = {The explicit determination of the matrices of the generators of the unitary groups, SUn, is carried out and discussed in two alternative treatments: (a) by purely algebraic infinitesimal methods, and (b) by Young‐pattern techniques employing the Schwinger‐Bargmann boson operator methods. The implication of this result for a tableau calculus is discussed and a determination of the [$\lambda$] × [1] Wigner coefficient for all SUn is indicated.},
author = {Baird, G. E. and Biedenharn, L. C.},
doi = {10.1063/1.1703926},
issn = {0022-2488},
journal = {J. Math. Phys.},
month = {dec},
number = {12},
pages = {1449--1466},
publisher = {American Institute of Physics},
title = {{On the Representations of the Semisimple Lie Groups. II}},
url = {http://aip.scitation.org/doi/10.1063/1.1703926},
volume = {4},
year = {1963}
}
@article{Geng2016,
author = {Geng, Jianpei and Wu, Yang and Wang, Xiaoting and Xu, Kebiao and Shi, Fazhan and Xie, Yijin and Rong, Xing and Du, Jiangfeng},
doi = {10.1103/PhysRevLett.117.170501},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {oct},
number = {17},
pages = {170501},
publisher = {American Physical Society},
title = {{Experimental Time-Optimal Universal Control of Spin Qubits in Solids}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.170501},
volume = {117},
year = {2016}
}
@article{Deffner2017,
author = {Deffner, Sebastian and Campbell, Steve},
doi = {10.1088/1751-8121/aa86c6},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Deffner, Campbell - 2017 - Quantum speed limits from Heisenberg's uncertainty principle to optimal quantum control.pdf:pdf},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {nov},
number = {45},
pages = {453001},
publisher = {IOP Publishing},
title = {{Quantum speed limits: from Heisenberg's uncertainty principle to optimal quantum control}},
url = {http://stacks.iop.org/1751-8121/50/i=45/a=453001?key=crossref.cf4e172afa6c6ff525d7f6de2d64df0e},
volume = {50},
year = {2017}
}
@article{Chau2010,
author = {Chau, H. F.},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Chau - 2010 - Tight upper bound of the maximum speed of evolution of a quantum state.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jun},
number = {6},
pages = {062133},
title = {{Tight upper bound of the maximum speed of evolution of a quantum state}},
url = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.81.062133},
volume = {81},
year = {2010}
}
@article{Kaufmann2017,
author = {Kaufmann, H. and Ruster, T. and Schmiegelow, C. T. and Luda, M. A. and Kaushal, V. and Schulz, J. and von Lindenfels, D. and Schmidt-Kaler, F. and Poschinger, U. G.},
doi = {10.1103/PhysRevLett.119.150503},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kaufmann et al. - 2017 - Scalable Creation of Long-Lived Multipartite Entanglement.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {oct},
number = {15},
pages = {150503},
publisher = {American Physical Society},
title = {{Scalable Creation of Long-Lived Multipartite Entanglement}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.150503},
volume = {119},
year = {2017}
}
@inproceedings{JunSun,
author = {{Jun Sun} and {Bin Feng} and {Wenbo Xu}},
booktitle = {Proc. 2004 Congr. Evol. Comput. (IEEE Cat. No.04TH8753)},
doi = {10.1109/CEC.2004.1330875},
isbn = {0-7803-8515-2},
pages = {325--331},
publisher = {IEEE},
title = {{Particle swarm optimization with particles having quantum behavior}},
url = {http://ieeexplore.ieee.org/document/1330875/}
}
@article{Luo2004,
author = {Luo, Shunlong and Zhang, Qiang},
doi = {10.1103/PhysRevA.69.032106},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Luo, Zhang - 2004 - Informational distance on quantum-state space.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {mar},
number = {3},
pages = {032106},
publisher = {American Physical Society},
title = {{Informational distance on quantum-state space}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.69.032106},
volume = {69},
year = {2004}
}
@article{Vaidman1992,
author = {Vaidman, Lev},
doi = {10.1119/1.16940},
issn = {00029505},
journal = {Am. J. Phys.},
keywords = {DECOMPOSITION,ENERGY DEPENDENCE,HAMILTONIANS,HERMITIAN OPERATORS,HILBERT SPACE,QUANTUM OPERATORS,SCHROEDINGER EQUATION,TIME DEPENDENCE,TRANSITION PROBABILITIES,UNCERTAINTY PRINCIPLE,WAVE FUNCTIONS},
month = {feb},
number = {2},
pages = {182},
publisher = {American Association of Physics Teachers},
title = {{Minimum time for the evolution to an orthogonal quantum state}},
url = {http://aapt.scitation.org/doi/10.1119/1.16940},
volume = {60},
year = {1992}
}
@article{Tseng1999,
author = {Tseng, C. H. and Somaroo, S. and Sharf, Y. and Knill, E. and Laflamme, R. and Havel, T. F. and Cory, D. G.},
doi = {10.1103/PhysRevA.61.012302},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Tseng et al. - 1999 - Quantum simulation of a three-body-interaction Hamiltonian on an NMR quantum computer.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {dec},
number = {1},
pages = {012302},
publisher = {American Physical Society},
title = {{Quantum simulation of a three-body-interaction Hamiltonian on an NMR quantum computer}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.61.012302},
volume = {61},
year = {1999}
}
@article{Hegerfeldt1994,
author = {Hegerfeldt, Gerhard C.},
doi = {10.1103/PhysRevLett.72.596},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hegerfeldt - 1994 - Causality problems for Fermi's two-atom system.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jan},
number = {5},
pages = {596--599},
publisher = {American Physical Society},
title = {{Causality problems for Fermi's two-atom system}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.72.596},
volume = {72},
year = {1994}
}
@article{Epstein2017,
author = {Epstein, Jeffrey M. and Whaley, K. Birgitta},
doi = {10.1103/PhysRevA.95.042314},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Epstein, Whaley - 2017 - Quantum speed limits for quantum-information-processing tasks.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {apr},
number = {4},
pages = {042314},
publisher = {American Physical Society},
title = {{Quantum speed limits for quantum-information-processing tasks}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.95.042314},
volume = {95},
year = {2017}
}
@article{Luo2000,
author = {Luo, Shunlong},
doi = {10.1023/A:1011080128419},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Luo - 2000 - Quantum Fisher Information and Uncertainty Relations.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Luo - 2000 - Quantum Fisher Information and Uncertainty Relations(2).pdf:pdf},
issn = {03779017},
journal = {Lett. Math. Phys.},
number = {3},
pages = {243--251},
publisher = {Kluwer Academic Publishers},
title = {{Quantum Fisher Information and Uncertainty Relations}},
url = {http://link.springer.com/10.1023/A:1011080128419},
volume = {53},
year = {2000}
}
@article{Werschnik2007,
author = {Werschnik, J and Gross, E K U},
doi = {10.1088/0953-4075/40/18/R01},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Werschnik, Gross - 2007 - Quantum optimal control theory(2).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Werschnik, Gross - 2007 - Quantum optimal control theory.pdf:pdf},
issn = {0953-4075},
journal = {J. Phys. B At. Mol. Opt. Phys.},
month = {sep},
number = {18},
pages = {R175--R211},
publisher = {IOP Publishing},
title = {{Quantum optimal control theory}},
url = {http://stacks.iop.org/0953-4075/40/i=18/a=R01?key=crossref.60cbe8e8974d26529807617c70f0badd},
volume = {40},
year = {2007}
}
@techreport{Vitali1998,
abstract = {We show how an initially prepared quantum state of a radiation mode in a cavity can be preserved for a long time using a feedback scheme based on the injection of appropriately prepared atoms. We present a feedback scheme both for optical cavities, which can be continuously monitored by a photodetector, and for microwave cavities, which can be monitored only indirectly via the detection of atoms that have interacted with the cavity field. We also discuss the possibility of applying these methods for decoherence control in quantum information processing. S1050-29479811206-4},
author = {Vitali, D and Tombesi, P and Milburn, G J},
file = {::},
keywords = {0365Bz,4250Lc,PACS numbers},
title = {{Quantum-state protection in cavities}},
url = {https://journals.aps.org/pra/pdf/10.1103/PhysRevA.57.4930},
year = {1998}
}
@article{Volkoff2018,
abstract = {{\textless}p{\textgreater} For both unitary and open qubit dynamics, we compare asymmetry monotone-based bounds on the minimal time required for an initial qubit state to evolve to a final qubit state from which it is probabilistically distinguishable with fixed minimal error probability (i.e., the minimal error distinguishability time). For the case of unitary dynamics generated by a time-independent Hamiltonian, we derive a necessary and sufficient condition on two asymmetry monotones that guarantees that an arbitrary state of a two-level quantum system or a separable state of {\textless}math{\textgreater} {\textless}mi{\textgreater}N{\textless}/mi{\textgreater} {\textless}/math{\textgreater} two-level quantum systems will unitarily evolve to another state from which it can be distinguished with a fixed minimal error probability {\textless}math{\textgreater} {\textless}mi{\textgreater}$\delta${\textless}/mi{\textgreater} {\textless}mo{\textgreater}∈{\textless}/mo{\textgreater} {\textless}mo stretchy="false"{\textgreater}[{\textless}/mo{\textgreater} {\textless}mn{\textgreater}0{\textless}/mn{\textgreater} {\textless}mo{\textgreater},{\textless}/mo{\textgreater} {\textless}mn{\textgreater}1{\textless}/mn{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mo{\textgreater}/{\textless}/mo{\textgreater} {\textless}/mrow{\textgreater} {\textless}mn{\textgreater}2{\textless}/mn{\textgreater} {\textless}mo stretchy="false"{\textgreater}]{\textless}/mo{\textgreater} {\textless}/math{\textgreater} . This condition is used to order the set of qubit states based on their distinguishability time, and to derive an optimal release time for driven two-level systems such as those that occur, e.g., in the Landau-Zener problem. For the case of non-unitary dynamics, we compare three lower bounds to the distinguishability time, including a new type of lower bound which is formulated in terms of the asymmetry of the uniformly time-twirled initial system-plus-environment state with respect to the generator {\textless}math{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}H{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}S{\textless}/mi{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}/math{\textgreater} of the Stinespring isometry corresponding to the dynamics, specifically, in terms of {\textless}math{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}‖{\textless}/mo{\textgreater} {\textless}mo stretchy="false"{\textgreater}[{\textless}/mo{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}H{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}S{\textless}/mi{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mo{\textgreater},{\textless}/mo{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}$\rho${\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mtext{\textgreater}av{\textless}/mtext{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mo stretchy="false"{\textgreater}({\textless}/mo{\textgreater} {\textless}mi{\textgreater}$\tau${\textless}/mi{\textgreater} {\textless}mo stretchy="false"{\textgreater}){\textless}/mo{\textgreater} {\textless}mo stretchy="false"{\textgreater}]{\textless}/mo{\textgreater} {\textless}msub{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}‖{\textless}/mo{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mn{\textgreater}1{\textless}/mn{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}/math{\textgreater} , where {\textless}math{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}$\rho${\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mtext{\textgreater}av{\textless}/mtext{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mo stretchy="false"{\textgreater}({\textless}/mo{\textgreater} {\textless}mi{\textgreater}$\tau${\textless}/mi{\textgreater} {\textless}mo stretchy="false"{\textgreater}){\textless}/mo{\textgreater} {\textless}mo{\textgreater}:={\textless}/mo{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mfrac{\textgreater} {\textless}mn{\textgreater}1{\textless}/mn{\textgreater} {\textless}mi{\textgreater}$\tau${\textless}/mi{\textgreater} {\textless}/mfrac{\textgreater} {\textless}/mrow{\textgreater} {\textless}msubsup{\textgreater} {\textless}mo{\textgreater}∫{\textless}/mo{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mn{\textgreater}0{\textless}/mn{\textgreater} {\textless}/mrow{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}$\tau${\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msubsup{\textgreater} {\textless}mi{\textgreater}d{\textless}/mi{\textgreater} {\textless}mi{\textgreater}t{\textless}/mi{\textgreater} {\textless}mspace width="thinmathspace"/{\textgreater} {\textless}msup{\textgreater} {\textless}mi{\textgreater}e{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mo{\textgreater}−{\textless}/mo{\textgreater} {\textless}mi{\textgreater}i{\textless}/mi{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}H{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}S{\textless}/mi{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mi{\textgreater}t{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msup{\textgreater} {\textless}mi{\textgreater}$\rho${\textless}/mi{\textgreater} {\textless}mo{\textgreater}⊗{\textless}/mo{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}|{\textless}/mo{\textgreater} {\textless}mn{\textgreater}0{\textless}/mn{\textgreater} {\textless}msub{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}⟩{\textless}/mo{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}⟨{\textless}/mo{\textgreater} {\textless}mn{\textgreater}0{\textless}/mn{\textgreater} {\textless}msub{\textgreater} {\textless}mo fence="false" stretchy="false"{\textgreater}|{\textless}/mo{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}msup{\textgreater} {\textless}mi{\textgreater}e{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}i{\textless}/mi{\textgreater} {\textless}msub{\textgreater} {\textless}mi{\textgreater}H{\textless}/mi{\textgreater} {\textless}mrow class="MJX-TeXAtom-ORD"{\textgreater} {\textless}mi{\textgreater}S{\textless}/mi{\textgreater} {\textless}mi{\textgreater}E{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msub{\textgreater} {\textless}mi{\textgreater}t{\textless}/mi{\textgreater} {\textless}/mrow{\textgreater} {\textless}/msup{\textgreater} {\textless}/math{\textgreater} . {\textless}/p{\textgreater}},
author = {Volkoff, T.J. and Whaley, K.B.},
doi = {10.22331/q-2018-10-01-96},
issn = {2521-327X},
journal = {Quantum},
month = {oct},
pages = {96},
title = {{Distinguishability times and asymmetry monotone-based quantum speed limits in the Bloch ball}},
url = {https://quantum-journal.org/papers/q-2018-10-01-96/},
volume = {2},
year = {2018}
}
@article{Gittings2002,
abstract = {Quantum-mechanical entanglement is essential for certain forms of quantum communication, and occurs as a consequence of some operations in quantum computation. The ability to quantify this resource correctly has thus become of great interest to those working in the field of quantum information theory. In this paper, we show that all existing entanglement measures but one fail important tests of fitness when applied to n-particle m-site states of indistinguishable particles, where n, mgreater than or equal to2. The accepted method of measuring the entanglement of a bipartite system of distinguishable particles is to use the von Neumann entropy of the reduced density matrix of one half of the system. We show that expressing the full density matrix using a site-spin occupation number basis, and reducing with respect to that basis, gives an entanglement that meets all currently known fitness criteria for systems composed of either distinguishable or indistinguishable particles. We consider an output state from a previously published thought experiment, a state that is entangled in both spin and spatial degrees of freedom, and show that the site entropy measure gives the correct total entanglement. We also show how the spin-space entanglement transfer occurring within the apparatus can be understood in terms of the transfer of probability from single-occupancy to double-occupancy sectors of the density matrix.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0202051},
author = {Gittings and Fisher, Aj},
doi = {10.1103/PhysRevA.66.032305},
eprint = {0202051},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gittings, Fisher - 2002 - Describing mixed spin-space entanglement of pure states of indistinguishable particles using an occupation num.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gittings, Fisher - Unknown - Describing mixed spin-space entanglement of pure states of indistinguishable particles using an occupation-.pdf:pdf},
issn = {1050-2947},
keywords = {0365Ud,0367-a,0530-d,PACS numbers},
pages = {1--11},
primaryClass = {quant-ph},
title = {{Describing mixed spin-space entanglement of pure states of indistinguishable particles using an occupation-number basis}},
url = {http://discovery.ucl.ac.uk/66577/},
year = {2002}
}
@article{Brody2015a,
author = {Brody, Dorje C. and Meier, David M.},
doi = {10.1103/PhysRevLett.114.100502},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {10},
pages = {100502},
publisher = {American Physical Society},
title = {{Solution to the Quantum Zermelo Navigation Problem}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.100502},
volume = {114},
year = {2015}
}
@book{Ross1995,
abstract = {Classical sets and fuzzy sets Classical relations and fuzzy relations Membership functions Fuzzy rule-based systems Fuzzy-to-crisp conversions Fuzzy arithmetic, numbers, vectors, and extension principle Fuzzy nonlinear simulation Fuzzy classification Fuzzy pattern recognition Fuzzy control systems.},
author = {Ross, Timothy J.},
isbn = {0070539170},
pages = {600},
publisher = {McGraw-Hill},
title = {{Fuzzy logic with engineering applications}},
year = {1995}
}
@book{Vincent1997,
abstract = {The importance of advanced power sources has increased in line with the proliferation of battery-powered consumer products and in this new edition the authors provide an overview of all the principle battery types. Introduction -- Theoretical background -- Primary aqueous electrolyte cells -- Primary lithium cells -- Secondary lead-acid cells -- Secondary alkaline cells -- Rechargeable lithium cells -- High temperature cells -- Miscellaneous cells.},
author = {Vincent, Colin Angus. and Scrosati, Bruno.},
isbn = {0340662786},
pages = {351},
publisher = {Arnold},
title = {{Modern batteries : an introduction to electrochemical power sources}},
year = {1997}
}
@misc{supplemental,
title = {{See Supplemental Material at [link] for deteails on the derivation of our bound and its tightness.}}
}
@article{Rosenberg2016,
author = {Rosenberg, Gili and Vazifeh, Mohammad and Woods, Brad and Haber, Eldad},
doi = {10.1007/s10589-016-9844-y},
issn = {0926-6003},
journal = {Comput. Optim. Appl.},
month = {dec},
number = {3},
pages = {845--869},
publisher = {Springer US},
title = {{Building an iterative heuristic solver for a quantum annealer}},
url = {http://link.springer.com/10.1007/s10589-016-9844-y},
volume = {65},
year = {2016}
}
@article{Lenard1978,
author = {Lenard, A.},
doi = {10.1007/BF01011769},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Lenard - 1978 - Thermodynamical proof of the Gibbs formula for elementary quantum systems.pdf:pdf},
issn = {0022-4715},
journal = {J. Stat. Phys.},
month = {dec},
number = {6},
pages = {575--586},
publisher = {Kluwer Academic Publishers-Plenum Publishers},
title = {{Thermodynamical proof of the Gibbs formula for elementary quantum systems}},
url = {http://link.springer.com/10.1007/BF01011769},
volume = {19},
year = {1978}
}
@article{Mostafazadeh2007,
abstract = {A non-Hermitian operator with a real spectrum and a complete set of eigenvectors may serve as the Hamiltonian operator for a unitary quantum system provided that one makes an appropriate choice for the defining the inner product of physical Hilbert state. We study the consequences of such a choice for the representation of states in terms of projection operators and the geometry of the state space. This allows for a careful treatment of the quantum Brachistochrone problem and shows that it is indeed impossible to achieve faster unitary evolutions using PT-symmetric or other non-Hermitian Hamiltonians than those given by Hermitian Hamiltonians.},
author = {Mostafazadeh, Ali},
issn = {00319007},
journal = {Phys. Rev. Lett.},
pmid = {17930566},
title = {{Quantum brachistochrone problem and the geometry of the state space in Pseudo-Hermitian quantum mechanics}},
url = {https://doi.org/10.1103/PhysRevLett.99.130502},
volume = {99},
year = {2007}
}
@article{Modi2016,
archivePrefix = {arXiv},
arxivId = {1608.01443},
author = {Modi, Kavan and C{\'{e}}leri, Lucas C. and Thompson, Jayne and Gu, Mile},
eprint = {1608.01443},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Modi et al. - 2016 - Fragile states are better for quantum metrology.pdf:pdf},
month = {aug},
title = {{Fragile states are better for quantum metrology}},
url = {http://arxiv.org/abs/1608.01443},
year = {2016}
}
@article{Eberly1973,
author = {Eberly, Joseph H. and Singh, L. P.S.},
doi = {10.1103/PhysRevD.7.359},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Eberly, Singh - 1973 - Time Operators, Partial Stationarity, and the Energy-Time Uncertainty Relation.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Eberly, Singh - 1973 - Time Operators, Partial Stationarity, and the Energy-Time Uncertainty Relation(2).pdf:pdf},
issn = {05562821},
journal = {Phys. Rev. D},
month = {jan},
number = {2},
pages = {359--362},
publisher = {American Physical Society},
title = {{Time operators, partial stationarity, and the energy-time uncertainty relation}},
url = {https://link.aps.org/doi/10.1103/PhysRevD.7.359},
volume = {7},
year = {1973}
}
@article{Guryanova2018,
abstract = {We show that with finite resources it is impossible to perform a perfect projective measurement of a quantum system. We model the measurement as an interaction of the system with an N-particle pointer and provide tight analytic expressions for the energy cost of performing such a measurement. Under the assumption that the statistics of the system are perfectly reproduced by the pointer, this cost breaks down into two parts. First, the cost of preparing the pointer in a suitable state, and second, the cost of a global interaction between the system and pointer in order to correlate them. Our results show that, even under the assumption that the interaction can be controlled perfectly, achieving perfect correlation is infinitely expensive. We provide measurement protocols for achieving optimal correlation between a system and pointer given finite resources.},
archivePrefix = {arXiv},
arxivId = {1805.11899},
author = {Guryanova, Yelena and Friis, Nicolai and Huber, Marcus},
eprint = {1805.11899},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Guryanova, Friis, Huber - 2018 - Ideal Projective Measurements Have an Infinite Energy Cost.pdf:pdf},
month = {may},
title = {{Ideal Projective Measurements Have an Infinite Energy Cost}},
url = {http://arxiv.org/abs/1805.11899},
year = {2018}
}
@article{Mintert2005,
abstract = {We develop an original approach for the quantitative characterisation of the entanglement properties of, possibly mixed, bi- and multipartite quantum states of arbitrary finite dimension. Particular emphasis is given to the derivation of reliable estimates which allow for an efficient evaluation of a specific entanglement measure, concurrence, for further implementation in the monitoring of the time evolution of multipartite entanglement under incoherent environment coupling. The flexibility of the technical machinery established here is illustrated by its implementation for different, realistic experimental scenarios.},
author = {Mintert, Florian and Carvalho, Andr{\'{e}} R.R. and Ku{\'{s}}, Marek and Buchleitner, Andreas},
doi = {10.1016/j.physrep.2005.04.006},
issn = {03701573},
journal = {Phys. Rep.},
number = {4},
pages = {207--259},
title = {{Measures and dynamics of entangled states}},
volume = {415},
year = {2005}
}
@article{Vinjanampathy2016a,
abstract = {Quantum thermodynamics is an emerging research field aiming to extend standard thermodynamics and non-equilibrium statistical physics to ensembles of sizes well below the thermodynamic limit, in non-equilibrium situations and with the full inclusion of quantum effects. Fuelled by experimental advances and the potential of future nanoscale applications, this research effort is pursued by scientists with different backgrounds, including statistical physics, many-body theory, mesoscopic physics and quantum information theory, who bring various tools and methods to the field. A multitude of theoretical questions are being addressed ranging from issues of thermalisation of quantum systems and various definitions of ‘work' to the efficiency and power of quantum engines. This overview provides a perspective on a selection of these current trends accessible to postgraduate students and researchers alike.},
author = {Vinjanampathy, Sai and Anders, Janet},
doi = {10.1080/00107514.2016.1201896},
issn = {0010-7514},
journal = {Contemp. Phys.},
keywords = {(Quantum) information–thermodynamics link,(quantum) fluctuation theorems,quantum thermal machines,single shot thermodynamics,thermalisation of quantum systems},
month = {oct},
number = {4},
pages = {545--579},
publisher = {Taylor {\&} Francis},
title = {{Quantum thermodynamics}},
url = {https://www.tandfonline.com/doi/full/10.1080/00107514.2016.1201896},
volume = {57},
year = {2016}
}
@article{Vuglar2016,
abstract = {A systematic approach is given for engineering dissipative environments that steer quantum wavepackets along desired trajectories. The methodology is demonstrated with several illustrative examples: environment-assisted tunneling, trapping, effective mass assignment, and pseudo-relativistic behavior. Non-conservative stochastic forces do not inevitably lead to decoherence - we show that purity can be well-preserved. These findings highlight the flexibility offered by non-equilibrium open quantum dynamics.},
archivePrefix = {arXiv},
arxivId = {1611.02736},
author = {Vuglar, Shanon L. and Zhdanov, Dmitry V. and Cabrera, Renan and Seideman, Tamar and Jarzynski, Christopher and Bondar, Denys I.},
eprint = {1611.02736},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Vuglar et al. - 2016 - Non-conservative Forces via Quantum Reservoir Engineering.pdf:pdf},
month = {nov},
title = {{Non-conservative Forces via Quantum Reservoir Engineering}},
url = {http://arxiv.org/abs/1611.02736},
year = {2016}
}
@article{Sun2015,
abstract = {Quantum speed limits in open systems: Non-Markovian dynamics without rotating-wave approximation},
author = {Sun, Zhe and Liu, Jing and Ma, Jian and Wang, Xiaoguang},
doi = {10.1038/srep08444},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Sun et al. - 2015 - Quantum speed limits in open systems Non-Markovian dynamics without rotating-wave approximation.pdf:pdf},
issn = {2045-2322},
journal = {Sci. Rep.},
keywords = {Quantum information,Quantum mechanics},
month = {jul},
number = {1},
pages = {8444},
publisher = {Nature Publishing Group},
title = {{Quantum speed limits in open systems: Non-Markovian dynamics without rotating-wave approximation}},
url = {http://www.nature.com/articles/srep08444},
volume = {5},
year = {2015}
}
@article{Jager2014,
author = {J{\"{a}}ger, Georg and Reich, Daniel M. and Goerz, Michael H. and Koch, Christiane P. and Hohenester, Ulrich},
doi = {10.1103/PhysRevA.90.033628},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {033628},
publisher = {American Physical Society},
title = {{Optimal quantum control of Bose-Einstein condensates in magnetic microtraps: Comparison of gradient-ascent-pulse-engineering and Krotov optimization schemes}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.90.033628},
volume = {90},
year = {2014}
}
@article{Sorensen2016,
abstract = {The crowd sourcing and gamification of a problem in quantum computing are described; human players succeed in solving the problem where purely numerical optimization fails, providing insight into, and a starting point for, strategies for optimization.},
author = {S{\o}rensen, Jens Jakob W. H. and Pedersen, Mads Kock and Munch, Michael and Haikka, Pinja and Jensen, Jesper Halkj{\ae}r and Planke, Tilo and Andreasen, Morten Ginnerup and Gajdacz, Miroslav and M{\o}lmer, Klaus and Lieberoth, Andreas and Sherson, Jacob F.},
doi = {10.1038/nature17620},
file = {::},
issn = {0028-0836},
journal = {Nature},
keywords = {Computational science,Quantum information,Quantum mechanics},
month = {apr},
number = {7598},
pages = {210--213},
publisher = {Nature Publishing Group},
title = {{Exploring the quantum speed limit with computer games}},
url = {http://www.nature.com/articles/nature17620},
volume = {532},
year = {2016}
}
@incollection{Bennett1984,
address = {Berlin, Heidelberg},
author = {Bennett, Charles H. and Brassard, Gilles},
booktitle = {Adv. Cryptol.},
doi = {10.1007/3-540-39568-7_39},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bennett, Brassard - 1984 - An Update on Quantum Cryptography.pdf:pdf},
pages = {475--480},
publisher = {Springer Berlin Heidelberg},
title = {{An Update on Quantum Cryptography}},
url = {http://link.springer.com/10.1007/3-540-39568-7{\_}39},
year = {1984}
}
@article{Uhlmann1992b,
abstract = {Given the density operator ??{\{}variant{\}}1 as an initial value of a Hamiltonian motion that evolves in a time interval ??t to ??{\{}variant{\}}2. Then ??t ??E, ??E being the energy dispersion (or energy uncertainty) of the motion, can be estimated from below by comparing the length of the Hamiltonian curve with a geodesic joining the initial and the final density operator. The lengths are calculated in the Bures metric. ?? 1992.},
author = {Uhlmann, Armin},
doi = {10.1016/0375-9601(92)90555-Z},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uhlmann - 1992 - An energy dispersion estimate.pdf:pdf},
issn = {03759601},
journal = {Phys. Lett. A},
month = {jan},
number = {4},
pages = {329--331},
title = {{An energy dispersion estimate}},
url = {http://linkinghub.elsevier.com/retrieve/pii/037596019290555Z},
volume = {161},
year = {1992}
}
@article{Kane1998,
author = {Kane, B. E.},
doi = {10.1038/30156},
issn = {00280836},
journal = {Nature},
number = {6681},
pages = {133--137},
publisher = {Nature Publishing Group},
title = {{A silicon-based nuclear spin quantum computer}},
url = {http://www.nature.com/doifinder/10.1038/30156},
volume = {393},
year = {1998}
}
@article{Hovhannisyan2013,
author = {Hovhannisyan, Karen V. and Perarnau-Llobet, Mart{\'{i}} and Huber, Marcus and Ac{\'{i}}n, Antonio},
doi = {10.1103/PhysRevLett.111.240401},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hovhannisyan et al. - 2013 - Entanglement Generation is Not Necessary for Optimal Work Extraction.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {24},
pages = {240401},
publisher = {American Physical Society},
title = {{Entanglement Generation is Not Necessary for Optimal Work Extraction}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.240401},
volume = {111},
year = {2013}
}
@article{DePasquale2011,
abstract = {The local purity of large many-body quantum systems can be studied by following a statistical mechanical approach based on a random matrix model. Restricting the analysis to the case of global pure states, this method proved to be successful and a full characterization of the statistical properties of the local purity was obtained by computing the partition function of the problem. Here we generalize these techniques to the case of global mixed states. Since the computation of the partition function is far more challenging than in the pure case, we focus on the computation of the first moments of the local purity. Finally, we establish a connection with the theory of twirling maps in quantum channels.},
archivePrefix = {arXiv},
arxivId = {1106.5330},
author = {{De Pasquale}, A. and Facchi, P. and Giovannetti, V. and Parisi, G. and Pascazio, S. and Scardicchio, A.},
doi = {10.1088/1751-8113/45/1/015308},
eprint = {1106.5330},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/De Pasquale et al. - 2011 - Statistical distribution of the local purity in a large quantum system(2).pdf:pdf},
month = {jun},
title = {{Statistical distribution of the local purity in a large quantum system}},
url = {http://arxiv.org/abs/1106.5330 http://dx.doi.org/10.1088/1751-8113/45/1/015308},
year = {2011}
}
@article{Alipour2014,
author = {Alipour, S. and Mehboudi, M. and Rezakhani, A. T.},
doi = {10.1103/PhysRevLett.112.120405},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Alipour, Mehboudi, Rezakhani - 2014 - Quantum Metrology in Open Systems Dissipative Cram{\'{e}}r-Rao Bound.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {12},
pages = {120405},
publisher = {American Physical Society},
title = {{Quantum Metrology in Open Systems: Dissipative Cram{\'{e}}r-Rao Bound}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.120405},
volume = {112},
year = {2014}
}
@article{Carlini2008,
abstract = {We present a general framework for finding the time-optimal evolution and the optimal Hamiltonian for a quantum system with a given set of initial and final states. Our formulation is based on the variational principle and is analogous to that for the brachistochrone in classical mechanics. We reduce the problem to a formal equation for the Hamiltonian which depends on certain constraint functions specifying the range of available Hamiltonians. For some simple examples of the constraints, we explicitly find the optimal solutions.},
author = {Carlini, Alberto and Hosoya, Akio and Koike, Tatsuhiko and Okudaira, Yosuke},
issn = {10797114},
journal = {J. Phys. A Math. Theor.},
number = {4},
pmid = {16605975},
title = {{Time Optimal Quantum Evolution of Mixed States}},
url = {http://iopscience.iop.org/article/10.1088/1751-8113/41/4/045303/meta},
volume = {41},
year = {2008}
}
@article{Compton1923,
author = {Compton, Arthur H.},
doi = {10.1103/PhysRev.21.483},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Compton - 1923 - A Quantum Theory of the Scattering of X-rays by Light Elements.pdf:pdf},
issn = {0031-899X},
journal = {Phys. Rev.},
month = {may},
number = {5},
pages = {483--502},
publisher = {American Physical Society},
title = {{A Quantum Theory of the Scattering of X-rays by Light Elements}},
url = {https://link.aps.org/doi/10.1103/PhysRev.21.483},
volume = {21},
year = {1923}
}
@article{Allahverdyan2004,
author = {Allahverdyan, A. E and Balian, R and Nieuwenhuizen, Th. M},
doi = {10.1209/epl/i2004-10101-2},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Allahverdyan, Balian, Nieuwenhuizen - 2004 - Maximal work extraction from finite quantum systems.pdf:pdf},
issn = {0295-5075},
journal = {Europhys. Lett.},
month = {aug},
number = {4},
pages = {565--571},
publisher = {IOP Publishing},
title = {{Maximal work extraction from finite quantum systems}},
url = {http://stacks.iop.org/0295-5075/67/i=4/a=565?key=crossref.441ef4f799a8946a3f6264e775c381f6},
volume = {67},
year = {2004}
}
@article{Acin2009,
abstract = {Device-independent quantum key distribution (DIQKD) represents a relaxation of the security assumptions made in usual quantum key distribution (QKD). As in usual QKD, the security of DIQKD follows from the laws of quantum physics, but contrary to usual QKD, it does not rely on any assumptions about the internal working of the quantum devices used in the protocol. In this paper, we present in detail the security proof for a DIQKD protocol introduced in Ac{\'{i}}n et al (2008 Phys. Rev. Lett. 98 230501). This proof exploits the full structure of quantum theory (as opposed to other proofs that exploit only the no-signaling principle), but only holds against collective attacks, where the eavesdropper is assumed to act on the quantum systems of the honest parties independently and identically in each round of the protocol (although she can act coherently on her systems at any time). The security of any DIQKD protocol necessarily relies on the violation of a Bell inequality. We discuss the issue of loopholes in Bell experiments in this context.},
author = {Ac{\'{i}}n, Antonio and Brunner, Nicolas and Massar, Serge and Pironio, Stefano and Gisin, Nicolas and Scarani, Valerio},
doi = {10.1088/1367-2630/11/4/045021},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ac{\'{i}}n et al. - 2009 - Device-independent quantum key distribution secure against collective attacks.pdf:pdf},
journal = {New J. Phys. New J. Phys. New J. Phys.},
number = {11},
title = {{Device-independent quantum key distribution secure against collective attacks}},
url = {http://iopscience.iop.org/1367-2630/11/4/045021},
volume = {11},
year = {2009}
}
@article{Kupferman2008,
abstract = {Entanglement speeds up evolution of a pure bipartite spin state, in line with the time energy uncertainty. However if the state is mixed this is not necessarily the case. We provide a counter example and point to other factors affecting evolution in mixed states, including classical correlations and entropy.},
author = {Kupferman, Judy and Reznik, Benni},
doi = {10.1103/PhysRevA.78.042305},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kupferman, Reznik - 2008 - Entanglement and the speed of evolution in mixed states.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kupferman, Reznik - 2008 - Entanglement and the speed of evolution in mixed states(2).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kupferman, Reznik - Unknown - Entanglement and the speed of evolution in mixed states.pdf:pdf;::},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {oct},
number = {4},
pages = {042305},
publisher = {American Physical Society},
title = {{Entanglement and the speed of evolution in mixed states}},
url = {https://doi.org/10.1103/PhysRevA.78.042305 https://link.aps.org/doi/10.1103/PhysRevA.78.042305},
volume = {78},
year = {2008}
}
@article{Hu2018,
abstract = {It is known that high intensity fields are usually required to implement shortcuts to adiabaticity via transitionless quantum driving (TQD). Here, we show that this requirement can be relaxed by exploiting the gauge freedom of generalized TQD, which is expressed in terms of an arbitrary phase when mimicking the adiabatic evolution. We experimentally investigate the performance of generalized TQD in comparison to both traditional TQD and adiabatic dynamics. By using a Yb+171 trapped ion hyperfine qubit, we implement a Landau{\&}{\#}x2013;Zener adiabatic Hamiltonian and its (traditional and generalized) TQD counterparts. We show that the generalized theory provides energy-optimal Hamiltonians for TQD, with no additional fields required. In addition, the optimal TQD Hamiltonian for the Landau{\&}{\#}x2013;Zener model is investigated under dephasing. Even using less intense fields, optimal TQD exhibits fidelities that are more robust against a decohering environment, with performance superior to that provided by the adiabatic dynamics.},
author = {Hu, Chang-Kang and Cui, Jin-Ming and Santos, Alan C. and Huang, Yun-Feng and Sarandy, Marcelo S. and Li, Chuan-Feng and Guo, Guang-Can},
doi = {10.1364/OL.43.003136},
issn = {0146-9592},
journal = {Opt. Lett.},
keywords = {Bandpass filters,Frequency modulation,Laser cooling,Magnetic fields,Quantum information processing,Two level systems},
month = {jul},
number = {13},
pages = {3136},
publisher = {Optical Society of America},
title = {{Experimental implementation of generalized transitionless quantum driving}},
url = {https://www.osapublishing.org/abstract.cfm?URI=ol-43-13-3136},
volume = {43},
year = {2018}
}
@article{Wong2001,
author = {Wong, Alexander and Christensen, Nelson},
doi = {10.1103/PhysRevA.63.044301},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wong, Christensen - 2001 - Potential multiparticle entanglement measure.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {mar},
number = {4},
pages = {044301},
publisher = {American Physical Society},
title = {{Potential multiparticle entanglement measure}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.63.044301},
volume = {63},
year = {2001}
}
@article{Cedergren2017,
abstract = {The low-temperature states of bosonic condensates exhibit fundamental quantum effects at the macroscopic scale. The combined effects of interaction and disorder in these can have drastic consequences, leading to the Mott insulator and Bose-Anderson glass. The latter is thought to describe helium-4 in porous media, cold atoms in disordered optical potentials, disordered magnetic insulators, and thin superconducting films. The prototypical Bose-Hubbard model without disorder predicts a Beresinskii-Kosterlitz-Thouless quantum phase transition between superfluid and Mott insulator. Experimental implementation using arrays of Josephson junctions has been explored, however, the possibility of the insulating glass has not been considered. The ubiquity of such a phase in Josephson-junction arrays would have important implications for their proposed use as a fundamental current standard. Unlike the Mott insulator, the insulating glass is compressible, therefore AC synchronisation of charge may not be possible. We have measured critical voltages for a large number of simple chains of sub-micron Josephson junctions with significantly varying energy scales. We observe universal scaling of critical voltage with single-junction Bloch bandwidth. Our measurements reveal a localisation length exponent that steepens with Luttinger parameter, arising from precursor fluctuations as one approaches the Bose glass-superfluid quantum phase transition. This contrasts with the fixed exponent found for classical pinning of charge density waves, vortex lattices, and disordered spin systems, and is in excellent agreement with the quantum theory of one-dimensional disordered bosonic insulators. We thereby demonstrate a unique signature of the charged Bose glass in insulating Josephson-junction chains.},
archivePrefix = {arXiv},
arxivId = {1702.04386},
author = {Cedergren, Karin and Ackroyd, Roger and Kafanov, Sergey and Vogt, Nicolas and Shnirman, Alexander and Duty, Timothy},
eprint = {1702.04386},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Cedergren et al. - 2017 - Depinning of the charged Bose glass origin of the critical voltage in nanostructured Josephson-junction chains.pdf:pdf},
month = {feb},
title = {{Depinning of the charged Bose glass: origin of the critical voltage in nanostructured Josephson-junction chains}},
url = {http://arxiv.org/abs/1702.04386},
year = {2017}
}
@article{Pires2016,
author = {Pires, Diego Paiva and Cianciaruso, Marco and C{\'{e}}leri, Lucas C. and Adesso, Gerardo and Soares-Pinto, Diogo O.},
doi = {10.1103/PhysRevX.6.021031},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pires et al. - 2016 - Generalized Geometric Quantum Speed Limits.pdf:pdf},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {jun},
number = {2},
pages = {021031},
publisher = {American Physical Society},
title = {{Generalized Geometric Quantum Speed Limits}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.6.021031},
volume = {6},
year = {2016}
}
@article{Xu2016,
author = {Xu, Zhen-Yu and I, Mandelstam L and Tamm and B, Margolus N and Levitin L and L, Markov I and {Giovanetti V}, Lloyd S and Maccone L and {Chin A W}, Huelga S F and Plenio M B and E, Deffner S and Lutz and {del Campo A}, Goold J and Paternostro M and {Caneva T}, Murphy M, Calarco T, Fazio R, Montangero S, Giovannetti V and Santoro G E and C, Hegerfeldt G and Y, Anandan J and Aharonov and A, Uhlmann and L, Vaidman and J, Pfeifer P and Frohlich and {Giovannetti V}, Lloyd S and Maccone L and S, Luo and Z, Luo S and Zhang and {Batle J}, Casas M, Plastino A and Plastino A R and {Borras A}, Casas M, Plastino A R and Plastino A and T, Levitin L B and Toffoli and P, Jones P J and Kok and {Fu S-S}, Li N and Luo S and F, Frowis and E, Deffner S and Lutz and S, Russell B and Stepney and C, Hegerfeldt G and I, Villamizar D V and Duzzioni E and M, Braunstein S L and Caves C and J, Braunstein S L and Milburn G and {Taddei M M}, Escher B M, Davidovich L and de Matos Filho R L and {del Campo A}, Egusquiza I L, Plenio M B and Huelga S F and E, Deffner S and Lutz and {Cimmarusti A D}, Yan Z, Patterson B D, Corcos L P, Orozco L A and Deffner S and A, Marvian I and Lidar D and {Latune C L}, Escher B M, de Matos Filho R L and Davidovich L and {Xu Z-Y}, Luo S, Yang W L, Liu C and Zhu S and {Zhang Y-J}, Han W, Xia Y-J, Cao J-P and Fan H and {Liu C}, Xu Z-Y and Zhu S and {Wu S}, Zhang Y, Yu C and Song H and {Sun Z}, Liu J, Ma J and Wang X and {Pires D P}, Cianciaruso M, C{\'{e}}leri L C, Adesso G and Soares-Pinto D O and {Jing J}, Wu L-A and del Campo A and {Liu H-B}, Yang W L, An J-H and Xu Z-Y and {Wei Y-B}, Zou J, Wang Z-M, Shao B and Li H and K, Mondal D and Pati A and F, Breuer H-P and Petruccione and K, Bengtsson I and {\.{Z}}yczkowski and M, Fecko and D, Petz and E, Deza M M and Deza and J, Sakurai J J and Napolitano J and K, Wootters W and {Breuer H-P}, Laine E-M, Piilo J and Vacchini B and {Rivas {\'{A}}}, Huelga S F and Plenio M B and {Xu Z-Y}, Yang W L and Feng M and {Bellomo B}, Lo Franco R and Compagno G and {Madsen K H}, Ates S, Lund-Hansen T, L{\"{o}}ffler A, Reitzenstein S, Forchel A and Lodahl P and {Doherty M W}, Manson N B, Delaneyc P, Jelezko F, Wrachtrup J and Hollenberg L},
doi = {10.1088/1367-2630/18/7/073005},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Xu et al. - 2016 - Detecting quantum speedup in closed and open systems.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
month = {jul},
number = {7},
pages = {073005},
publisher = {IOP Publishing},
title = {{Detecting quantum speedup in closed and open systems}},
url = {http://stacks.iop.org/1367-2630/18/i=7/a=073005?key=crossref.7a1055ae43005f0d01b7a24adb0d5584},
volume = {18},
year = {2016}
}
@article{Deffnera,
abstract = {The quantum speed limit is a fundamental upper bound on the speed of quantum evolution. However, the actual mathematical expression of this fundamental limit depends on the choice of a measure of distinguishability of quantum states. We show that quantum speed limits are universally characterized by the Schatten-p-norm of the generator of quantum dynamics. Since computing Schatten-p-norms can be mathematically involved, we then develop an alternative approach in Wigner phase space. We find that the quantum speed limit in Wigner space is fully equivalent to expressions in density operator space, but that the new bound is significantly easier to compute. Our results are illustrated for the parametric harmonic oscillator and for quantum Brownian motion.},
author = {Deffner, Sebastian},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Deffner - Unknown - Geometric quantum speed limits a case for Wigner phase space.pdf:pdf},
title = {{Geometric quantum speed limits: a case for Wigner phase space}},
url = {https://arxiv.org/pdf/1704.03357.pdf}
}
@article{Viola1998,
author = {Viola, Lorenza and Lloyd, Seth},
doi = {10.1103/PhysRevA.58.2733},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {oct},
number = {4},
pages = {2733--2744},
publisher = {American Physical Society},
title = {{Dynamical suppression of decoherence in two-state quantum systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.58.2733},
volume = {58},
year = {1998}
}
@article{Short2012,
author = {Short, Anthony J and Farrelly, Terence C},
doi = {10.1088/1367-2630/14/1/013063},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Short, Farrelly - 2012 - Quantum equilibration in finite time.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
month = {jan},
number = {1},
pages = {013063},
publisher = {IOP Publishing},
title = {{Quantum equilibration in finite time}},
url = {http://stacks.iop.org/1367-2630/14/i=1/a=013063?key=crossref.b41e456470b0de57bbf0087f5f5b6357},
volume = {14},
year = {2012}
}
@article{M2016,
abstract = {Fermi's golden rule is of great importance in quantum dynamics. However, in many textbooks on quantum mechanics, its contents and limitations are obscured by the approximations and arguments in the derivation, which are inevitable because of the generic setting considered. Here we propose to introduce it by an ideal model, in which the quasi-continuum band consists of equaldistant levels extending from −∞ to +∞, and each of them couples to the discrete level with the same strength. For this model, the transition probability in the first order perturbation approximation can be calculated analytically by invoking the Poisson summation formula. It turns out to be a piecewise linear function of time, demonstrating on one hand the key features of Fermi's golden rule, and on the other hand that the rule breaks down beyond the Heisenberg time, even when the first order perturbation approximation itself is still valid.},
archivePrefix = {arXiv},
arxivId = {arXiv:1604.06916v2},
author = {M, Zhang J},
eprint = {arXiv:1604.06916v2},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/M - 2016 - Fermi's golden rule its derivation and breakdown by an ideal model.pdf:pdf},
keywords = {()},
title = {{Fermi's golden rule: its derivation and breakdown by an ideal model}},
url = {https://arxiv.org/pdf/1604.06916.pdf},
year = {2016}
}
@article{Trofymchuk,
author = {Trofymchuk, Kateryna and Reisch, Andreas and Didier, Pascal and Fras, Fran{\c{c}}ois and Gilliot, Pierre and Mely, Yves and Klymchenko, Andrey S},
doi = {10.1038/s41566-017-0001-7},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Trofymchuk et al. - Unknown - Giant light-harvesting nanoantenna for single-molecule detection in ambient light.pdf:pdf},
journal = {Nat. Photonics},
title = {{Giant light-harvesting nanoantenna for single-molecule detection in ambient light}},
url = {https://www.nature.com/articles/s41566-017-0001-7.pdf}
}
@article{Raussendorf2001,
author = {Raussendorf, Robert and Briegel, Hans J.},
doi = {10.1103/PhysRevLett.86.5188},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
number = {22},
pages = {5188--5191},
title = {{A One-Way Quantum Computer}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.86.5188},
volume = {86},
year = {2001}
}
@article{Korzekwa2016,
author = {Korzekwa, Kamil and Lostaglio, Matteo and Oppenheim, Jonathan and Jennings, David},
doi = {10.1088/1367-2630/18/2/023045},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Korzekwa et al. - 2016 - The extraction of work from quantum coherence.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
month = {feb},
number = {2},
pages = {023045},
publisher = {IOP Publishing},
title = {{The extraction of work from quantum coherence}},
url = {http://stacks.iop.org/1367-2630/18/i=2/a=023045?key=crossref.736f297386b5d1712392b8f24aa31202},
volume = {18},
year = {2016}
}
@article{Marchand2018,
abstract = {Discovering the low-energy conformations of a molecule is of great interest to computational chemists, with applications in in silico materials design and drug discovery. In this paper, we propose a variable neighbourhood search heuristic for the conformational search problem. Using the structure of a molecule, neighbourhoods are chosen to allow for efficient optimization using a binary quadratic optimizer. The method is flexible with respect to the choice of molecular force field and the number of discretization levels in the search space, and can be further generalized to take advantage of higher-order binary polynomial optimizers. It is well-suited for the use of devices such as quantum annealers. After carefully defining neighbourhoods, the method easily adapts to the size and topology of these devices, allowing for seamless scaling alongside their future improvements.},
archivePrefix = {arXiv},
arxivId = {1811.06999},
author = {Marchand, D. J. J. and Noori, M. and Roberts, A. and Rosenberg, G. and Woods, B. and Yildiz, U. and Coons, M. and Devore, D. and Margl, P.},
eprint = {1811.06999},
file = {::},
month = {nov},
title = {{A Variable Neighbourhood Descent Heuristic for Conformational Search Using a Quantum Annealer}},
url = {http://arxiv.org/abs/1811.06999},
year = {2018}
}
@article{Demkowicz-Dobrzanski2012,
abstract = {Quantum metrology employs the properties of quantum states to further enhance the accuracy of some of the most precise measurement schemes to date. Here, a method for estimating the upper bounds to achievable precision in quantum-enhanced metrology protocols in the presence of decoherence is presented.},
author = {Demkowicz-Dobrza{\'{n}}ski, Rafa{\l} and Ko{\l}ody{\'{n}}ski, Jan and Guţă, Mădălin},
doi = {10.1038/ncomms2067},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Demkowicz-Dobrza{\'{n}}ski, Ko{\l}ody{\'{n}}ski, Guţă - 2012 - The elusive Heisenberg limit in quantum-enhanced metrology.pdf:pdf},
issn = {2041-1723},
journal = {Nat. Commun.},
keywords = {Atomic and molecular physics,Quantum optics},
month = {jan},
number = {1},
pages = {1063},
publisher = {Nature Publishing Group},
title = {{The elusive Heisenberg limit in quantum-enhanced metrology}},
url = {http://www.nature.com/articles/ncomms2067},
volume = {3},
year = {2012}
}
@article{Fung2014,
author = {Fung, Chi-Hang Fred and Chau, H. F.},
doi = {10.1103/PhysRevA.90.022333},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Fung, Chau - 2014 - Relation between physical time-energy cost of a quantum process and its information fidelity.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {aug},
number = {2},
pages = {022333},
publisher = {American Physical Society},
title = {{Relation between physical time-energy cost of a quantum process and its information fidelity}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.90.022333},
volume = {90},
year = {2014}
}
@article{Binder2015a,
author = {Binder, Felix and Vinjanampathy, Sai and Modi, Kavan and Goold, John},
doi = {10.1103/PhysRevE.91.032119},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Binder et al. - 2015 - Quantum thermodynamics of general quantum processes.pdf:pdf},
issn = {1539-3755},
journal = {Phys. Rev. E},
month = {mar},
number = {3},
pages = {032119},
publisher = {American Physical Society},
title = {{Quantum thermodynamics of general quantum processes}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.91.032119},
volume = {91},
year = {2015}
}
@article{Anwar2012,
author = {Anwar, Hussain and Campbell, Earl T and Browne, Dan E},
doi = {10.1088/1367-2630/14/6/063006},
issn = {1367-2630},
journal = {New J. Phys.},
month = {jun},
number = {6},
pages = {063006},
publisher = {IOP Publishing},
title = {{Qutrit magic state distillation}},
url = {http://stacks.iop.org/1367-2630/14/i=6/a=063006?key=crossref.ffdb61c9de1ffc41f92d4f7067a5755b},
volume = {14},
year = {2012}
}
@article{Horodecki2013,
author = {Horodecki, Micha{\l} and Oppenheim, Jonathan and Scovil, H. E. D. and Schulz-DuBois, E. O. and Geusic, J. E. and Schulz-DuBios, E. O. and Scovil, H. E. D. and Alicki, R. and Howard, J. and Geva, E. and Kosloff, R. and H{\"{a}}nggi, P. and Marchesoni, F. and Allahverdyan, A. E. and Nieuwenhuizen, T. M. and Feldmann, T. and Kosloff, R. and Linden, N. and Popescu, S. and Skrzypczyk, P. and Scully, M. O. and Rousselet, J. and Salome, L. and Ajdari, A. and Prost, J. and Faucheux, L. P. and Bourdieu, L. S. and Kaplan, P. D. and Libchaber, A. J. and Bennett, C. H. and Baugh, J. and Moussa, O. and Ryan, C. and Nayak, A. and Laflamme, R. and Popescu, S. and Short, A. and Winter, A. and Rio, L. Del and {\AA}berg, J. and Renner, R. and Dahlsten, O. and Vedral, V. and Donald, M. J. and Esposito, M. and den Broeck, C. V. and Horodecki, M. and Horodecki, P. and Oppenheim, J. and Dahlsten, O. and Renner, R. and Rieper, E. and Vedral, V. and Gour, G. and Spekkens, R. W. and Janzing, D. and Wocjan, P. and Zeier, R. and Geiss, R. and Beth, T. and Werner, R. F. and Bennett, C. H. and DiVincenzo, D. P. and Smolin, J. A. and Wootters, W. K. and Horodecki, M. and Oppenheim, J. and Horodecki, R. and Petz, D. and Datta, N. and {\AA}berg, J. and Ruch, E. and Ruch, E. and Mead, A. and Ruch, E. and Schranner, R. and Seligman, T. H. and Janzing, D. and Wocjan, P. and Zeier, R. and Geiss, R. and Beth, T. and Brand{\~{a}}o, F. G. and Plenio, M. B.},
doi = {10.1038/ncomms3059},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Horodecki et al. - 2013 - Fundamental limitations for quantum and nanoscale thermodynamics.pdf:pdf},
issn = {2041-1723},
journal = {Nat. Commun.},
month = {jun},
pages = {262--263},
publisher = {Nature Publishing Group},
title = {{Fundamental limitations for quantum and nanoscale thermodynamics}},
url = {http://www.nature.com/doifinder/10.1038/ncomms3059},
volume = {4},
year = {2013}
}
@article{Poulin,
abstract = {We consider the manifold of all quantum many-body states that can be generated by arbitrary time-dependent local Hamiltonians in a time that scales polynomially in the system size, and show that it occupies an exponentially small volume in Hilbert space. This implies that the overwhelming majority of states in Hilbert space are not physical as they can only be produced after an exponentially long time. We establish this fact by making use of a time-dependent generalization of the Suzuki-Trotter expansion, followed by a well-known counting argument. This also demonstrates that a computational model based on arbitrarily rapidly changing Hamiltonians is no more powerful than the standard quantum circuit model.},
author = {Poulin, David and Qarry, Angie and Somma, Rolando and Verstraete, Frank},
doi = {10.1103/PhysRevLett.106.170501},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Poulin et al. - Unknown - Quantum Simulation of Time-Dependent Hamiltonians and the Convenient Illusion of Hilbert Space.pdf:pdf},
title = {{Quantum Simulation of Time-Dependent Hamiltonians and the Convenient Illusion of Hilbert Space}}
}
@article{Bender2000,
author = {Bender, Carl M and Brody, Dorje C and Meister, Bernhard K},
doi = {10.1088/0305-4470/33/24/302},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bender, Brody, Meister - 2000 - Quantum mechanical Carnot engine.pdf:pdf},
journal = {J. Phys. A. Math. Gen.},
month = {jun},
number = {24},
pages = {4427--4436},
publisher = {IOP Publishing},
title = {{Quantum mechanical Carnot engine}},
url = {http://stacks.iop.org/0305-4470/33/i=24/a=302?key=crossref.3fca8c5b9cde5e935cb6f1ae0c1a3459},
volume = {33},
year = {2000}
}
@article{Steffen2003,
author = {Steffen, Matthias and van Dam, Wim and Hogg, Tad and Breyta, Greg and Chuang, Isaac},
doi = {10.1103/PhysRevLett.90.067903},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {6},
pages = {067903},
publisher = {American Physical Society},
title = {{Experimental Implementation of an Adiabatic Quantum Optimization Algorithm}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.067903},
volume = {90},
year = {2003}
}
@article{Russell2014,
abstract = {We derive a family of quantum speed limit results in time independent systems with pure states and a finite dimensional state space, by using a geometric method based on right invariant action functionals on SU (N). The method relates speed limits for implementing quantum gates to bounds on orthogonality times. We reproduce the known result of the Margolus Levitin theorem, and a known generalisation of the Margolis-Levitin theorem, as special cases of our method, which produces a rich family of other similar speed limit formulas corresponding to positive homogeneous functions on su(n). We discuss the general relationship between speed limits for controlling a quantum state and a system's time evolution operator. 1 Problem and Motivation There is much interest in the speed limit to QIP tasks; a range of perspectives can be found in [9, 19, 16, 7, 20]. There is also recent interest in applications of geometry to such issues [2, 14, 27]. The first of the central problems concerning the quantum speed limit (QSL) is how quickly the time evolution operator of a given system can be driven to a certain desired operato O. This problem is the topic of many papers, notably [9, 19, 23, 24, 1, 3], which apply techniques from differential geometry. The second central problem is that of controlling a system's state |$\psi$ 0 so that it reaches a desired state |$\psi$ 1 in the fastest possible time. This question has a special instance for orthogonal states, 1 |$\psi$ 0 = 0. This case has attracted much attention since shortly after the dawn of quantum theory [16, 6]. More recently it has gained new attention due to its relevance to computer science and the physical limits to computation [15, 17]. Lloyd [15] provides a short discussion of the importance of orthogonal states (in the standard inner product of C N) to assessing the capacity of a physical system for QIP: there are pairs of (pure) states which are distinguishable with a single quantum measurement, at least in principle. Additional interesting work on both these problems, hinting at the mathematical connection between them, can be found in [9]. Here we focus on the relationship between the two problems in time independent systems, and on showing that well known bounds like the Margolus-Levitin theorem [16] can be thought of as speed limits on SU (N). This view is clarifying and unifies the two seemingly separate issues: that of controllin U t and of orthogonalising a given state. The structure of this paper is as follows. First we review existing QSL results (2). In 3 we derive a speed limit theorem for positive homogeneous functions on su(n). Then we apply this theorem to derive a family of limits for orthogonality times in 4, and show that the ML bound and Time-Energy uncertainty relation are special cases of this family. In 5 we discuss the connection between such speed limits for the two central problems.},
archivePrefix = {arXiv},
arxivId = {1410.3209v1},
author = {Russell, Benjamin and Stepney, Susan},
eprint = {1410.3209v1},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Russell, Stepney - 2014 - A Geometrical Derivation of a Family of Quantum Speed Limit Results.pdf:pdf},
keywords = {()},
title = {{A Geometrical Derivation of a Family of Quantum Speed Limit Results}},
url = {https://arxiv.org/abs/1410.3209v1},
year = {2014}
}
@article{Macieszczak2016,
author = {Macieszczak, Katarzyna and Guţă, Mădălin and Lesanovsky, Igor and Garrahan, Juan P.},
doi = {10.1103/PhysRevLett.116.240404},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Macieszczak et al. - 2016 - Towards a Theory of Metastability in Open Quantum Dynamics.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jun},
number = {24},
pages = {240404},
publisher = {American Physical Society},
title = {{Towards a Theory of Metastability in Open Quantum Dynamics}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.240404},
volume = {116},
year = {2016}
}
@article{Friis2017,
abstract = {One of the most fundamental tasks in quantum thermodynamics is extracting energy from one system and subsequently storing this energy in an appropriate battery. Both of these steps, work extraction and charging, can be viewed as cyclic Hamiltonian processes acting on individual quantum systems. Interestingly, so-called passive states exist, whose energy cannot be lowered by unitary operations, but it is safe to assume that the energy of any not fully charged battery may be increased unitarily. However, unitaries raising the average energy by the same amount may differ in qualities such as their precision, fluctuations, and charging power. Moreover, some unitaries may be extremely difficult to realize in practice. It is hence of crucial importance to understand the qualities that can be expected from practically implementable transformations. Here, we consider the limitations on charging batteries when restricting to the feasibly realizable family of Gaussian unitaries. We derive optimal protocols for general unitary operations as well as for the restriction to Gaussian unitaries. We find that Gaussian battery charging, while simpler to implement, comes at the price of inevitable energy fluctuations that may render the charging process less useful.},
archivePrefix = {arXiv},
arxivId = {1708.00749},
author = {Friis, Nicolai and Huber, Marcus},
doi = {10.22331/q-2018-04-23-61},
eprint = {1708.00749},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Friis, Huber - 2017 - Precision and Work Fluctuations in Gaussian Battery Charging.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Friis, Huber - 2017 - Precision and Work Fluctuations in Gaussian Battery Charging(2).pdf:pdf},
journal = {Quantum},
month = {aug},
pages = {61},
publisher = {Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften},
title = {{Precision and Work Fluctuations in Gaussian Battery Charging}},
url = {http://arxiv.org/abs/1708.00749 https://arxiv.org/pdf/1708.00749.pdf http://dx.doi.org/10.22331/q-2018-04-23-61},
volume = {2},
year = {2017}
}
@article{Jurcevic2014a,
abstract = {The fine control afforded by trapped atomic ions is used to explore experimentally how the range of interactions between the ions influences the spreading of information in quantum many-body systems.},
author = {Jurcevic, P. and Lanyon, B. P. and Hauke, P. and Hempel, C. and Zoller, P. and Blatt, R. and Roos, C. F.},
doi = {10.1038/nature13461},
file = {::},
issn = {0028-0836},
journal = {Nature},
keywords = {Quantum information,Quantum mechanics,Qubits},
month = {jul},
number = {7508},
pages = {202--205},
publisher = {Nature Publishing Group},
title = {{Quasiparticle engineering and entanglement propagation in a quantum many-body system}},
url = {http://www.nature.com/articles/nature13461},
volume = {511},
year = {2014}
}
@article{Groblacher2006,
author = {Gr{\"{o}}blacher, Simon and Jennewein, Thomas and Vaziri, Alipasha and Weihs, Gregor and Zeilinger, Anton and S, Wiesner and G, Bennett C H Brassard and G, Bennett C H and Brassard and K, Ekert A and {Gobby C}, Yuan Z L and Shields A J and {Takesue H}, Diamanti E, Honjo T, Langrock C, Fejer M M, Inoue K and Yamamoto Y and {Stucki D}, Gisin N, Guinnard O, Ribordy G and Zbinden H and {Gobby C}, Yuan Z L and Shields A J and {Kurtsiefer C}, Zarda P, Halder M, Weinfurter H, Gorman P M, Tapster P R and Rarity J G and et Al, Resch K J and et Al, Peng C-Z and et Al, Poppe A and {Barreiro J T}, Langford N K, Peters N A and Kwiat P G and {Cinelli C}, Barbieri M, Perris R, Mataloni P and Martini F D and {Fitzi M}, Gisin N and Maurer U and {Molina-Terriza G}, Vaziri A, Ursin R and Zeilinger A and {Walborn S P}, Lemelle D S, Almeida M P and Ribeiro P H S and {Yang T}, Zhang Q, Zhang J, Yin J, Zhao Z, {\.{Z}}ukowski M, Chen Z-B and Pan J-W and {Fuchs C A}, Gisin N, Griffiths R B, Niu C-S and Peres A and D, Bru{\ss} and {Durt T}, Cerf N J, Gisin N and {\.{Z}}ukowski M and {Jennewein T}, Simon C, Weihs G, Weinfurter H and Zeilinger A and {Mair A}, Vaziri A, Weihs G and Zeilinger A and {Caetano D P}, Almeida M P, Ribeiro P H S, Huguenin J A O, dos Santos B C and Khoury A Z and {Franke-Arnold S}, Barnett S M, Padgett M J and Allen L and {Torres J P}, Molina-Terriza G and Torner L and {Vaziri A}, Pan J-W, Jennewein T, Weihs G and Zeilinger A and {Collins D}, Gisin N, Linden N, Massar S and Popescu S and {Kaszlikowski D}, Kwek L C, Chen J-L, Zukowski M and Oh C H and {Clauser J F}, Horne M A, Shimony A and Holt R A and {Ac{\'{i}}n A}, Durt T, Gisin N and Latorre J I and {Vaziri A}, Weihs G and Zeilinger A and {Arlt J}, Dholakia K, Allen L and Padgett M J and {Bazhenov V Y}, Vasnetsov M V and Soskin M S and {Vaziri A}, Weihs G and Zeilinger A and {Gibson G}, Courtial J, Padgett M J, Vasnetsov M, Pas'ko V, Barnett S M and Franke-Arnold S and {Thew R T}, Ac{\'{i}}n A, Zbinden H and Gisin N and J-W, Chen Z-B Zhang Q Bao X-H Schmiedmayer J Pan},
doi = {10.1088/1367-2630/8/5/075},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gr{\"{o}}blacher et al. - 2006 - Experimental quantum cryptography with qutrits.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
month = {may},
number = {5},
pages = {75--75},
publisher = {IOP Publishing},
title = {{Experimental quantum cryptography with qutrits}},
url = {http://stacks.iop.org/1367-2630/8/i=5/a=075?key=crossref.573f2b8a35f0eb373ce957b5369c9a12},
volume = {8},
year = {2006}
}
@article{Lloyd2000,
author = {Lloyd, Seth},
doi = {10.1038/35023282},
issn = {00280836},
journal = {Nature},
month = {aug},
number = {6799},
pages = {1047--1054},
publisher = {Nature Publishing Group},
title = {{Ultimate physical limits to computation}},
url = {http://www.nature.com/doifinder/10.1038/35023282},
volume = {406},
year = {2000}
}
@article{Bukov2018a,
archivePrefix = {arXiv},
arxivId = {1705.00565},
author = {Bukov, Marin and Day, Alexandre G. R. R. and Sels, Dries and Weinberg, Phillip and Polkovnikov, Anatoli and Mehta, Pankaj},
doi = {10.1103/PhysRevX.8.031086},
eprint = {1705.00565},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bukov et al. - 2018 - Reinforcement Learning in Different Phases of Quantum Control.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bukov et al. - 2017 - Reinforcement Learning in Different Phases of Quantum Control.pdf:pdf},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {may},
number = {3},
pages = {031086},
publisher = {American Physical Society},
title = {{Reinforcement Learning in Different Phases of Quantum Control}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.8.031086 http://arxiv.org/abs/1705.00565 https://arxiv.org/pdf/1705.00565.pdf},
volume = {8},
year = {2017}
}
@article{Frowis2012,
abstract = {The “speed” of unitary quantum evolution was recently shown to be connected to entanglement in multipartite quantum systems. Here, we discuss a tighter version of the Mandelstam-Tamm uncertainty relation that depends on the Fisher information. The passage time is estimated by a lower bound that depends inversely proportional to the square root of the Fisher information. This leads to a better understanding of the origin of a fast quantum time-evolution of entangled states.},
author = {Fr{\"{o}}wis, F.},
doi = {10.1103/PhysRevA.85.052127},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Fr{\"{o}}wis - 2012 - Kind of entanglement that speeds up quantum evolution.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Fr{\"{o}}wis - 2012 - Kind of entanglement that speeds up quantum evolution(2).pdf:pdf},
issn = {10502947},
journal = {Phys. Rev. A},
month = {may},
number = {5},
pages = {052127},
publisher = {American Physical Society},
title = {{Kind of entanglement that speeds up quantum evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.85.052127},
volume = {85},
year = {2012}
}
@article{Ozols2009,
author = {Ozols, Maris},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ozols - 2009 - How to generate a random unitary matrix(2).pdf:pdf},
title = {{How to generate a random unitary matrix}},
url = {http://home.lu.lv/{~}sd20008/papers/essays/Random unitary [paper].pdf},
year = {2009}
}
@article{Mondal2016,
abstract = {We cast observable measure of quantum coherence as a resource to control the quantum speed limit (QSL) for unitary evolutions. For non-unitary evolutions, QSL depends on that of the state of the system and environment together. We show that the product of the time bound and the coherence (asymmetry) or the quantum part of the uncertainty behaves in a geometric way under partial elimination and classical mixing of states. These relations give a new insight into the quantum speed limit. We also show that our bound is experimentally measurable and is tighter than various existing bounds in the literature.},
author = {Mondal, Debasis and Datta, Chandan and Sazim, Sk},
doi = {10.1016/J.PHYSLETA.2015.12.015},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Mondal, Datta, Sazim - 2016 - Quantum coherence sets the quantum speed limit for mixed states.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Mondal, Datta, Sazim - 2015 - Quantum Coherence Sets The Quantum Speed Limit For Mixed States.pdf:pdf},
issn = {0375-9601},
journal = {Phys. Lett. A},
keywords = {CPTP maps,Coherence,Quantum speed limit,Skew information},
month = {feb},
number = {5-6},
pages = {689--695},
publisher = {North-Holland},
title = {{Quantum coherence sets the quantum speed limit for mixed states}},
url = {https://www.sciencedirect.com/science/article/pii/S0375960115010518 http://linkinghub.elsevier.com/retrieve/pii/S0375960115010518 www.elsevier.com/locate/pla},
volume = {380},
year = {2015}
}
@article{Law2011,
abstract = {The problem of generating random quantum states is of a great interest from the quantum in-formation theory point of view. In this paper we present a package for Mathematica computing system harnessing a specific piece of hardware, namely Quantis quantum random number generator (QRNG), for investigating statistical properties of quantum states. The described package imple-ments a number of functions for generating random states, which use Quantis QRNG as a source of randomness. It also provides procedures which can be used in simulations not related directly to quantum information processing.},
author = {Law, Jaross and Miszczak, Adam},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Law, Miszczak - 2011 - Generating and using truly random quantum states in Mathematica.pdf:pdf},
keywords = {0270Wz,0367-a,0705Tp Program Summary,quantum information,quantum random number generators PACS numbers,random density matrices},
title = {{Generating and using truly random quantum states in Mathematica}},
url = {https://arxiv.org/pdf/1102.4598.pdf},
year = {2011}
}
@article{Papoular,
abstract = {We report a prediction for the delay measured in an optical tunneling experiment using Hong–Ou–Mandel (HOM) interference, taking into account the Goos-H{\"{a}}nchen shift generalized to frustrated total internal reflection situations. We precisely state assumptions under which the tunneling delay measured by an HOM interferometer can be calculated. We show that, under these assumptions, the measured delay is the group delay, and that it is apparently 'superluminal' for sufficiently thick air gaps. We also show how an HOM signal with multiple minima can be obtained, and that the shape of such a signal is not appreciably affected by the presence of the optical tunneling zone, thus ruling out the explanation of the anomalously short tunneling delays in terms of a reshaping of the wavepacket as it goes through the tunneling zone. Finally, we compare the predicted tunneling delay to a relevant classical delay and conclude that our predictions involve no non–causal effect.},
author = {Papoular, D J and Clad{\'{e}}, P and Polyakov, S V and Mccormick, C F and Migdall, A L and Lett, P D},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Papoular et al. - Unknown - Measuring optical tunneling times using a Hong–Ou–Mandel interferometer.pdf:pdf},
title = {{Measuring optical tunneling times using a Hong–Ou–Mandel interferometer}},
url = {https://physics.nist.gov/Divisions/Div844/publications/migdall/Tunneling{\_}Papoular.pdf}
}
@article{Ekert2002,
author = {Ekert, Artur K. and Alves, Carolina Moura and Oi, Daniel K. L. and Horodecki, Micha{\l} and Horodecki, Pawe{\l} and Kwek, L. C.},
doi = {10.1103/PhysRevLett.88.217901},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ekert et al. - 2002 - Direct Estimations of Linear and Nonlinear Functionals of a Quantum State.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {may},
number = {21},
pages = {217901},
publisher = {American Physical Society},
title = {{Direct Estimations of Linear and Nonlinear Functionals of a Quantum State}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.88.217901},
volume = {88},
year = {2002}
}
@article{Shivam2016,
abstract = {We compare the roles of the Bures-Helstrom (BH) and Bogoliubov-Kubo-Mori (BKM) metrics in the subject of quantum information geometry. We note that there are two limits involved in state discrimination, which we call the "thermodynamic" limit (of {\$}N{\$}, the number of realizations going to infinity) and the infinitesimal limit (of the separation of states tending to zero). We show that these two limits do not commute in the quantum case. Taking the infinitesimal limit first leads to the BH metric and the corresponding Cram$\backslash$'er-Rao bound, which is widely accepted in this subject. Taking limits in the opposite order leads to the BKM metric, which results in a weaker Cram$\backslash$'er-Rao bound. This lack of commutation of limits is a purely quantum phenomenon arising from quantum entanglement. We can exploit this phenomenon to gain a quantum advantage in state discrimination and get around the limitation imposed by the Bures-Helstrom Cram$\backslash$'er-Rao (BHCR) bound. We propose a technologically feasible experiment with cold atoms to demonstrate the quantum advantage in the simple case of two qubits.},
archivePrefix = {arXiv},
arxivId = {1609.07279},
author = {Shivam, Kumar and Reddy, Anirudh and Samuel, Joseph and Sinha, Supurna},
doi = {10.1142/S0219749918500326},
eprint = {1609.07279},
file = {::},
month = {sep},
title = {{Entropy and Geometry of Quantum States}},
url = {http://arxiv.org/abs/1609.07279 http://dx.doi.org/10.1142/S0219749918500326},
year = {2016}
}
@article{Khajavikhan2012,
abstract = {Nanoscale resonant cavities can be engineered to enhance the interaction between light and matter, one practical objective being the realization of efficient lasers that occupy a tiny volume on a chip. Mercedeh Khajavikhan and colleagues describe a new family of resonators that overcome one of the main obstacles that have hindered previous efforts toward this goal. Specifically, their resonator design allows the size of the laser cavity to be scaled down without increasing the threshold power required to drive lasing and can even be engineered to remove the threshold altogether.},
author = {Khajavikhan, M. and Simic, A. and Katz, M. and Lee, J. H. and Slutsky, B. and Mizrahi, A. and Lomakin, V. and Fainman, Y.},
doi = {10.1038/nature10840},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Khajavikhan et al. - 2012 - Thresholdless nanoscale coaxial lasers.pdf:pdf},
issn = {0028-0836},
journal = {Nature},
keywords = {Electronics,LEDs and light sources,Lasers,Nanoscale devices,photonics and device physics},
month = {feb},
number = {7384},
pages = {204--207},
publisher = {Nature Publishing Group},
title = {{Thresholdless nanoscale coaxial lasers}},
url = {http://www.nature.com/articles/nature10840},
volume = {482},
year = {2012}
}
@article{Campaioli2018a,
abstract = {Book chapter in "Thermodynamics in the quantum regime - Recent Progress and Outlook" -- This chapter is a survey of the published literature on quantum batteries -- ensembles of non-degenerate quantum systems on which energy can be deposited, and from which work can be extracted. A pedagogical approach is used to familiarize the reader with the main results obtained in this field, starting from simple examples and proceeding with in-depth analysis. An outlook for the field and future developments are discussed at the end of the chapter.},
archivePrefix = {arXiv},
arxivId = {1805.05507},
author = {Campaioli, Francesco and Pollock, Felix A. and Vinjanampathy, Sai},
eprint = {1805.05507},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli, Pollock, Vinjanampathy - 2018 - Quantum Batteries - Review Chapter.pdf:pdf},
month = {may},
title = {{Quantum Batteries - Review Chapter}},
url = {http://arxiv.org/abs/1805.05507},
year = {2018}
}
@article{Senko2015,
author = {Senko, C. and Richerme, P. and Smith, J. and Lee, A. and Cohen, I. and Retzker, A. and Monroe, C.},
doi = {10.1103/PhysRevX.5.021026},
file = {::},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {jun},
number = {2},
pages = {021026},
publisher = {American Physical Society},
title = {{Realization of a Quantum Integer-Spin Chain with Controllable Interactions}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.5.021026},
volume = {5},
year = {2015}
}
@article{Meng2015,
abstract = {We derive a sharp bound as the quantum speed limit (QSL) for the minimal evolution time of quantum open systems in the non-Markovian strong-coupling regime with initial mixed states by considering the effects of both renormalized Hamiltonian and dissipator. For a non-Markovian quantum open system, the possible evolution time between two arbitrary states is not unique, among the set of which we find that the minimal one and its QSL can decrease more steeply by adjusting the coupling strength of the dissipator, which thus provides potential improvements of efficiency in many quantum physics and quantum information areas. As a fundamental bound for the evolution time of quantum systems, the quantum speed limit (QSL) (also referred to as quantum evolution time limit) plays an important role in tremendous areas of quan-tum physics and quantum information, such as quantum computation and communication 1,2 , quantum metrology 3 , cavity quantum electrodynamics 4 , quantum control 5 , etc. The derivation of QSL is most required for the purpose of simplification and/or optimization in theoretical analysis, since in most quantum-cases one only needs to derive a lower bound on the minimal time of evolution without solving the exact equation to see the dominant factors in evolution and/or optimize our demand. For closed quantum systems, two types of QSL have been derived at the start: the Mandelstam-Tamm (MT) bound $\tau$ $\pi$ ≥ /(∆) ħ E 2 6},
author = {Meng, Xiangyi and Wu, Chengjun and Guo, Hong},
doi = {10.1038/srep16357},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Meng, Wu, Guo - 2015 - Minimal evolution time and quantum speed limit of non- Markovian open systems.pdf:pdf},
title = {{Minimal evolution time and quantum speed limit of non- Markovian open systems}},
url = {https://www.nature.com/articles/srep16357.pdf},
year = {2015}
}
@article{Amico,
abstract = {Recent interest in aspects common to quantum information and condensed matter has prompted a flurry of activity at the border of these disciplines that were far distant until a few years ago. Numerous interesting questions have been addressed so far. Here an important part of this field, the properties of the entanglement in many-body systems, are reviewed. The zero and finite temperature properties of entanglement in interacting spin, fermion, and boson model systems are discussed. Both bipartite and multipartite entanglement will be considered. In equilibrium entanglement is shown tightly connected to the characteristics of the phase diagram. The behavior of entanglement can be related, via certain witnesses, to thermodynamic quantities thus offering interesting possibilities for an experimental test. Out of equilibrium entangled states are generated and manipulated by means of many-body Hamiltonians. DOI: 10.1103/RevModPhys.80.517 PACS number͑s͒: 05.30.Ϫd, 03.65.Ud CONTENTS I. Introduction 518 II. Measures of Entanglement 519 A. Bipartite entanglement in pure states 519 B. Pairwise qubit entanglement in mixed states 520 C. Localizable entanglement 521 D. Entanglement witnesses 521 E. Multipartite entanglement measures 522 F. Indistinguishable particles 523 1. Two fermion entanglement 524 2. Multipartite entanglement for fermions 525 3. Entanglement of particles 525 4. Entanglement for bosons 526 G. Entanglement in harmonic systems 526 III. Model Systems 527 A. Spin models 527 1. Spin-1 / 2 models with short range interactions 527 2. Spin-1 / 2 models with infinite range interaction 528 3. Frustrated spin-1 / 2 models 529 4. Spin-1 models 529 B. Strongly correlated fermionic models 530 C. Spin-boson models 530 D. Harmonic lattices 531 IV. Pairwise Entanglement 531},
author = {Amico, Luigi and Fazio, Rosario and Osterloh, Andreas and Vedral, Vlatko},
doi = {10.1103/RevModPhys.80.517},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Amico et al. - Unknown - Entanglement in many-body systems.pdf:pdf},
title = {{Entanglement in many-body systems}}
}
@article{Das2018,
abstract = {Pati (Physics Letters A, 2000) derived a sufficient condition for the existence of Schmidt decomposition in tripartite Hilbert spaces. In this paper, we show that the condition is erroneous by demonstrating some counter-examples. Moreover, we suitably modify the condition and provide a correctness proof. We also show for the first time how this can be generalized to {\$}n{\$}-partite Hilbert spaces for any {\$}n\backslashgeq 2{\$}. Finally, we prove that this condition is also a necessary condition.},
archivePrefix = {arXiv},
arxivId = {1805.12274},
author = {Das, Spandan and Paul, Goutam},
eprint = {1805.12274},
file = {::},
month = {may},
title = {{Necessary and sufficient condition for the existence of Schmidt decomposition in multipartite Hilbert spaces}},
url = {http://arxiv.org/abs/1805.12274},
year = {2018}
}
@article{Heisenberg,
author = {Heisenberg, W.},
doi = {10.1007/BF01397280},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Heisenberg - Unknown - {\"{U}}ber den anschaulichen Inhalt der quantentheoretischen Kinematik und Mechanik.pdf:pdf},
journal = {Zeitschrift f{\"{u}}r Phys.},
number = {3-4},
pages = {172--198},
publisher = {Springer-Verlag},
title = {{{\"{U}}ber den anschaulichen Inhalt der quantentheoretischen Kinematik und Mechanik}},
volume = {43}
}
@article{Uffink1985,
author = {Uffink, J. B. M. and Hilgevoord, J.},
doi = {10.1007/BF00739034},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uffink, Hilgevoord - 1985 - Uncertainty principle and uncertainty relations.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uffink, Hilgevoord - 1985 - Uncertainty principle and uncertainty relations(2).pdf:pdf},
issn = {00159018},
journal = {Found. Phys.},
month = {sep},
number = {9},
pages = {925--944},
publisher = {Kluwer Academic Publishers-Plenum Publishers},
title = {{Uncertainty principle and uncertainty relations}},
url = {http://link.springer.com/10.1007/BF00739034},
volume = {15},
year = {1985}
}
@article{Anandan1990,
abstract = {For an arbitrary quantum evolution, it is shown that the integral of the uncertainty of energy with respect to time is independent of the particular Hamiltonian used to transport the quantum system along a given curve in the projective Hilbert space. It is the distance along this curve measured by the Fubini- Study metric. This gives a new time-energy uncertainty principle. New geometric meanings to time as measured by a clock and the transition probability during a quantum measurement are also obtained},
author = {Anandan, J. and Aharonov, Y.},
doi = {10.1103/PhysRevLett.65.1697},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Anandan, Aharonov - 1990 - Geometry of quantum evolution.pdf:pdf},
issn = {00319007},
journal = {Phys. Rev. Lett.},
month = {oct},
number = {14},
pages = {1697--1700},
publisher = {American Physical Society},
title = {{Geometry of quantum evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.65.1697},
volume = {65},
year = {1990}
}
@article{Fleischhauer2002,
author = {Fleischhauer, M. and Lukin, M. D.},
doi = {10.1103/PhysRevA.65.022314},
file = {::},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jan},
number = {2},
pages = {022314},
publisher = {American Physical Society},
title = {{Quantum memory for photons: Dark-state polaritons}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.65.022314},
volume = {65},
year = {2002}
}
@article{Bhattacharyya1983,
abstract = {The Mandelstam-Tamm time-energy inequality is exploited to obtain a transparent expression of the lifetime-energy uncertainty relation for decaying quantum systems along with some useful features of the quantum non-decay probability.},
author = {Bhattacharyya, K},
doi = {10.1088/0305-4470/16/13/021},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bhattacharyya - 1983 - Quantum decay and the Mandelstam-Tamm-energy inequality.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bhattacharyya - 1983 - Quantum decay and the Mandelstam-Tamm-energy inequality(2).pdf:pdf},
issn = {0305-4470},
journal = {J. Phys. A. Math. Gen.},
month = {sep},
number = {13},
pages = {2993--2996},
publisher = {IOP Publishing},
title = {{Quantum decay and the Mandelstam-Tamm-energy inequality}},
url = {http://stacks.iop.org/0305-4470/16/i=13/a=021?key=crossref.a6b0402182ae69bc07e04b642dd39ebd},
volume = {16},
year = {1999}
}
@article{Knee2015,
abstract = {Universal quantum simulation may provide insights into those many-body systems that cannot be described classically and that cannot be efficiently simulated with current technology. The Trotter formula, which decomposes a desired unitary time evolution of the simulator into a stroboscopic sequence of repeated elementary evolutions, is a key algorithmic component which makes quantum simulation of dynamics tractable. The Trotter number n sets the time scale on which a computer running this algorithm is switched from one elementary evolution to another. In the ideal case, the precision of the simulation can be arbitrarily controlled by increasing n. We study a more realistic scenario where each gate is applied imperfectly. The resultant trade-off in errors leads to an ultimate limit on the precision of the simulation. We calculate the optimum Trotter number n∗ that achieves this limit, which is the minimum statistical distance from the actual simulation to the ideal one.},
archivePrefix = {arXiv},
arxivId = {arXiv:1502.04536v1},
author = {Knee, George C and Munro, William J},
doi = {10.1103/PhysRevA.91.052327},
eprint = {arXiv:1502.04536v1},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Knee, Munro - 2015 - Optimal Trotterization in universal quantum simulators under faulty control.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
number = {5},
pages = {052327},
publisher = {Ac},
title = {{Optimal Trotterization in universal quantum simulators under faulty control}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.91.052327{\%}5Cnhttp://journals.aps.org/pra/abstract/10.1103/PhysRevA.91.052327{\%}5Cnhttp://journals.aps.org/pra/pdf/10.1103/PhysRevA.91.052327},
volume = {91},
year = {2015}
}
@article{Glaser2015,
author = {Glaser, Steffen J. and Boscain, Ugo and Calarco, Tommaso and Koch, Christiane P. and K{\"{o}}ckenberger, Walter and Kosloff, Ronnie and Kuprov, Ilya and Luy, Burkhard and Schirmer, Sophie and Schulte-Herbr{\"{u}}ggen, Thomas and Sugny, Dominique and Wilhelm, Frank K.},
doi = {10.1140/epjd/e2015-60464-1},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Glaser et al. - 2015 - Training Schr{\"{o}}dinger's cat quantum optimal control(2).pdf:pdf},
issn = {1434-6060},
journal = {Eur. Phys. J. D},
month = {dec},
number = {12},
pages = {279},
publisher = {Springer Berlin Heidelberg},
title = {{Training Schr{\"{o}}dinger's cat: quantum optimal control}},
url = {http://link.springer.com/10.1140/epjd/e2015-60464-1},
volume = {69},
year = {2015}
}
@article{Santos2015,
abstract = {Superadiabatic Controlled Evolutions and Universal Quantum Computation},
author = {Santos, Alan C. and Sarandy, Marcelo S.},
doi = {10.1038/srep15775},
file = {::},
issn = {2045-2322},
journal = {Sci. Rep.},
keywords = {Information theory and computation,Quantum information},
month = {dec},
number = {1},
pages = {15775},
publisher = {Nature Publishing Group},
title = {{Superadiabatic Controlled Evolutions and Universal Quantum Computation}},
url = {http://www.nature.com/articles/srep15775},
volume = {5},
year = {2015}
}
@article{Feynman1982,
author = {Feynman, Richard P.},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Feynman - 1982 - Simulating Physics with Computers.pdf:pdf},
journal = {Int. J. Theor. Phys.},
number = {6},
title = {{Simulating Physics with Computers}},
volume = {217},
year = {1982}
}
@article{Garcia-Pintos2018,
abstract = {The pace of evolution of physical systems is fundamentally constrained by quantum speed limits (QSL), which have found broad applications in quantum science and technology. We consider the speed of evolution for quantum systems undergoing stochastic dynamics due to continuous measurements. It is shown that that there are trajectories for which standard QSL are violated, and we provide estimates for the range of velocities in an ensemble of realizations of continuous measurement records. We determine the dispersion of the speed of evolution and characterize the full statistics of single trajectories.},
archivePrefix = {arXiv},
arxivId = {1804.01600},
author = {Garc{\'{i}}a-Pintos, Luis Pedro and del Campo, Adolfo},
eprint = {1804.01600},
month = {apr},
title = {{Violation of Quantum Speed Limits under Continuous Quantum Measurements}},
url = {http://arxiv.org/abs/1804.01600},
year = {2018}
}
@article{Zuo2002,
author = {Zuo, W. and Lejeune, A. and Lombardo, U. and Mathiot, J.F.},
doi = {10.1140/epja/i2002-10031-y},
issn = {1434-6001},
journal = {Eur. Phys. J. A},
month = {aug},
number = {4},
pages = {469--475},
publisher = {Springer-Verlag},
title = {{Microscopic three-body force for asymmetric nuclear matter}},
url = {http://link.springer.com/10.1140/epja/i2002-10031-y},
volume = {14},
year = {2002}
}
@article{Zhang2014,
author = {Zhang, Ying-Jie and Han, Wei and Xia, Yun-Jie and Cao, Jun-Peng and Fan, Heng},
doi = {10.1038/srep04890},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zhang et al. - 2014 - Quantum speed limit for arbitrary initial states.pdf:pdf},
issn = {2045-2322},
journal = {Sci. Rep.},
month = {may},
pages = {4890},
publisher = {Nature Publishing Group},
title = {{Quantum speed limit for arbitrary initial states}},
url = {http://www.nature.com/articles/srep04890},
volume = {4},
year = {2014}
}
@article{DeJong2013,
abstract = {The world needs young people who are skillful in and enthusiastic about science and who view science as their future career field. Ensuring that we will have such young people requires initiatives that engage students in interesting and motivating science experiences. Today, students can investigate scientific phenomena using the tools, data collection techniques, models, and theories of science in physical laboratories that support interactions with the material world or in virtual laboratories that take advantage of simulations. Here, we review a selection of the literature to contrast the value of physical and virtual investigations and to offer recommendations for combining the two to strengthen science learning.},
author = {de Jong, Ton and Linn, Marcia C and Zacharia, Zacharias C},
doi = {10.1126/science.1230579},
issn = {1095-9203},
journal = {Science},
month = {apr},
number = {6130},
pages = {305--8},
pmid = {23599479},
publisher = {American Association for the Advancement of Science},
title = {{Physical and virtual laboratories in science and engineering education.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/23599479},
volume = {340},
year = {2013}
}
@article{Hauke,
abstract = {Entanglement is considered an essential resource in quantum technologies, and central to the understanding of quantum many-body physics. Developing protocols to detect and quantify the entanglement of many-particle quantum states is thus a key challenge for present experiments. Here, we show that the quantum Fisher information, a witness for genuinely multipartite entanglement, becomes measurable for thermal ensembles by means of the dynamic susceptibility—that is, with resources readily available in present cold atomic-gas and condensed-matter experiments. This establishes a connection between multipartite entanglement and many-body correlations contained in response functions, with immediate implications close to quantum phase transitions, where the quantum Fisher information becomes universal, allowing us to identify strongly entangled phase transitions with a divergent multipartite entanglement. We illustrate our framework using paradigmatic quantum Ising models, and point out potential signatures in optical-lattice experiments and strongly correlated materials. A lthough entanglement is central to our understanding of quantum many-body physics 1 , its direct measurement in an actual experiment to characterize quantum phases and phase transitions has remained elusive. In a few-body quantum system, in particular in a quantum information context involving few qubits, entanglement can be measured and quantified through tomography of the density matrix 2–5 . In experiments with few atoms in optical lattices, such as engineered Bose– or Fermi– Hubbard models, entanglement entropy and purity of quantum states become measurable with protocols based on preparing copies of the quantum system in combination with the unique tools of atomic physics, including single-site manipulation and observation 6,7 . However, an intrinsic feature of these protocols is an exponential scaling of resources, and thus an a priori limit to small system sizes. In contrast, we will be interested below in quantifying multipar-tite entanglement for large system size, while still being accessible with experimentally realistic tools and resources. Our approach is based on measurement of the quantum Fisher information (QFI) as a witness of m-particle entanglement 8–10 , as familiar from quantum metrology 11–13 . As our main result, we will show that the QFI for thermodynamic equilibrium is directly related to measurement of dynamic susceptibilities (Fig. 1). To illustrate detection of entan-glement by means of the QFI, we study several examples of quan-tum phase transitions (QPTs). We are able to identify a class of strongly entangled QPTs with divergent multipartite entanglement by studying the universal scaling of the QFI (refs 14–17), also at non-zero temperatures (see also refs 18–20 for scaling of related quantum metrics). The entanglement quantified through the QFI is not only a resource for quantum metrology 8,9 , it also permits the characterization of exotic quantum effects such as many-body local-ization 21 . Although the outstanding feature of the presented protocol is its experimental simplicity, we will also discuss that the QFI as entanglement witness will be blind to non-local entanglement 22,23 , such as, for example, in topological systems. Background on the quantum Fisher information},
author = {Hauke, Philipp and Heyl, Markus and Tagliacozzo, Luca and Zoller, Peter},
doi = {10.1038/NPHYS3700},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hauke et al. - Unknown - Measuring multipartite entanglement through dynamic susceptibilities.pdf:pdf},
title = {{Measuring multipartite entanglement through dynamic susceptibilities}},
url = {http://www.nature.com/nphys/journal/v12/n8/pdf/nphys3700.pdf}
}
@article{Kalajdzievski2018,
abstract = {We propose a method for decomposing continuous-variable operations into a universal gate set, without the use of any approximations. We fully characterize a set of transformations admitting exact decompositions and describe a process for obtaining them systematically. Gates admitting these decompositions can be synthesized exactly, using circuits that are several orders of magnitude smaller than those achievable with previous methods. Our method relies on strategically using unitary conjugation and a lemma to the Baker-Campbell-Hausdorff formula to derive new exact decompositions from previously known ones, leading to exact decompositions for a large class of gates. We demonstrate the wide applicability of these exact gate decompositions by identifying several quantum algorithms and simulations of bosonic systems that can be implemented with higher precision and shorter circuit depths using our techniques.},
archivePrefix = {arXiv},
arxivId = {1811.10651},
author = {Kalajdzievski, Timjan and Arrazola, Juan Miguel},
eprint = {1811.10651},
file = {::},
month = {nov},
title = {{Exact gate decompositions for photonic quantum computing}},
url = {http://arxiv.org/abs/1811.10651},
year = {2018}
}
@article{Lopez-Incera2018,
abstract = {We study the effect of local decoherence on arbitrary quantum states. Adapting techniques developed in quantum metrology, we show that the action of generic local noise processes -though arbitrarily small- always yields a state whose Quantum Fisher Information (QFI) with respect to local observables is linear in system size N, independent of the initial state. This implies that all macroscopic quantum states, which are characterized by a QFI that is quadratic in N, are fragile under decoherence, and cannot be maintained if the system is not perfectly isolated. We also provide analytical bounds on the effective system size, and show that the effective system size scales as the inverse of the noise parameter p for small p, making it increasingly difficult to generate mesoscopic or even macroscopic quantum states. In turn, we also show that the preparation of a macroscopic quantum state, with respect to a conserved quantity, requires a device whose QFI is already at least as large as the one of the desired state. Given that the preparation device itself is classical and not a perfectly isolated macroscopic quantum state, the preparation device needs to be quadratically bigger than the macroscopic target state.},
archivePrefix = {arXiv},
arxivId = {1805.09868},
author = {L{\'{o}}pez-Incera, Andrea and Sekatski, Pavel and D{\"{u}}r, Wolfgang},
eprint = {1805.09868},
file = {::},
month = {may},
title = {{All macroscopic quantum states are fragile and hard to prepare}},
url = {http://arxiv.org/abs/1805.09868},
year = {2018}
}
@article{Arenz2016,
author = {Arenz, Christian and Burgarth, Daniel and Facchi, Paolo and Giovannetti, Vittorio and Nakazato, Hiromichi and Pascazio, Saverio and Yuasa, Kazuya},
doi = {10.1103/PhysRevA.93.062308},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Arenz et al. - 2016 - Universal control induced by noise.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {jun},
number = {6},
pages = {062308},
publisher = {American Physical Society},
title = {{Universal control induced by noise}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.93.062308},
volume = {93},
year = {2016}
}
@article{Zhou2017,
abstract = {Adiabatic processes are useful in quantum control, but they are slow. A way around this is to exploit shortcuts to adiabaticity, which can speed things up — for instance, by boosting stimulated Raman adiabatic passage.},
author = {Zhou, Brian B. and Baksic, Alexandre and Ribeiro, Hugo and Yale, Christopher G. and Heremans, F. Joseph and Jerger, Paul C. and Auer, Adrian and Burkard, Guido and Clerk, Aashish A. and Awschalom, David D.},
doi = {10.1038/nphys3967},
file = {::},
issn = {1745-2473},
journal = {Nat. Phys.},
keywords = {Quantum information,Qubits,Semiconductors,Spintronics},
month = {apr},
number = {4},
pages = {330--334},
publisher = {Nature Publishing Group},
title = {{Accelerated quantum control using superadiabatic dynamics in a solid-state lambda system}},
url = {http://www.nature.com/articles/nphys3967},
volume = {13},
year = {2017}
}
@article{Bennett2000,
author = {Bennett, Charles H. and DiVincenzo, David P.},
doi = {10.1038/35005001},
issn = {00280836},
journal = {Nature},
month = {mar},
number = {6775},
pages = {247--255},
publisher = {Nature Publishing Group},
title = {{Quantum information and computation}},
url = {http://www.nature.com/doifinder/10.1038/35005001},
volume = {404},
year = {2000}
}
@article{Deffner2013b,
abstract = {We derive a Margolus-Levitin-type bound on the minimal evolution time of an arbitrarily driven open quantum system. We express this quantum speed limit time in terms of the operator norm of the nonunitary generator of the dynamics. We apply these results to the damped Jaynes-Cummings model and demonstrate that the corresponding bound is tight. We further show that non-Markovian effects can speed up quantum evolution and therefore lead to a smaller quantum speed limit time.},
author = {Deffner, Sebastian and Lutz, Eric},
doi = {10.1103/PhysRevLett.111.010402},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Deffner, Lutz - Unknown - Quantum Speed Limit for Non-Markovian Dynamics.pdf:pdf},
journal = {Phys. Rev. Lett},
keywords = {0365Yz,PACS numbers},
pages = {010402},
title = {{Quantum Speed Limit for Non-Markovian Dynamics}},
url = {https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.111.010402},
volume = {111},
year = {2013}
}
@article{Funo2017a,
author = {Funo, Ken and Zhang, Jing-Ning and Chatou, Cyril and Kim, Kihwan and Ueda, Masahito and del Campo, Adolfo},
doi = {10.1103/PhysRevLett.118.100602},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Funo et al. - 2017 - Universal Work Fluctuations During Shortcuts to Adiabaticity by Counterdiabatic Driving(2).pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {10},
pages = {100602},
publisher = {American Physical Society},
title = {{Universal Work Fluctuations During Shortcuts to Adiabaticity by Counterdiabatic Driving}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.100602},
volume = {118},
year = {2017}
}
@article{Uzdin2016,
author = {Uzdin, Raam and Kosloff, Ronnie},
doi = {10.1209/0295-5075/115/40003},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uzdin, Kosloff - 2016 - Speed limits in Liouville space for open quantum systems.pdf:pdf},
issn = {0295-5075},
journal = {EPL (Europhysics Lett.},
month = {aug},
number = {4},
pages = {40003},
publisher = {IOP Publishing},
title = {{Speed limits in Liouville space for open quantum systems}},
url = {http://stacks.iop.org/0295-5075/115/i=4/a=40003?key=crossref.fb6c28939ede2f8745f2898a1d92c729},
volume = {115},
year = {2016}
}
@article{Coffman2000,
author = {Coffman, Valerie and Kundu, Joydip and Wootters, William K.},
doi = {10.1103/PhysRevA.61.052306},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Coffman, Kundu, Wootters - 2000 - Distributed entanglement.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {apr},
number = {5},
pages = {052306},
publisher = {American Physical Society},
title = {{Distributed entanglement}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.61.052306},
volume = {61},
year = {2000}
}
@inproceedings{Wiseman2003,
abstract = {Using an operational definition we quantify the entanglement, EP, between two parties who share an arbitrary pure state of N indistinguishable particles. We show that EP ≤ EM, where EM is the bipartite entanglement calculated from the mode-occupation representation. Unlike EM, EP is super-additive. For example, EP = 0 for any single-particle state, but the state |1?|1?, where both modes are split between the two parties, has EP = 1/2. We discuss how this relates to quantum correlations between particles, for both fermions and bosons.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0210002},
author = {Wiseman, H. and Vaccaro, John A},
booktitle = {2003 Eur. Quantum Electron. Conf. EQEC 2003},
doi = {10.1109/EQEC.2003.1314282},
eprint = {0210002},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wiseman, Vaccaro - 2003 - The entanglement of indistinguishable particles shared between two parties.pdf:pdf},
isbn = {0780377338},
issn = {0031-9007},
pages = {424},
pmid = {14525210},
primaryClass = {quant-ph},
title = {{The Entanglement of indistinguishable particles shared between two parties}},
year = {2003}
}
@article{Pfeifer1993,
abstract = {Lower and upper bounds are derived for the decay and transitions of quantum states, evolving under a time-dependent Hamiltonian, in terms of the energy uncertainty of the initial and final state. The bounds are simultaneously a rigorous version of Fermi's golden rule and of the time-energy uncertainty relation. They are sharp, refer to short times, and are compared with recent long-time results for time- independent Hamiltonians. Illustrations for tunneling systems, laser-driven processes, and neutron inter- ferometry in time-dependent magnetic fields are given.},
author = {Pfeifer, Peter},
doi = {10.1103/PhysRevLett.70.3365},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pfeifer - 1993 - How fast can a quantum state change with time.pdf:pdf},
issn = {00319007},
journal = {Phys. Rev. Lett.},
month = {may},
number = {22},
pages = {3365--3368},
publisher = {American Physical Society},
title = {{How fast can a quantum state change with time?}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.70.3365},
volume = {70},
year = {1993}
}
@article{Werner2001,
abstract = {We discuss general Bell inequalities for bipartite and multipartite systems, emphasizing the connection with convex geometry on the mathematical side, and the communication aspects on the physical side. Known results on families of generalized Bell inequalities are summarized. We investigate maximal violations of Bell inequalities as well as states not violating (certain) Bell inequalities. Finally, we discuss the relation between Bell inequality violations and entanglement properties currently discussed in quantum information theory.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0107093},
author = {Werner, Reinhard F. and Wolf, Michael M.},
eprint = {0107093},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Werner, Wolf - 2001 - Bell inequalities and Entanglement.pdf:pdf},
issn = {1533-7146},
journal = {Quantum Inf. Comput.},
keywords = {bell inequalities,entanglement,local hidden variable theories},
number = {3},
pages = {1--25},
primaryClass = {quant-ph},
publisher = {Rinton Press, Incorporated},
title = {{Bell inequalities and Entanglement}},
url = {http://arxiv.org/abs/quant-ph/0107093},
volume = {1},
year = {2001}
}
@inproceedings{Hollerer2007,
address = {New York, New York, USA},
author = {H{\"{o}}llerer, Tobias and Kuchera-Morin, JoAnn and Amatriain, Xavier},
booktitle = {Proc. 2007 Work. Emerg. displays Technol. images beyond Futur. displays Interact. - EDT '07},
doi = {10.1145/1278240.1278243},
isbn = {9781595936691},
pages = {3--es},
publisher = {ACM Press},
title = {{The allosphere}},
url = {http://dl.acm.org/citation.cfm?doid=1278240.1278243},
year = {2007}
}
@inproceedings{Deterding2011a,
address = {New York, New York, USA},
author = {Deterding, Sebastian and Dixon, Dan and Khaled, Rilla and Nacke, Lennart},
booktitle = {Proc. 15th Int. Acad. MindTrek Conf. Envisioning Futur. Media Environ. - MindTrek '11},
doi = {10.1145/2181037.2181040},
isbn = {9781450308168},
keywords = {alternate reality games,game-based technologies,gameful design,gamefulness,games,gamification,pervasive games,play,playful design,playfulness,serious games},
pages = {9},
publisher = {ACM Press},
title = {{From game design elements to gamefulness}},
url = {http://dl.acm.org/citation.cfm?doid=2181037.2181040},
year = {2011}
}
@article{Russell2016,
abstract = {Received (Day Month Year) Accepted (Day Month Year) Communicated by (xxxxxxxxxx) We study the maximum speed of quantum computation and how it is affected by limita-tions on physical resources. We show how the resulting concepts generalize to a broader class of physical models of computation within dynamical systems and introduce a spe-cific algebraic structure representing these speed limits. We derive a family of quantum speed limit results in resource-constrained quantum systems with pure states and a finite dimensional state space, by using a geometric method based on right invariant action functionals on SU (N). We show that when the action functional is bi-invariant, the minimum time for implementing any quantum gate using a potentially time-dependent Hamiltonian is equal to the minimum time when using a constant Hamiltonian, thus con-stant Hamiltonians are time optimal for these constraints. We give an explicit formula for the time in these cases, in terms of the resource constraint. We show how our method produces a rich family of speed limit results, of which the generalized Margolus–Levitin theorem and the Mandelstam–Tamm inequality are special cases. We discuss the broader context of geometric approaches to speed limits in physical computation, including the way geometric approaches to quantum speed limits are a model for physical speed limits to computation arising from a limited resource.},
author = {Russell, Benjamin and Stepney, Susan},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Russell, Stepney - 2016 - The Geometry of Speed Limiting Resources in Physical Models of Computation.pdf:pdf},
keywords = {Quantum Computation,Quantum Speed Limit},
title = {{The Geometry of Speed Limiting Resources in Physical Models of Computation}},
url = {https://arxiv.org/pdf/1611.09220.pdf},
year = {2016}
}
@article{Shanahan2018,
author = {Shanahan, B. and Chenu, A. and Margolus, N. and del Campo, A.},
doi = {10.1103/PhysRevLett.120.070401},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {7},
pages = {070401},
publisher = {American Physical Society},
title = {{Quantum Speed Limits across the Quantum-to-Classical Transition}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.070401},
volume = {120},
year = {2018}
}
@article{Tang2018,
author = {Tang, Yijun and Kao, Wil and Li, Kuan-Yu and Lev, Benjamin L.},
doi = {10.1103/PhysRevLett.120.230401},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Tang et al. - 2018 - Tuning the Dipole-Dipole Interaction in a Quantum Gas with a Rotating Magnetic Field.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jun},
number = {23},
pages = {230401},
publisher = {American Physical Society},
title = {{Tuning the Dipole-Dipole Interaction in a Quantum Gas with a Rotating Magnetic Field}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.230401},
volume = {120},
year = {2018}
}
@article{Matsuura2018,
abstract = {The accelerated progress in manufacturing noisy intermediate-scale quantum (NISQ) computing hardware has opened the possibility of exploring its application in transforming approaches to solving computationally challenging problems. The important limitations common among all NISQ computing technologies are the absence of error correction and the short coherence time, which limit the computational power of these systems. Shortening the required time of a single run of a quantum algorithm is essential for reducing environment-induced errors and for the efficiency of the computation. We have investigated the ability of a variational version of adiabatic quantum computation (AQC) to generate an accurate state more efficiently compared to existing adiabatic methods. The standard AQC method uses a time-dependent Hamiltonian, connecting the initial Hamiltonian with the final Hamiltonian. In the current approach, a navigator Hamiltonian is introduced which has a finite amplitude only in the middle of the annealing process. Both the initial and navigator Hamiltonians are determined using variational methods. The cluster operator of coupled-cluster theory, truncated to single and double excitations, is used as a navigator Hamiltonian. A comparative study of our variational algorithm (VanQver) with that of standard AQC, starting with a Hartree--Fock Hamiltonian, is presented. The results indicate that the introduction of the navigator Hamiltonian significantly improves the annealing time required to achieve chemical accuracy by two to three orders of magnitude. The efficiency of the method is demonstrated in the ground-state energy estimation of molecular systems, namely, H{\$}{\_}2{\$}, P4, and LiH.},
archivePrefix = {arXiv},
arxivId = {1810.11511},
author = {Matsuura, Shunji and Yamazaki, Takeshi and Senicourt, Valentin and Zaribafiyan, Arman},
eprint = {1810.11511},
file = {::},
month = {oct},
title = {{VanQver: The Variational and Adiabatically Navigated Quantum Eigensolver}},
url = {http://arxiv.org/abs/1810.11511},
year = {2018}
}
@article{Lee2018,
abstract = {We extend the work in New J. Phys. 19, 103015 (2017) by deriving a lower bound for the minimum time necessary to implement a unitary transformation on a generic, closed quantum system with an arbitrary number of classical control fields. This bound is explicitly analyzed for a specific N-level system similar to those used to represent simple models of an atom, or the first excitation sector of a Heisenberg spin chain, both of which are of interest in quantum control for quantum computation. Specifically, it is shown that the resultant bound depends on the dimension of the system, and on the number of controls used to implement a specific target unitary operation. The value of the bound determined numerically, and an estimate of the true minimum gate time are systematically compared for a range of system dimension and number of controls; special attention is drawn to the relationship between these two variables. It is seen that the bound captures the scaling of the minimum time well for the systems studied, and quantitatively is correct in the order of magnitude.},
archivePrefix = {arXiv},
arxivId = {1803.00027},
author = {Lee, Juneseo and Arenz, Christian and Rabitz, Herschel and Russell, Benjamin},
eprint = {1803.00027},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Lee et al. - 2018 - Dependence of the Quantum Speed Limit on System Size and Control Complexity.pdf:pdf},
month = {feb},
title = {{Dependence of the Quantum Speed Limit on System Size and Control Complexity}},
url = {http://arxiv.org/abs/1803.00027},
year = {2018}
}
@article{Krishnan2007,
author = {Krishnan, Shankar and Garimella, Suresh V. and Chrysler, Gregory M. and Mahajan, Ravi V.},
doi = {10.1109/TADVP.2007.898517},
issn = {1521-3323},
journal = {IEEE Trans. Adv. Packag.},
month = {aug},
number = {3},
pages = {462--474},
title = {{Towards a Thermal Moore's Law}},
url = {http://ieeexplore.ieee.org/document/4285937/},
volume = {30},
year = {2007}
}
@article{Kuk-HyunHan2002,
author = {{Kuk-Hyun Han} and {Jong-Hwan Kim}},
doi = {10.1109/TEVC.2002.804320},
issn = {1089-778X},
journal = {IEEE Trans. Evol. Comput.},
month = {dec},
number = {6},
pages = {580--593},
title = {{Quantum-inspired evolutionary algorithm for a class of combinatorial optimization}},
url = {http://ieeexplore.ieee.org/document/1134125/},
volume = {6},
year = {2002}
}
@article{Russell2014a,
abstract = {We are interested in fundamental limits to computation imposed by physical constraints. In particular, the physical laws of motion constrain the speed at which a computer can transition between well-defined states. Here, we discuss speed limits in the context of quantum computing. We review some relevant parts of the theory of Finsler metrics on Lie groups and homogeneous spaces such as the special unitary groups and complex projective spaces. We show how these constructions can be applied to analysing the limit to the speed of quantum information processing operations in constrained quantum systems with finite dimensional Hilbert spaces of states. We demonstrate the approach applied to a spin chain system.},
author = {Russell, Benjamin and Stepney, Susan},
doi = {10.1142/s0129054114400073},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Russell, Stepney - Unknown - APPLICATIONS OF FINSLER GEOMETRY TO SPEED LIMITS TO QUANTUM INFORMATION PROCESSING.pdf:pdf},
isbn = {0129-0541},
issn = {01290541},
journal = {Int. J. Found. Comput. Sci.},
keywords = {Finsler Geometric,Quan-tum Computing,Quantum Optimal Control,Quantum Speed Limit},
number = {4},
pages = {489--505},
title = {{Applications of Finsler Geometry to Speed Limits to Quantum Information Processing}},
url = {https://www-users.cs.york.ac.uk/susan/bib/ss/nonstd/ijfcs14.pdf},
volume = {25},
year = {2014}
}
@book{Bengtsson2008,
abstract = {Repr., with corrections. Originally published 2006.},
author = {Bengtsson, Ingemar. and Zyczkowski, Karol},
isbn = {052189140X},
pages = {419},
publisher = {Cambridge University Press},
title = {{Geometry of quantum states : an introduction to quantum entanglement}},
year = {2008}
}
@article{Assis2007,
abstract = {Recently Bender, Brody, Jones and Meister found that in the quantum brachistochrone problem the passage time needed for the evolution of certain initial states into specified final states can be made arbitrarily small, when the time-evolution operator is taken to be non-Hermitian but PT-symmetric. Here we demonstrate that such phenomena can also be obtained for non-Hermitian Hamiltonians for which PT-symmetry is completely broken, i.e. dissipative systems. We observe that the effect of a tunable passage time can be achieved by projecting between orthogonal eigenstates by means of a time-evolution operator associated to a non-Hermitian Hamiltonian. It is not essential that this Hamiltonian is PT-symmetric.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0703254},
author = {Assis, Paulo E. G. and Fring, Andreas},
doi = {10.1088/1751-8113/41/24/244002},
eprint = {0703254},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Assis, Fring - 2007 - The quantum brachistochrone problem for non-Hermitian Hamiltonians.pdf:pdf},
month = {mar},
primaryClass = {quant-ph},
title = {{The quantum brachistochrone problem for non-Hermitian Hamiltonians}},
url = {http://arxiv.org/abs/quant-ph/0703254 http://dx.doi.org/10.1088/1751-8113/41/24/244002},
year = {2007}
}
@article{Geiger,
abstract = {We develop a diagrammatic scattering theory for interacting bosons in a three-dimensional, weakly disordered potential. We show how collisional energy transfer between the bosons induces the thermalization of the inelastic single-particle current which, after only a few collision events, dominates over the elastic contribution described by the Gross-Pitaevskii ansatz.},
archivePrefix = {arXiv},
arxivId = {arXiv:1203.1722v3},
author = {Geiger, Tobias and Wellens, Thomas and Buchleitner, Andreas},
doi = {10.1103/PhysRevLett.109.030601},
eprint = {arXiv:1203.1722v3},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Geiger, Wellens, Buchleitner - Unknown - Inelastic Multiple Scattering of Interacting Bosons in Weak Random Potentials.pdf:pdf},
isbn = {1079-7114 (Electronic)$\backslash$r0031-9007 (Linking)},
issn = {00319007},
journal = {Phys. Rev. Lett.},
number = {3},
pmid = {22861833},
title = {{Inelastic multiple scattering of interacting bosons in weak random potentials}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.109.030601},
volume = {109},
year = {2012}
}
@article{Wang2015,
author = {Wang, Xiaoting and Allegra, Michele and Jacobs, Kurt and Lloyd, Seth and Lupo, Cosmo and Mohseni, Masoud},
doi = {10.1103/PhysRevLett.114.170501},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wang et al. - 2015 - Quantum Brachistochrone Curves as Geodesics Obtaining Accurate Minimum-Time Protocols for the Control of Quantum Sy.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {apr},
number = {17},
pages = {170501},
publisher = {American Physical Society},
title = {{Quantum Brachistochrone Curves as Geodesics: Obtaining Accurate Minimum-Time Protocols for the Control of Quantum Systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.114.170501},
volume = {114},
year = {2015}
}
@article{Andrecut2004,
author = {Andrecut, M and Ali, M K},
doi = {10.1088/0305-4470/37/34/L01},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Andrecut, Ali - 2004 - Adiabatic quantum oracles.pdf:pdf},
issn = {0305-4470},
journal = {J. Phys. A. Math. Gen.},
month = {aug},
number = {34},
pages = {L421--L427},
publisher = {IOP Publishing},
title = {{Adiabatic quantum oracles}},
url = {http://stacks.iop.org/0305-4470/37/i=34/a=L01?key=crossref.5f329da4deae79a729f75a948e880598},
volume = {37},
year = {2004}
}
@article{Jones2018,
author = {Jones, Nicola},
doi = {10.1038/d41586-018-06831-1},
issn = {0028-0836},
journal = {Nature},
month = {oct},
number = {7725},
pages = {S5--S7},
title = {{Simulated labs are booming}},
url = {http://www.nature.com/articles/d41586-018-06831-1},
volume = {562},
year = {2018}
}
@article{Chenu2017,
author = {Chenu, A. and Beau, M. and Cao, J. and del Campo, A.},
doi = {10.1103/PhysRevLett.118.140403},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Chenu et al. - 2017 - Quantum Simulation of Generic Many-Body Open System Dynamics Using Classical Noise.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {apr},
number = {14},
pages = {140403},
publisher = {American Physical Society},
title = {{Quantum Simulation of Generic Many-Body Open System Dynamics Using Classical Noise}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.118.140403},
volume = {118},
year = {2017}
}
@article{Kievsky1999,
abstract = {In order to improve the description of the N-d vector analyzing powers A y and iT 11 ͑the so-called A y puzzle͒ a spin-orbit three-body force has been introduced. The L • S term in the NN potential has been modified including a two-parameter three-body function depending on the hyperradius ␳. The modification has been performed in channels where the pair of nucleons (i, j) are coupled to spin S i j ϭ1 and isospin T i j ϭ1. Calcu-lations have been done in the energy region from E lab ϭ648 keV up to E lab ϭ10 MeV. A noticeable improve-ment in the description of the polarization observables has been obtained. ͓S0556-2813͑99͒03908-4͔ PACS number͑s͒: 21.30.Ϫx, 21.45.ϩv, 25.10.ϩs},
author = {Kievsky, A},
doi = {10.1103/PhysRevC.60.034001},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kievsky - Unknown - Phenomenological spin-orbit three-body force.pdf:pdf},
issn = {0556-2813},
journal = {Phys. Rev. C},
number = {3},
pages = {34001},
title = {{Phenomenological spin-orbit three-body force}},
url = {http://link.aps.org/doi/10.1103/PhysRevC.60.034001},
volume = {60},
year = {1999}
}
@article{Campbell2012,
author = {Campbell, Earl T. and Anwar, Hussain and Browne, Dan E.},
doi = {10.1103/PhysRevX.2.041021},
file = {::},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {dec},
number = {4},
pages = {041021},
publisher = {American Physical Society},
title = {{Magic-State Distillation in All Prime Dimensions Using Quantum Reed-Muller Codes}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.2.041021},
volume = {2},
year = {2012}
}
@article{Davis2000,
abstract = {Some new identities for quantum variance and covariance involv-ing commutators are presented, in which the density matrix and the operators are treated symmetrically. A measure of entanglement is proposed for bipartite systems, based upon covariance. This works for two-and three-component systems but produces ambiguities for multicomponent systems of composite diemnsion. Its relationship to angular momentum dispersion for symmetric spin states is described.},
archivePrefix = {arXiv},
arxivId = {arXiv:quant-ph/0001076v1},
author = {Davis, R I A and Delbourgo, R and Jarvis, P D},
eprint = {0001076v1},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Davis, Delbourgo, Jarvis - 2000 - COVARIANCE, CORRELATION AND ENTANGLEMENT(2).pdf:pdf},
primaryClass = {arXiv:quant-ph},
title = {{COVARIANCE, CORRELATION AND ENTANGLEMENT}},
url = {https://arxiv.org/pdf/quant-ph/0001076.pdf},
year = {2000}
}
@article{Campaioli2017,
abstract = {Can collective quantum effects make a difference in a meaningful thermodynamic operation? Focusing on energy storage and batteries, we demonstrate that quantum mechanics can lead to an enhancement in the amount of work deposited per unit time, i.e., the charging power, when {\$}N{\$} batteries are charged collectively. We first derive analytic upper bounds for the collective $\backslash$emph{\{}quantum advantage{\}} in charging power for two choices of constraints on the charging Hamiltonian. We then highlight the importance of entanglement by proving that the quantum advantage vanishes when the collective state of the batteries is restricted to be in the separable ball. Finally, we provide an upper bound to the achievable quantum advantage when the interaction order is restricted, i.e., at most {\$}k{\$} batteries are interacting. Our result is a fundamental limit on the advantage offered by quantum technologies over their classical counterparts as far as energy deposition is concerned.},
author = {Campaioli, Francesco and Pollock, Felix A. and Binder, Felix C. and C{\'{e}}leri, Lucas and Goold, John and Vinjanampathy, Sai and Modi, Kavan},
doi = {10.1103/PhysRevLett.118.150601},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli et al. - 2017 - Enhancing the Charging Power of Quantum Batteries(2).pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
month = {apr},
number = {15},
pages = {150601},
publisher = {American Physical Society},
title = {{Enhancing the Charging Power of Quantum Batteries}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.118.150601},
volume = {118},
year = {2017}
}
@article{Chin2012,
author = {Chin, Alex W. and Huelga, Susana F. and Plenio, Martin B.},
doi = {10.1103/PhysRevLett.109.233601},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Chin, Huelga, Plenio - 2012 - Quantum Metrology in Non-Markovian Environments.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {23},
pages = {233601},
publisher = {American Physical Society},
title = {{Quantum Metrology in Non-Markovian Environments}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.233601},
volume = {109},
year = {2012}
}
@article{Mondal2016b,
author = {Mondal, Debasis and Pati, Arun Kumar},
doi = {10.1016/J.PHYSLETA.2016.02.018},
issn = {0375-9601},
journal = {Phys. Lett. A},
month = {apr},
number = {16},
pages = {1395--1400},
publisher = {North-Holland},
title = {{Quantum speed limit for mixed states using an experimentally realizable metric}},
url = {http://www.sciencedirect.com/science/article/pii/S0375960116001559},
volume = {380},
year = {2016}
}
@article{Fischer2018,
abstract = {The Jaynes--Cummings system is one of the most fundamental models of how light and matter interact. When driving the system with a coherent state (e.g. laser light), it is often assumed that whether the light couples through the cavity or atom plays an important role in determining the dynamics of the system and its emitted field. Here, we prove that the dynamics are identical in either case except for the offset of a trivial coherent state. Further, this offset coherent state can be interferometrically canceled by appropriately homodyning the emitted light, which is especially important for nanocavity quantum electrodynamics where driving the atom is much more difficult than driving the cavity.},
archivePrefix = {arXiv},
arxivId = {1805.12248},
author = {Fischer, Kevin and Sun, Shuo and Lukin, Daniil and Kelaita, Yousif and Trivedi, Rahul and Vu{\v{c}}kovi{\'{c}}, Jelena},
eprint = {1805.12248},
file = {::},
month = {may},
title = {{Coherent drive in the Jaynes--Cummings model}},
url = {http://arxiv.org/abs/1805.12248},
year = {2018}
}
@article{Goold2016,
author = {Goold, John and Huber, Marcus and Riera, Arnau and del Rio, L{\'{i}}dia and Skrzypczyk, Paul},
doi = {10.1088/1751-8113/49/14/143001},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Goold et al. - 2016 - The role of quantum information in thermodynamics—a topical review.pdf:pdf},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {apr},
number = {14},
pages = {143001},
publisher = {IOP Publishing},
title = {{The role of quantum information in thermodynamics—a topical review}},
url = {http://stacks.iop.org/1751-8121/49/i=14/a=143001?key=crossref.ce80cac2171964cc6d6c51ed12d1e014},
volume = {49},
year = {2016}
}
@article{Brody2015,
abstract = {The quantum navigation problem of finding the time-optimal control Hamiltonian that transports a given initial state to a target state through quantum wind, that is, under the influence of external fields, is analysed. By lifting the problem from the state space to the space of unitary gates realising the required task, we are able to deduce the form of the solution to the problem by deriving a universal quantum speed limit. The expression thus obtained indicates that further simplifications of this apparently difficult problem are possible if we switch to the interaction picture of quantum mechanics. A complete solution to the navigation problem for an arbitrary quantum system is then obtained, and the behaviour of the solution is illustrated in the case of a two-level system.},
author = {Brody, Dorje C and Gibbons, Gary W and Meier, David M},
doi = {10.1088/1367-2630/17/3/033048},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Brody, Gibbons, Meier - 2015 - Time-optimal navigation through quantum wind.pdf:pdf},
issn = {13672630},
journal = {New J. Phys.},
keywords = {Controlled quantum dynamics,Finsler geometry,Zermelo navigation},
month = {mar},
number = {3},
pages = {1--8},
publisher = {IOP Publishing},
title = {{Time-optimal navigation through quantum wind}},
url = {http://iopscience.iop.org/article/10.1088/1367-2630/17/3/033048/meta},
volume = {17},
year = {2015}
}
@article{Provost1980,
abstract = {A metric tensor is defined from the underlying Hubert space structure for any submanifold of quantum states. The case where the manifold is generated by the action of a Lie group on a fixed state vector (generalized coherent states manifold hereafter noted G.C.S.M.) is studied in details; the geometrical properties of some wellknown G.C.S.M. are reviewed and an explicit expression for the scalar Riemannian curvature is given in the general case. The physical meaning of such Riemannian structures (which have been recently introduced to describe collective manifolds in nuclear physics) is discussed. It is shown on examples that the distance between nearby states is related to quantum fluctuations; in the particular case of the harmonic oscillator group the condition of zero curvature appears to be identical to that of non dispersion of wave packets.},
author = {Provost, J P and Vallee, G},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Provost, Vallee - 1980 - Riemannian Structure on Manifolds of Quantum States.pdf:pdf},
journal = {Commun. Commun. Math. Phys. Math. Phys.},
pages = {289--301},
title = {{Riemannian Structure on Manifolds of Quantum States}},
url = {http://projecteuclid.org.ezproxy.lib.monash.edu.au/download/pdf{\_}1/euclid.cmp/1103908308},
volume = {76},
year = {1980}
}
@article{Pfeifer1995,
author = {Pfeifer, Peter and Fr{\"{o}}hlich, J{\"{u}}rg},
doi = {10.1103/RevModPhys.67.759},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pfeifer, Fr{\"{o}}hlich - 1995 - Generalized time-energy uncertainty relations and bounds on lifetimes of resonances.pdf:pdf},
issn = {0034-6861},
journal = {Rev. Mod. Phys.},
month = {oct},
number = {4},
pages = {759--779},
publisher = {American Physical Society},
title = {{Generalized time-energy uncertainty relations and bounds on lifetimes of resonances}},
url = {https://link.aps.org/doi/10.1103/RevModPhys.67.759},
volume = {67},
year = {1995}
}
@article{Schliemann,
abstract = {We characterize and classify quantum correlations in two-fermion systems having 2K single-particle states. For pure states we introduce the Slater decomposition and rank (in analogy to Schmidt decomposition and rank), i.e. we decompose the state into a combination of elementary Slater determinants formed by mutually orthogonal single-particle states. Mixed states can be characterized by their Slater number which is the minimal Slater rank required to generate them. For K=2 we give a necessary and sufficient condition for a state to have a Slater number of 1. We introduce a correlation measure for mixed states which can be evaluated analytically for K=2. For higher K, we provide a method of constructing and optimizing Slater number witnesses, i.e. operators that detect Slater number for some states.},
archivePrefix = {arXiv},
arxivId = {quant-ph/0012094},
author = {Schliemann, John and Cirac, J Ignacio and Kus, Marek and Lewenstein, Maciej and Loss, Daniel},
doi = {10.1103/PhysRevA.64.022303},
eprint = {0012094},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Schliemann et al. - Unknown - Quantum correlations in two-fermion systems.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
keywords = {0365Ta,8970ϩc,PACS number͑s͒},
pages = {9},
primaryClass = {quant-ph},
title = {{Quantum Correlations in Two-Fermion Systems}},
url = {http://arxiv.org/abs/quant-ph/0012094},
volume = {64},
year = {2000}
}
@article{Ektesabi2017,
author = {Ektesabi, Abbas and Behzadi, Naghi and Faizi, Esfandyar},
doi = {10.1103/PhysRevA.95.022115},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ektesabi, Behzadi, Faizi - 2017 - Improved bound for quantum-speed-limit time in open quantum systems by introducing an alternative fide.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {feb},
number = {2},
pages = {022115},
publisher = {American Physical Society},
title = {{Improved bound for quantum-speed-limit time in open quantum systems by introducing an alternative fidelity}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.95.022115},
volume = {95},
year = {2017}
}
@article{Debnath2016,
author = {Debnath, S. and Linke, N. M. and Figgatt, C. and Landsman, K. A. and Wright, K. and Monroe, C.},
doi = {10.1038/nature18648},
issn = {0028-0836},
journal = {Nature},
number = {7614},
pages = {63--66},
publisher = {Nature Research},
title = {{Demonstration of a small programmable quantum computer with atomic qubits}},
url = {http://www.nature.com/doifinder/10.1038/nature18648},
volume = {536},
year = {2016}
}
@article{GiuliaCampa,
author = {Campaioli, Giulia and Sale, Eleonora and Simonelli, Alessandra and Pomini, Valeria},
doi = {10.1007/s10591-017-9443-9},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli et al. - 2017 - The Dual Value of the Web Risks and Benefits of the Use of the Internet in Disorders with A Self-Destructive C.pdf:pdf},
issn = {0892-2764},
journal = {Contemp. Fam. Ther.},
month = {dec},
number = {4},
pages = {301--313},
publisher = {Springer US},
title = {{The Dual Value of the Web: Risks and Benefits of the Use of the Internet in Disorders with A Self-Destructive Component in Adolescents and Young Adults}},
url = {http://link.springer.com/10.1007/s10591-017-9443-9},
volume = {39},
year = {2017}
}
@article{Ho2005,
author = {Ho, Choon-Lin and Lee, Chung-Chieh},
doi = {10.1103/PhysRevA.71.012102},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ho, Lee - 2005 - Stabilizing quantum metastable states in a time-periodic potential.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jan},
number = {1},
pages = {012102},
publisher = {American Physical Society},
title = {{Stabilizing quantum metastable states in a time-periodic potential}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.71.012102},
volume = {71},
year = {2005}
}
@article{Pollock2016,
author = {Pollock, Felix A. and Ch{\c{e}}ci{\'{n}}ska, Agata and Pascazio, Saverio and Modi, Kavan},
doi = {10.1103/PhysRevA.94.032112},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pollock et al. - 2016 - Using a biased qubit to probe complex systems.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {032112},
publisher = {American Physical Society},
title = {{Using a biased qubit to probe complex systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.94.032112},
volume = {94},
year = {2016}
}
@article{Ferraro2018,
archivePrefix = {arXiv},
arxivId = {1707.04930},
author = {Ferraro, Dario and Campisi, Michele and Andolina, Gian Marcello and Pellegrini, Vittorio and Polini, Marco},
doi = {10.1103/PhysRevLett.120.117702},
eprint = {1707.04930},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ferraro et al. - 2018 - High-Power Collective Charging of a Solid-State Quantum Battery(2).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ferraro et al. - 2018 - High-Power Collective Charging of a Solid-State Quantum Battery.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ferraro et al. - Unknown - High-power collective charging of a solid-state quantum battery.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {11},
pages = {117702},
publisher = {American Physical Society},
title = {{High-Power Collective Charging of a Solid-State Quantum Battery}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.117702 https://arxiv.org/pdf/1707.04930.pdf http://arxiv.org/abs/1707.04930},
volume = {120},
year = {2018}
}
@article{Taddei2013,
abstract = {The evaluation of the minimal evolution time between two distinguishable states of a system is important for assessing the maximal speed of quantum computers and communication channels. Lower bounds for this minimal time have been proposed for unitary dynamics. Here we show that it is possible to extend this concept to nonunitary processes, using an attainable lower bound that is connected to the quantum Fisher information for time estimation. This result is used to delimit the minimal evolution time for typical noisy channels.},
author = {Taddei, M. M. and Escher, B. M. and Davidovich, L. and {De Matos Filho}, R. L.},
doi = {10.1103/PhysRevLett.110.050402},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Taddei et al. - Unknown - Quantum Speed Limit for Physical Processes.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Taddei et al. - 2013 - Quantum Speed Limit for Physical Processes(3).pdf:pdf},
isbn = {9781557529787},
issn = {00319007},
journal = {Phys. Rev. Lett.},
month = {jan},
number = {5},
pages = {050402},
publisher = {American Physical Society},
title = {{Quantum speed limit for physical processes}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.050402 https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.110.050402},
volume = {110},
year = {2013}
}
@article{Giovannetti2003a,
abstract = {We establish the minimum time it takes for an initial state of mean energy E and energy spread ∆E to move from its initial configuration by a predetermined amount. Distances in Hilbert space are estimated by the fidelity between the initial and final state. In this context, we also show that entanglement is necessary to achieve the ultimate evolution speed when the energy resources are distributed among all subsystems.},
author = {Giovannetti, Vittorio and Lloyd, Seth and Maccone, Lorenzo},
doi = {10.1103/PhysRevA.67.052109},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Giovannetti, Lloyd, Maccone - 2003 - Quantum limits to dynamical evolution.pdf:pdf},
isbn = {1050-2947$\backslash$r1094-1622},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {may},
number = {5},
pages = {1--8},
publisher = {American Physical Society},
title = {{Quantum limits to dynamical evolution}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.67.052109},
volume = {67},
year = {2003}
}
@book{Fuchs1997,
author = {Fuchs, Jürgen and Schweigert, Christoph.},
isbn = {9780521560016},
pages = {438},
publisher = {Cambridge University Press},
title = {{Symmetries, lie algebras and representations : a graduate course for physicists}},
year = {1997}
}
@article{Zyczkowski2011,
abstract = {We study various methods to generate ensembles of random density matrices of a fixed size N , obtained by partial trace of pure states on composite systems. Structured ensembles of random pure states, invariant with respect to local unitary transformations are introduced. To analyze statistical properties of quantum entanglement in bi-partite systems we analyze the distribution of Schmidt coefficients of random pure states. Such a distribution is derived in the case of a superposition of k random maximally entangled states. For another ensemble, obtained by performing selective measurements in a maximally entangled basis on a multi–partite system, we show that this distri-bution is given by the Fuss-Catalan law and find the average entanglement entropy. A more general class of structured ensembles proposed, containing also the case of Bures, forms an extension of the standard ensemble of structureless random pure states, described asymptotically, as N → ∞, by the Marchenko-Pastur distribution.},
archivePrefix = {arXiv},
arxivId = {arXiv:1010.3570v2},
author = {Zyczkowski, Karol ˙ and Penson, Karol A and Nechita, Ion and Collins, Benot},
eprint = {arXiv:1010.3570v2},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zyczkowski et al. - 2011 - Generating random density matrices.pdf:pdf},
keywords = {()},
title = {{Generating random density matrices}},
url = {https://arxiv.org/pdf/1010.3570.pdf},
year = {2011}
}
@article{Bennett2002,
author = {Bennett, C.H. and Shor, P.W. and Smolin, J.A. and Thapliyal, A.V.},
doi = {10.1109/TIT.2002.802612},
issn = {0018-9448},
journal = {IEEE Trans. Inf. Theory},
number = {10},
pages = {2637--2655},
title = {{Entanglement-assisted capacity of a quantum channel and the reverse Shannon theorem}},
url = {http://ieeexplore.ieee.org/document/1035117/},
volume = {48},
year = {2002}
}
@article{Keyl2001,
author = {Keyl, M. and Werner, R. F.},
doi = {10.1103/PhysRevA.64.052311},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Keyl, Werner - 2001 - Estimating the spectrum of a density operator.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {oct},
number = {5},
pages = {052311},
publisher = {American Physical Society},
title = {{Estimating the spectrum of a density operator}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.64.052311},
volume = {64},
year = {2001}
}
@article{Pashkin2009,
abstract = {The field of solid-state quantum computation is expanding rapidly initi-ated by our original charge qubit demonstrations. Various types of solid-state qubits are being studied, and their coherent properties are improving. The goal of this review is to summarize achievements on Josephson charge qubits. We cover the results obtained in our joint group of NEC Nano Electronics Research Laboratories and RIKEN Advanced Science Institute, also referring to the works done by other groups. Starting from a short introduction, we describe the principle of the Josephson charge qubit, its manipulation and readout. We proceed with coupling of two charge qubits and implementation of a logic gate. We also discuss decoherence issues. Finally, we show how a charge qubit can be used as an artificial atom coupled to a resonator to demonstrate lasing action.},
author = {Pashkin, Yu A and Astafiev, O and Yamamoto, T and Nakamura, Y and Tsai, J S},
doi = {10.1007/s11128-009-0101-5},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pashkin et al. - 2009 - Josephson charge qubits a brief review.pdf:pdf},
journal = {Quantum Inf Process},
keywords = {Artificial atom {\textperiodcentered},Cooper pair box {\textperiodcentered},Cp {\textperiodcentered} 8535,Decoherence {\textperiodcentered},Dephasing {\textperiodcentered},Energy relaxation {\textperiodcentered},Gv,Hk {\textperiodcentered} 8525,Josephson charge qubit {\textperiodcentered},Lasing PACS 0365,Lx {\textperiodcentered} 4250,Pq {\textperiodcentered} 7323,Quantum coherence {\textperiodcentered},Quantum logic gate {\textperiodcentered},Quantum state manipulation {\textperiodcentered},Single-shot readout {\textperiodcentered},Yz {\textperiodcentered} 0367},
pages = {55--80},
title = {{Josephson charge qubits: a brief review}},
url = {https://link.springer.com/content/pdf/10.1007{\%}2Fs11128-009-0101-5.pdf},
volume = {8},
year = {2009}
}
@article{Meier2012,
abstract = {The distillation of magic states is an often-cited technique for enabling universal quantum computing once the error probability for a special subset of gates has been made negligible by other means. We present a routine for magic-state distillation that reduces the required overhead for a range of parameters of practical interest. Each iteration of the routine uses a four-qubit error-detecting code to distill the +1 eigenstate of the Hadamard gate at a cost of ten input states per two improved output states. Use of this routine in combination with the 15-to-1 distillation routine described by Bravyi and Kitaev allows for further improvements in overhead.},
archivePrefix = {arXiv},
arxivId = {1204.4221},
author = {Meier, Adam M. and Eastin, Bryan and Knill, Emanuel},
eprint = {1204.4221},
file = {::},
month = {apr},
title = {{Magic-state distillation with the four-qubit code}},
url = {http://arxiv.org/abs/1204.4221},
year = {2012}
}
@article{Giovannetti2011,
author = {Giovannetti, Vittorio and Lloyd, Seth and Maccone, Lorenzo},
doi = {10.1038/nphoton.2011.35},
issn = {1749-4885},
journal = {Nat. Photonics},
month = {apr},
number = {4},
pages = {222--229},
publisher = {Nature Research},
title = {{Advances in quantum metrology}},
url = {http://www.nature.com/doifinder/10.1038/nphoton.2011.35},
volume = {5},
year = {2011}
}
@article{Taranto2018,
archivePrefix = {arXiv},
arxivId = {1805.11341},
author = {Taranto, Philip and Pollock, Felix A. and Milz, Simon and Tomamichel, Marco and Modi, Kavan},
eprint = {1805.11341},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Taranto et al. - 2018 - Quantum Markov Order.pdf:pdf},
month = {may},
title = {{Quantum Markov Order}},
url = {https://arxiv.org/abs/1805.11341},
year = {2018}
}
@article{Zielinski2006,
author = {Zieli{\'{n}}ski, Bartosz and Zych, Magdalena},
doi = {10.1103/PhysRevA.74.034301},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Zieli{\'{n}}ski, Zych - 2006 - Generalization of the Margolus-Levitin bound.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {sep},
number = {3},
pages = {034301},
publisher = {American Physical Society},
title = {{Generalization of the Margolus-Levitin bound}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.74.034301},
volume = {74},
year = {2006}
}
@article{Vedral2018,
abstract = {We are building machines to undermine nature's most rigid rule, says physicist Vlatko Vedral},
author = {Vedral, Vlatko},
doi = {10.1016/S0262-4079(18)30616-X},
issn = {0262-4079},
journal = {New Sci.},
month = {apr},
number = {3172},
pages = {32--35},
publisher = {Reed Business Information},
title = {{Law and Disorder}},
url = {https://www.sciencedirect.com/science/article/pii/S026240791830616X},
volume = {237},
year = {2018}
}
@article{Duty2004,
author = {Duty, T. and Gunnarsson, D. and Bladh, K. and Delsing, P.},
doi = {10.1103/PhysRevB.69.140503},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Duty et al. - 2004 - Coherent dynamics of a Josephson charge qubit.pdf:pdf},
issn = {1098-0121},
journal = {Phys. Rev. B},
month = {apr},
number = {14},
pages = {140503},
publisher = {American Physical Society},
title = {{Coherent dynamics of a Josephson charge qubit}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.69.140503},
volume = {69},
year = {2004}
}
@article{Epstein,
abstract = {We derive algebraic bounds on achievable rates for quantum state transfer and entanglement generation in general quantum systems. We apply these bounds to graph-based models of local quantum spin systems to obtain speed limits on these tasks. Comparison with numerical optimal control results for spin chains suggests that unexplored regions of the dynamical landscape may support enhanced performance of key quantum information processing tasks.},
author = {Epstein, Jeffrey M and Whaley, K Birgitta},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Epstein, Whaley - Unknown - Quantum Speed Limits for Quantum Information Processing Tasks.pdf:pdf},
title = {{Quantum Speed Limits for Quantum Information Processing Tasks}}
}
@article{Giorgi2015,
author = {Giorgi, Gian Luca and Campbell, Steve},
doi = {10.1088/0953-4075/48/3/035501},
issn = {0953-4075},
journal = {J. Phys. B At. Mol. Opt. Phys.},
month = {feb},
number = {3},
pages = {035501},
publisher = {IOP Publishing},
title = {{Correlation approach to work extraction from finite quantum systems}},
url = {http://stacks.iop.org/0953-4075/48/i=3/a=035501?key=crossref.2043d6eca0172484e09dab3acd00e547},
volume = {48},
year = {2015}
}
@article{Hegerfeldt2013,
author = {Hegerfeldt, Gerhard C.},
doi = {10.1103/PhysRevLett.111.260501},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Hegerfeldt - 2013 - Driving at the Quantum Speed Limit Optimal Control of a Two-Level System.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {26},
pages = {260501},
publisher = {American Physical Society},
title = {{Driving at the Quantum Speed Limit: Optimal Control of a Two-Level System}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.111.260501},
volume = {111},
year = {2013}
}
@article{Mingo2018,
abstract = {In this chapter we address the topic of quantum thermodynamics in the presence of additional observables beyond the energy of the system. In particular we discuss the special role that the generalized Gibbs ensemble plays in this theory, and derive this state from the perspectives of a micro-canonical ensemble, dynamical typicality and a resource-theory formulation. A notable obstacle occurs when some of the observables do not commute, and so it is impossible for the observables to simultaneously take on sharp microscopic values. We show how this can be circumvented, discuss information-theoretic aspects of the setting, and explain how thermodynamic costs can be traded between the different observables. Finally, we discuss open problems and future directions for the topic.},
archivePrefix = {arXiv},
arxivId = {1806.08325},
author = {Mingo, Erick Hinds and Guryanova, Yelena and Faist, Philippe and Jennings, David},
eprint = {1806.08325},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Mingo et al. - 2018 - Quantum thermodynamics with multiple conserved quantities.pdf:pdf},
month = {jun},
title = {{Quantum thermodynamics with multiple conserved quantities}},
url = {http://arxiv.org/abs/1806.08325},
year = {2018}
}
@article{Bertlmann2008,
author = {Bertlmann, Reinhold A and Krammer, Philipp},
doi = {10.1088/1751-8113/41/23/235303},
file = {::},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {jun},
number = {23},
pages = {235303},
publisher = {IOP Publishing},
title = {{Bloch vectors for qudits}},
url = {http://stacks.iop.org/1751-8121/41/i=23/a=235303?key=crossref.3502dcae736ba306771a3520bf06acb2},
volume = {41},
year = {2008}
}
@article{Ekert1992,
author = {Ekert, Artur K. and Rarity, John G. and Tapster, Paul R. and {Massimo Palma}, G.},
doi = {10.1103/PhysRevLett.69.1293},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ekert et al. - 1992 - Practical quantum cryptography based on two-photon interferometry.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {aug},
number = {9},
pages = {1293--1295},
publisher = {American Physical Society},
title = {{Practical quantum cryptography based on two-photon interferometry}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.69.1293},
volume = {69},
year = {1992}
}
@article{Bourin2012,
author = {Bourin, Jean-Christophe and Lee, Eun-Young},
doi = {10.1112/blms/bds080},
issn = {00246093},
journal = {Bull. London Math. Soc.},
month = {dec},
number = {6},
pages = {1085--1102},
publisher = {Oxford University Press (OUP)},
title = {{Unitary orbits of Hermitian operators with convex or concave functions}},
url = {http://doi.wiley.com/10.1112/blms/bds080},
volume = {44},
year = {2012}
}
@article{Gislason1985,
author = {Gislason, Eric A. and Sabelli, Nora H. and Wood, John W.},
doi = {10.1103/PhysRevA.31.2078},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gislason, Sabelli, Wood - 1985 - New form of the time-energy uncertainty relation.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gislason, Sabelli, Wood - 1985 - New form of the time-energy uncertainty relation(2).pdf:pdf},
issn = {10502947},
journal = {Phys. Rev. A},
month = {apr},
number = {4},
pages = {2078--2081},
publisher = {American Physical Society},
title = {{New form of the time-energy uncertainty relation}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.31.2078},
volume = {31},
year = {1985}
}
@article{Marvian2016,
author = {Marvian, Iman and Spekkens, Robert W. and Zanardi, Paolo},
doi = {10.1103/PhysRevA.93.052331},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Marvian, Spekkens, Zanardi - 2016 - Quantum speed limits, coherence, and asymmetry.pdf:pdf},
issn = {2469-9926},
journal = {Phys. Rev. A},
month = {may},
number = {5},
pages = {052331},
publisher = {American Physical Society},
title = {{Quantum speed limits, coherence, and asymmetry}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.93.052331},
volume = {93},
year = {2016}
}
@article{Gombosi1999,
abstract = {NATURE | VOL 412 | 26 JULY 2001 | www.nature.com 417 26. Raeder, J. Modeling the magnetosphere for northward interplanetary magnetic {\textregistered}eld: Effects of electrical resistivity.},
author = {Gombosi, T I and Dezeeuw, D L and Groth, C P T and Powell, K G and Song, P and Sonnerup, B U and O, {\`{E}} and Cahill, L J},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gombosi et al. - 1999 - letters to nature.pdf:pdf},
journal = {J. Geophys. Res. Phys. Sp. Plasmas J. Geophys. Res},
number = {72},
pages = {17357--17368},
publisher = {MIT Press},
title = {letters to nature},
url = {https://www.nature.com/nature/journal/v412/n6845/pdf/412417a0.pdf},
volume = {104},
year = {1999}
}
@article{Modi2011,
author = {Modi, Kavan and Cable, Hugo and Williamson, Mark and Vedral, Vlatko},
doi = {10.1103/PhysRevX.1.021022},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Modi et al. - 2011 - Quantum Correlations in Mixed-State Metrology.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Modi et al. - 2011 - Quantum Correlations in Mixed-State Metrology(2).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Modi et al. - 2011 - Quantum Correlations in Mixed-State Metrology(3).pdf:pdf},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {dec},
number = {2},
pages = {021022},
publisher = {American Physical Society},
title = {{Quantum Correlations in Mixed-State Metrology}},
url = {http://link.aps.org/doi/10.1103/PhysRevX.1.021022 https://link.aps.org/doi/10.1103/PhysRevX.1.021022},
volume = {1},
year = {2011}
}
@article{DelCampo2013,
author = {del Campo, A. and Egusquiza, I. L. and Plenio, M. B. and Huelga, S. F.},
doi = {10.1103/PhysRevLett.110.050403},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/del Campo et al. - 2013 - Quantum Speed Limits in Open System Dynamics.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/del Campo et al. - 2013 - Quantum Speed Limits in Open System Dynamics(2).pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jan},
number = {5},
pages = {050403},
publisher = {American Physical Society},
title = {{Quantum Speed Limits in Open System Dynamics}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.050403 http://link.aps.org/doi/10.1103/PhysRevLett.110.050403},
volume = {110},
year = {2013}
}
@article{Arrazola2018,
abstract = {We show how techniques from machine learning and optimization can be used to find circuits of photonic quantum computers that perform a desired transformation between input and output states. In the simplest case of a single input state, our method discovers circuits for preparing a desired quantum state. In the more general case of several input and output relations, our method obtains circuits that reproduce the action of a target unitary transformation. We use a continuous-variable quantum neural network as the circuit architecture. The network is composed of several layers of optical gates with variable parameters that are optimized by applying automatic differentiation using the TensorFlow backend of the Strawberry Fields photonic quantum computer simulator. We demonstrate the power and versatility of our methods by learning how to use short-depth circuits to synthesize single photons, Gottesman-Kitaev-Preskill states, NOON states, cubic phase gates, random unitaries, cross-Kerr interactions, as well as several other states and gates. We routinely obtain high fidelities above 99$\backslash${\%} using short-depth circuits, typically consisting of a few hundred gates. The circuits are obtained automatically by simply specifying the target state or gate and running the optimization algorithm.},
archivePrefix = {arXiv},
arxivId = {1807.10781},
author = {Arrazola, Juan Miguel and Bromley, Thomas R. and Izaac, Josh and Myers, Casey R. and Br{\'{a}}dler, Kamil and Killoran, Nathan},
eprint = {1807.10781},
file = {::},
month = {jul},
title = {{Machine learning method for state preparation and gate synthesis on photonic quantum computers}},
url = {http://arxiv.org/abs/1807.10781},
year = {2018}
}
@article{Kelkar2017,
abstract = {Tunneling is one of the most bizarre phenomena in quantum mechanics. An attempt to understand it led to the next natural question of how long does a particle need to tunnel a barrier. The latter gave rise to several definitions such as the phase, dwell, Larmor and traversal times among others. A short review of the evolution of these time concepts, followed by an account of experiments involving field-induced tunnel ionization and electron tunneling in a solid state junction is presented here. Whereas the former experiments use sophisticated techniques involving femtosecond laser pulses and determine the tunneling time by mapping the angle of rotation of the field vector to time, like the hands of a watch, the latter provides a simpler method through the measurement of current-voltage characteristics of the junction.},
archivePrefix = {arXiv},
arxivId = {1708.05101},
author = {Kelkar, N. G.},
eprint = {1708.05101},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Kelkar - 2017 - Electron tunneling times.pdf:pdf},
month = {aug},
title = {{Electron tunneling times}},
url = {http://arxiv.org/abs/1708.05101},
year = {2017}
}
@article{Perez-Garcia2006,
abstract = {We provide a complete picture of contractivity of trace preserving positive maps with respect to p-norms. We show that for p{\textgreater}1 contractivity holds in general if and only if the map is unital. When the domain is restricted to the traceless subspace of Hermitian matrices, then contractivity is shown to hold in the case of qubits for arbitrary p⩾1 and in the case of qutrits if and only if p=1, ∞. In all noncontractive cases best possible bounds on the p-norms are derived.},
author = {P{\'{e}}rez-Garc{\'{i}}a, David and Wolf, Michael M. and Petz, Denes and Ruskai, Mary Beth},
doi = {10.1063/1.2218675},
file = {::},
issn = {0022-2488},
journal = {J. Math. Phys.},
keywords = {Hermitian matrices},
month = {aug},
number = {8},
pages = {083506},
publisher = {American Institute of Physics},
title = {{Contractivity of positive and trace-preserving maps under Lp norms}},
url = {http://aip.scitation.org/doi/10.1063/1.2218675},
volume = {47},
year = {2006}
}
@inproceedings{Hamari2014a,
abstract = {This paper reviews peer-reviewed empirical studies on gamification. We create a framework for examining the effects of gamification by drawing from the definitions of gamification and the discussion on motivational affordances. The literature review covers results, independent variables (examined motivational affordances), dependent variables (examined psychological/behavioral outcomes from gamification), the contexts of gamification, and types of studies performed on the gamified systems. The paper examines the state of current research on the topic and points out gaps in existing literature. The review indicates that gamification provides positive effects, however, the effects are greatly dependent on the context in which the gamification is being implemented, as well as on the users using it. The findings of the review provide insight for further studies as well as for the design of gamified systems.},
author = {Hamari, Juho and Koivisto, Jonna and Sarsa, Harri},
booktitle = {2014 47th Hawaii Int. Conf. Syst. Sci.},
doi = {10.1109/HICSS.2014.377},
file = {::},
isbn = {978-1-4799-2504-9},
keywords = {Context,Databases,Educational institutions,Games,HCI,Libraries,Psychology,gamification,motivation,motivational affordance,persuasive technology},
month = {jan},
pages = {3025--3034},
publisher = {IEEE},
title = {{Does Gamification Work? -- A Literature Review of Empirical Studies on Gamification}},
url = {http://ieeexplore.ieee.org/document/6758978/},
year = {2014}
}
@article{Bauer1978,
author = {Bauer, M and Mello, P.A},
doi = {10.1016/0003-4916(78)90223-3},
issn = {00034916},
journal = {Ann. Phys. (N. Y).},
month = {mar},
number = {1},
pages = {38--60},
title = {{The time-energy uncertainty relation}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0003491678902233},
volume = {111},
year = {1978}
}
@article{Grover1997,
abstract = {Quantum mechanics can speed up a range of search applications over unsorted data. For example, imagine a phone directory containing N names arranged in completely random order. To find some-one's phone number with a probability of 50{\%}, any classical algorithm (whether deterministic or proba-bilistic) will need to access the database a minimum of 0.5N times. Quantum mechanical systems can be in a superposition of states and simultaneously examine multiple names. By properly adjusting the phases of various operations, successful computations reinforce each other while others interfere ran-domly. As a result, the desired phone number can be obtained in only O͑ p N ͒ accesses to the database. [S0031-9007(97)03564-3] PACS numbers: 89.70. + c, 03.65. – w In 1994 Shor discovered a quantum mechanical algo-rithm for factorization that was exponentially faster than any known classical algorithm [1]. This Letter presents a quantum mechanical algorithm for search that is only polynomially faster than any classical algorithm; however, it does not depend for its impact on the unproven diffi-culty of the factorization problem. The search problem is this: there is an unsorted database containing N items out of which just one item satisfies a given condition—that one item has to be retrieved. Once an item is examined, it is possible to tell whether or not it satisfies the condition in one step. However, there does not exist any sorting on the database that would aid its selection. The most effi-cient classical algorithm for this is to examine the items in the database one by one. If an item satisfies the required condition, stop; if it does not, keep track of this item so that it is not examined again. It is easily seen that this algorithm will need to examine an average of 0.5N items before finding the desired item. It is possible for quantum mechanical systems to make interaction-free measurements by using the duality properties of photons [2]. In these the presence (or absence) of an object can be deduced by allowing a small probability of a photon interacting with the object. Therefore, most probably the photon will not interact; however, just allowing a small probability of interaction is enough to make the measurement. Thus in the search problem also, it might be possible to find the object without examining all of the objects, but just by allowing a certain probability of examining the desired object. Indeed, this Letter shows that by using the same amount of hardware as in the classical case, but by having the input and output in superpositions of states, we can find an object in O͑ p N ͒ quantum mechanical steps instead of O͑N͒ classical steps. Each quantum mechanical step consists of an elementary unitary operation (discussed in the following paragraph). 1. Quantum mechanical algorithms.— In a quantum computer, the logic circuitry and time steps are essentially classical, only the memory bits that hold the variables are in quantum superpositions (see [1] and [3] for a more de-tailed introduction to quantum computers). Quantum me-chanical operations that can be carried out in a controlled way are unitary operations that act on a small number of bits in each step. The quantum search algorithm of this Letter is a sequence of such unitary operations on a pure state, followed by a measurement operation. The three ele-mentary unitary operations needed are the following. First is the creation of a superposition in which the amplitude of the system being in any of the N basic states of the sys-tem is equal; second is the Walsh-Hadamard transforma-tion operation, and third the selective rotation of the phases of states. A basic operation in quantum computing is the opera-tion M performed on a single bit that is represented by the following matrix:},
author = {Grover, Lov K},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Grover - 1997 - Quantum Mechanics Helps in Searching for a Needle in a Haystack.pdf:pdf},
number = {2},
title = {{Quantum Mechanics Helps in Searching for a Needle in a Haystack}},
url = {https://journals.aps.org/prl/pdf/10.1103/PhysRevLett.79.325},
volume = {79},
year = {1997}
}
@article{Hernandez2019,
abstract = {Measuring similarity between molecules is an important part of virtual screening (VS) experiments deployed during the early stages of drug discovery. Most widely used methods for evaluating the similarity of molecules use molecular fingerprints to encode structural information. While similarity methods using fingerprint encodings are efficient, they do not consider all the relevant aspects of molecular structure. In this paper, we describe a quantum-inspired graph-based molecular similarity (GMS) method for ligand-based VS. The GMS method is formulated as a quadratic unconstrained binary optimization problem that can be solved using a quantum annealer, providing the opportunity to take advantage of this nascent and potentially groundbreaking technology. In this study, we consider various features relevant to ligand-based VS, such as pharmacophore features and three-dimensional atomic coordinates, and include them in the GMS method. We evaluate this approach on various datasets from the DUD{\_}LIB{\_}VS{\_}1.0 library. Our results show that using three-dimensional atomic coordinates as features for comparison yields higher early enrichment values. In addition, we evaluate the performance of the GMS method against conventional fingerprint approaches. The results demonstrate that the GMS method outperforms fingerprint methods for most of the datasets, presenting a new alternative in ligand-based VS with the potential for future enhancement.},
archivePrefix = {arXiv},
arxivId = {1902.00352},
author = {Hernandez, Maritza and Gan, Guo Liang and Linvill, Kirby and Dukatz, Carl and Feng, Jun and Bhisetti, Govinda},
eprint = {1902.00352},
file = {::},
month = {jan},
title = {{A Quantum-Inspired Method for Three-Dimensional Ligand-Based Virtual Screening}},
url = {http://arxiv.org/abs/1902.00352},
year = {2019}
}
@article{Friis2016,
author = {Friis, Nicolai and Huber, Marcus and Perarnau-Llobet, Mart{\'{i}}},
doi = {10.1103/PhysRevE.93.042135},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Friis, Huber, Perarnau-Llobet - 2016 - Energetics of correlations in interacting systems.pdf:pdf},
issn = {2470-0045},
journal = {Phys. Rev. E},
month = {apr},
number = {4},
pages = {042135},
publisher = {American Physical Society},
title = {{Energetics of correlations in interacting systems}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.93.042135},
volume = {93},
year = {2016}
}
@article{Campaioli2018,
abstract = {Conventional quantum speed limits perform poorly for mixed quantum states: They are generally not tight and often significantly underestimate the fastest possible evolution speed. To remedy this, for unitary driving, we derive two quantum speed limits that outperform the traditional bounds for almost all quantum states. Moreover, our bounds are significantly simpler to compute as well as experimentally more accessible. Our bounds have a clear geometric interpretation; they arise from the evaluation of the angle between generalized Bloch vectors.},
author = {Campaioli, Francesco and Pollock, Felix A. and Binder, Felix C. and Modi, Kavan},
doi = {10.1103/PhysRevLett.120.060409},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli et al. - 2017 - Tightening Quantum Speed Limits for Almost All States.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli et al. - 2018 - Tightening Quantum Speed Limits for Almost All States.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Campaioli et al. - 2018 - Tightening Quantum Speed Limits for Almost All States(2).pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {6},
pages = {060409},
publisher = {American Physical Society},
title = {{Tightening Quantum Speed Limits for Almost All States}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.060409},
volume = {120},
year = {2017}
}
@article{Petz2002,
author = {Petz, D{\'{e}}nes},
doi = {10.1088/0305-4470/35/4/305},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Petz - 2002 - Covariance and Fisher information in quantum mechanics.pdf:pdf},
issn = {0305-4470},
journal = {J. Phys. A. Math. Gen.},
month = {feb},
number = {4},
pages = {929--939},
publisher = {IOP Publishing},
title = {{Covariance and Fisher information in quantum mechanics}},
url = {http://stacks.iop.org/0305-4470/35/i=4/a=305?key=crossref.0af54f763e469a9856c39b713de5a9a0},
volume = {35},
year = {2002}
}
@article{OMalley2016,
author = {O'Malley, P. J. J. and Babbush, R. and Kivlichan, I. D. and Romero, J. and McClean, J. R. and Barends, R. and Kelly, J. and Roushan, P. and Tranter, A. and Ding, N. and Campbell, B. and Chen, Y. and Chen, Z. and Chiaro, B. and Dunsworth, A. and Fowler, A. G. and Jeffrey, E. and Lucero, E. and Megrant, A. and Mutus, J. Y. and Neeley, M. and Neill, C. and Quintana, C. and Sank, D. and Vainsencher, A. and Wenner, J. and White, T. C. and Coveney, P. V. and Love, P. J. and Neven, H. and Aspuru-Guzik, A. and Martinis, J. M.},
doi = {10.1103/PhysRevX.6.031007},
file = {::},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {jul},
number = {3},
pages = {031007},
publisher = {American Physical Society},
title = {{Scalable Quantum Simulation of Molecular Energies}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.6.031007},
volume = {6},
year = {2016}
}
@article{Gelbwaser-Klimovsky2013,
author = {Gelbwaser-Klimovsky, D. and Alicki, R. and Kurizki, G. and B., Callen H. and {Gemmer J.}, Michel M. and Mahler G. and R., Alicki and {Geusic J. E.}, Schulz-DuBios E. O. and Scovil H. E. D. and R., Kosloff and F., Ford G. W. and O'Connell R. and E., Geva and {Quan H. T.}, Liu Y.-x., Sun C. P. and Nori F. and C., Van den Broeck and J., Lin B. and Chen and {Esposito M.}, Lindenberg K. and Van den Broeck C. and D., Kieu T. and {Linden N.}, Popescu S. and Skrzypczyk P. and S., Agarwal G. S. and Chaturvedi S. and {Scully M. O.}, Chapin K. R., Dorfman K. E., Kim M. B. and Svidzinsky A. and C., Blickle V. and Bechinger and M., Allahverdyan A. E. and Nieuwenhuizen T. and {Campisi M.}, Talkner P. and H{\"{a}}nggi P. and {Campisi M.}, H{\"{a}}nggi P. and Talkner P. and S., Scully M. O. and Zubairy M. and {Gelbwaser-Klimovsky D.}, Alicki R. and Kurizki G. and {Kol{\'{a}}rř M.}, Gelbwaser-Klimovsky D., Alicki R. and Kurizki G. and {Skrzypczyk P.}, Short A. J. and Popescu S. and {Xiang Z.-L.}, Ashhab S., You J. Q. and Nori F. and {Aspelmeyer Markus}, Kippenberg Tobias J. and Marquardt Florian and E., Scovil H. E. D. and Schulz-DuBois and A., Lenard and S., Pusz W. and Woronowicz and C., Jarzynski and {Blais A.}, Huang R.-S., Wallraff A., Girvin S. M. and Schoelkopf R. J. and G., Lindblad and H., Carmichael and W., Schleich and {Petrosyan D.}, Bensky G., Kurizki G., Mazets I., Majer J. and Schmiedmayer J. and {Kubo Y.}, Ong F. R., Bertet P., Vion D., Jacques V., Zheng D., Dr{\'{e}}au A., Roch J.-F., Auffeves A., Jelezko F., Wrachtrup J., Barthe M. F., Bergonzo P. and Esteve D. and {Scully M. O.}, Zubairy M. S., Agarwal G. S. and Walther H. and U., Goswami H. P. and Harbola and H., Boukobza E. and Ritsch and {Bhaktavatsala Rao D. D.}, Bar-Gill N. and Kurizki G. and G., Kurizki and {Kurizki G.}, Kofman A. G. and Yudson V. and A., Scully M. O. and Svidzinsky A. and G., Mazets I. and Kurizki and E., Dillenschneider R. and Lutz and {Clausen J.}, Bensky G. and Kurizki G. and {Kofman A.}, Kurizki G. and Sherman B. and {Erez N.}, Gordon G., Nest M. and Kurizki G. and G., Jahnke T. and Mahler and {Gelbwaser-Klimovsky D.}, Erez N., Alicki R. and Kurizki G.},
doi = {10.1209/0295-5075/103/60005},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gelbwaser-Klimovsky et al. - 2013 - Work and energy gain of heat-pumped quantized amplifiers.pdf:pdf},
issn = {0295-5075},
journal = {EPL (Europhysics Lett.},
month = {sep},
number = {6},
pages = {60005},
publisher = {IOP Publishing},
title = {{Work and energy gain of heat-pumped quantized amplifiers}},
url = {http://stacks.iop.org/0295-5075/103/i=6/a=60005?key=crossref.34e90d2acaead34fdac9da4a944a3146},
volume = {103},
year = {2013}
}
@article{Bekenstein1981,
author = {Bekenstein, Jacob D.},
doi = {10.1103/PhysRevLett.46.623},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bekenstein - 1981 - Energy Cost of Information Transfer.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {mar},
number = {10},
pages = {623--626},
publisher = {American Physical Society},
title = {{Energy Cost of Information Transfer}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.46.623},
volume = {46},
year = {1981}
}
@article{Tomka2016,
abstract = {We propose a method to obtain optimal protocols for adiabatic ground-state preparation near the adiabatic limit, extending earlier ideas from [D. A. Sivak and G. E. Crooks, Phys. Rev. Lett. 108, 190602 (2012)] to quantum non-dissipative systems. The space of controllable parameters of isolated quantum many-body systems is endowed with a Riemannian quantum metric structure, which can be exploited when such systems are driven adiabatically. Here, we use this metric structure to construct optimal protocols in order to accomplish the task of adiabatic ground-state preparation in a fixed amount of time. Such optimal protocols are shown to be geodesics on the parameter manifold, maximizing the local fidelity. Physically, such protocols minimize the average energy fluctuations along the path. Our findings are illustrated on the Landau-Zener model and the anisotropic XY spin chain. In both cases we show that geodesic protocols drastically improve the final fidelity. Moreover, this happens even if one crosses a critical point, where the adiabatic perturbation theory fails.},
archivePrefix = {arXiv},
arxivId = {1606.05890},
author = {Tomka, Michael and Souza, Tiago and Rosenberg, Steven and Polkovnikov, Anatoli},
eprint = {1606.05890},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Tomka et al. - 2016 - Geodesic Paths for Quantum Many-Body Systems.pdf:pdf},
month = {jun},
title = {{Geodesic Paths for Quantum Many-Body Systems}},
url = {http://arxiv.org/abs/1606.05890},
year = {2016}
}
@article{VanFrank2016,
abstract = {Optimal control of complex atomic quantum systems},
author = {van Frank, S. and Bonneau, M. and Schmiedmayer, J. and Hild, S. and Gross, C. and Cheneau, M. and Bloch, I. and Pichler, T. and Negretti, A. and Calarco, T. and Montangero, S.},
doi = {10.1038/srep34187},
file = {::},
issn = {2045-2322},
journal = {Sci. Rep.},
keywords = {Quantum information,Quantum mechanics},
month = {dec},
number = {1},
pages = {34187},
publisher = {Nature Publishing Group},
title = {{Optimal control of complex atomic quantum systems}},
url = {http://www.nature.com/articles/srep34187},
volume = {6},
year = {2016}
}
@article{Korbicz2008,
abstract = {Structural approximations to positive, but not completely positive maps are approximate physical realiza-tions of these nonphysical maps. They find applications in the design of direct entanglement-detection meth-ods. We show that many of these approximations, in the relevant case of optimal positive maps, define an entanglement breaking channel and, consequently, can be implemented via a measurement and state-preparation protocol. We also show how our findings can be useful for the design of better and simpler direct entanglement detection methods.},
author = {Korbicz, J K and Almeida, M L and Bae, J and Lewenstein, M and Ac{\'{i}}n, A},
doi = {10.1103/PhysRevA.78.062105},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Korbicz et al. - 2008 - Structural approximations to positive maps and entanglement-breaking channels.pdf:pdf},
keywords = {0365Ud,0367Ϫa,PACS number͑s͒},
title = {{Structural approximations to positive maps and entanglement-breaking channels}},
url = {https://journals.aps.org/pra/pdf/10.1103/PhysRevA.78.062105},
year = {2008}
}
@article{Wootters1981,
abstract = {A concept of "statistical distance" is defined between different preparations of the same quantum system, or in other words, between different rays in the same Hilbert space. Statistical distance is determined entirely by the size of statistical fluctuations occurring in measurements designed to distinguish one state from another. It is not related, a priori, to the usual distance (or angle) between rays. One finds, however, that these two kinds of distance are in fact the same, a result which depends on certain peculiarities of quantum mechanics.},
author = {Wootters, W. K.},
doi = {10.1103/PhysRevD.23.357},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wootters - 1981 - Statistical distance and Hilbert space.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Wootters - 1981 - Statistical distance and Hilbert space(2).pdf:pdf},
issn = {05562821},
journal = {Phys. Rev. D},
month = {jan},
number = {2},
pages = {357--362},
publisher = {American Physical Society},
title = {{Statistical distance and Hilbert space}},
url = {https://link.aps.org/doi/10.1103/PhysRevD.23.357},
volume = {23},
year = {1981}
}
@article{Alicki2013,
author = {Alicki, Robert and Fannes, Mark},
doi = {10.1103/PhysRevE.87.042123},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Alicki, Fannes - 2013 - Entanglement boost for extractable work from ensembles of quantum batteries.pdf:pdf},
issn = {1539-3755},
journal = {Phys. Rev. E},
month = {apr},
number = {4},
pages = {042123},
publisher = {American Physical Society},
title = {{Entanglement boost for extractable work from ensembles of quantum batteries}},
url = {https://link.aps.org/doi/10.1103/PhysRevE.87.042123},
volume = {87},
year = {2013}
}
@article{Tang2018a,
author = {Tang, Yijun and Kao, Wil and Li, Kuan-Yu and Seo, Sangwon and Mallayya, Krishnanand and Rigol, Marcos and Gopalakrishnan, Sarang and Lev, Benjamin L.},
doi = {10.1103/PhysRevX.8.021030},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Tang et al. - 2018 - Thermalization near Integrability in a Dipolar Quantum Newton's Cradle.pdf:pdf},
issn = {2160-3308},
journal = {Phys. Rev. X},
month = {may},
number = {2},
pages = {021030},
publisher = {American Physical Society},
title = {{Thermalization near Integrability in a Dipolar Quantum Newton's Cradle}},
url = {https://link.aps.org/doi/10.1103/PhysRevX.8.021030},
volume = {8},
year = {2018}
}
@article{Loiseau1967,
author = {Loiseau, B.A. and Nogami, Y.},
doi = {10.1016/0550-3213(67)90184-8},
issn = {05503213},
journal = {Nucl. Phys. B},
keywords = {expectation value,interactions,many body problem,nuclear models,nucleons,quantum mechanics,three body problem,tritons},
number = {4},
pages = {470--478},
title = {{Three-nucleon force}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0550321367901848},
volume = {2},
year = {1967}
}
@article{Mathger2007,
author = {M{\"{a}}thger, Lydia M. and Hanlon, Roger T.},
doi = {10.1007/s00441-007-0384-8},
issn = {0302-766X},
journal = {Cell Tissue Res.},
month = {may},
number = {1},
pages = {179--186},
publisher = {Springer-Verlag},
title = {{Malleable skin coloration in cephalopods: selective reflectance, transmission and absorbance of light by chromatophores and iridophores}},
url = {http://link.springer.com/10.1007/s00441-007-0384-8},
volume = {329},
year = {2007}
}
@article{Escher2011,
abstract = {The estimation of parameters characterizing dynamical processes is central to science and technology. The estimation error changes with the number N of resources employed in the experiment (which could quantify, for instance, the number of probes or the probing energy). Typically, it scales as 1/ √ N. Quantum strategies may improve the precision, for noiseless processes, by an extra factor 1/ √ N. For noisy processes, it is not known in general if and when this improvement can be achieved. Here we propose a general framework for obtaining attainable and useful lower bounds for the ultimate limit of precision in noisy systems. We apply this bound to lossy optical interferometry and atomic spectroscopy in the presence of dephasing, showing that it captures the main features of the transition from the 1/N to the 1/ √ N behaviour as N increases, independently of the initial state of the probes, and even with use of adaptive feedback. I t is by now well established that, in the absence of noise, the quantum properties of probes help to increase the precision in the estimation of parameters that characterize dynamical processes, such as phase shifts in optical interferometry or transition frequencies in atomic spectroscopy 1–4 . The estimation error decreases with the amount of resources employed in the measurement, which might be for instance the energy of a probing light field or the number N of identical probes. For independent probes, it is proportional to 1/ √ N , a consequence of the central limit theorem. By entangling the probes one may attain, for noiseless processes, the ultimate lower bound for the estimation error, which scales then as 1/N (refs 3,4), the so-called Heisenberg limit, thus allowing better accuracy for the same number of resources. For noisy processes, however, it is not known in general if this limit can be attained, and if entanglement can still be a helpful resource for this purpose. For lossy optical interferometry, it was shown recently 5,6 that the Heisenberg limit is not attainable when N → ∞. General expressions for the uncertainty in the estimation are known, but their calculation involves complex optimization procedures, which become quite cumbersome when the number of resources increases. Here we show that the effectiveness of quantum states for parameter estimation in the presence of noise can be precisely assessed. We introduce a bound for this uncertainty, proven to be attainable, which leads to useful expressions for the ultimate limit of precision in noisy systems. We exemplify the utility of this bound by applying it to lossy optical interferometry and atomic spectroscopy in the presence of dephasing.},
author = {Escher, B M and De, R L and Filho, Matos and Davidovich, L},
doi = {10.1038/NPHYS1958},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Escher et al. - 2011 - General framework for estimating the ultimate precision limit in noisy quantum-enhanced metrology.pdf:pdf},
journal = {Nat. Phys.},
title = {{General framework for estimating the ultimate precision limit in noisy quantum-enhanced metrology}},
volume = {7},
year = {2011}
}
@article{Leubner1985,
author = {Leubner, C. and Kiener, C.},
doi = {10.1103/PhysRevA.31.483},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Leubner, Kiener - 1985 - Improvement of the Eberly-Singh time-energy inequality by combination with the Mandelstam-Tamm approach.pdf:pdf},
issn = {0556-2791},
journal = {Phys. Rev. A},
month = {jan},
number = {1},
pages = {483--485},
publisher = {American Physical Society},
title = {{Improvement of the Eberly-Singh time-energy inequality by combination with the Mandelstam-Tamm approach}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.31.483},
volume = {31},
year = {1985}
}
@article{Abernethy2009,
author = {Abernethy, J and Bach, F and Evgeniou, T},
file = {::},
journal = {J. Mach. Learn. Res.},
pages = {803--826},
title = {{A new approach to collaborative filtering: Operator estimation with spectral regularization}},
url = {http://www.jmlr.org/papers/v10/abernethy09a.html},
volume = {10},
year = {2009}
}
@article{Agarwal2018,
author = {Agarwal, Kartiek and Bhatt, R. N. and Sondhi, S. L.},
doi = {10.1103/PhysRevLett.120.210604},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {may},
number = {21},
pages = {210604},
publisher = {American Physical Society},
title = {{Fast Preparation of Critical Ground States Using Superluminal Fronts}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.210604},
volume = {120},
year = {2018}
}
@book{Provost1980a,
author = {Provost, J. P. and Vallee, G.},
booktitle = {Commun. Math. Phys.},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Provost, Vallee - 1980 - Communications in mathematical physics.pdf:pdf},
issn = {0010-3616},
number = {3},
pages = {289--301},
publisher = {Springer-Verlag Heidelberg},
title = {{Communications in mathematical physics.}},
url = {https://projecteuclid.org/euclid.cmp/1103908308},
volume = {76},
year = {1980}
}
@article{Yamaguchi1979,
author = {Yamaguchi, N. and Kasahara, T. and Nagata, S. and Akaishi, Y.},
doi = {10.1143/PTP.62.1018},
issn = {0033-068X},
journal = {Prog. Theor. Phys.},
month = {oct},
number = {4},
pages = {1018--1034},
publisher = {Oxford University Press},
title = {{Effective Interaction with Three-Body Effects}},
url = {http://ptp.oxfordjournals.org/cgi/doi/10.1143/PTP.62.1018},
volume = {62},
year = {1979}
}
@article{Yu2006,
author = {Yu, T. and Eberly, J. H.},
doi = {10.1103/PhysRevLett.97.140403},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Yu, Eberly - 2006 - Quantum Open System Theory Bipartite Aspects.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett},
month = {oct},
number = {14},
pages = {140403},
publisher = {American Physical Society},
title = {{Quantum Open System Theory: Bipartite Aspects}},
url = {http://link.aps.org/doi/10.1103/PhysRevLett.97.140403},
volume = {97},
year = {2006}
}
@article{Markham2008,
author = {Markham, Damian and Miszczak, Jaros{\l}aw Adam and Pucha{\l}a, Zbigniew and {\.{Z}}yczkowski, Karol},
doi = {10.1103/PhysRevA.77.042111},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Markham et al. - 2008 - Quantum state discrimination A geometric approach.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {apr},
number = {4},
pages = {042111},
publisher = {American Physical Society},
title = {{Quantum state discrimination: A geometric approach}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.77.042111},
volume = {77},
year = {2008}
}
@article{Dillavou2018,
author = {Dillavou, Sam and Rubinstein, Shmuel M.},
doi = {10.1103/PhysRevLett.120.224101},
file = {::},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {jun},
number = {22},
pages = {224101},
publisher = {American Physical Society},
title = {{Nonmonotonic Aging and Memory in a Frictional Interface}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.224101},
volume = {120},
year = {2018}
}
@article{Margolus1998,
author = {Margolus, Norman and Levitin, Lev B.},
doi = {10.1016/S0167-2789(98)00054-2},
issn = {01672789},
journal = {Phys. D Nonlinear Phenom.},
number = {1-2},
pages = {188--195},
publisher = {North-Holland},
title = {{The maximum speed of dynamical evolution}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0167278998000542},
volume = {120},
year = {1998}
}
@article{Byrd2003,
abstract = {A parameterization of the density operator, a coherence vector representation, which uses a basis of orthogonal, traceless, Hermitian matrices is discussed. Using this parameterization we find the region of permissible vectors which represent a density operator. The inequalities which specify the region are shown to involve the Casimir invariants of the group. In particular cases, this allows the determination of degeneracies in the spectrum of the operator. The identification of the Casimir invariants also provides a method of constructing quantities which are invariant under local unitary operations. Several examples are given which illustrate the constraints provided by the positivity requirements and the utility of the coherence vector parameterization.},
author = {Byrd, Mark S and Khaneja, Navin},
doi = {10.1103/PhysRevA.68.062322},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Byrd, Khaneja - 2003 - Characterization of the Positivity of the Density Matrix in Terms of the Coherence Vector Representation.pdf:pdf},
journal = {Phys. Rev. A},
pages = {062322},
title = {{Characterization of the Positivity of the Density Matrix in Terms of the Coherence Vector Representation}},
url = {https://journals.aps.org/pra/abstract/10.1103/PhysRevA.68.062322},
volume = {68},
year = {2003}
}
@article{Gong2016,
abstract = {We employ the quantum jump trajectory approach to construct a systematic framework to study the thermodynamics at the trajectory level in a nonequilibrium open quantum system under discrete feedback control. Within this framework, we derive quantum versions of the generalized Jarzynski equalities, which are demonstrated in an isolated pseudospin system and a coherently driven two-level open quantum system. Due to quantum coherence and measurement backaction, a fundamental distinction from the classical generalized Jarzynski equalities emerges in the quantum versions, which is characterized by a large negative information gain reflecting genuinely quantum rare events. A possible experimental scheme to test our findings in superconducting qubits is discussed.},
archivePrefix = {arXiv},
arxivId = {1602.04616},
author = {Gong, Zongping and Ashida, Yuto and Ueda, Masahito},
doi = {10.1103/PhysRevA.94.012107},
eprint = {1602.04616},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gong, Ashida, Ueda - 2016 - Quantum Trajectory Thermodynamics with Discrete Feedback Control(2).pdf:pdf},
month = {feb},
title = {{Quantum Trajectory Thermodynamics with Discrete Feedback Control}},
url = {http://arxiv.org/abs/1602.04616 http://dx.doi.org/10.1103/PhysRevA.94.012107 https://arxiv.org/abs/1602.04616},
year = {2016}
}
@article{DelCampo2013b,
author = {del Campo, Adolfo},
doi = {10.1103/PhysRevLett.111.100502},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/del Campo - 2013 - Shortcuts to Adiabaticity by Counterdiabatic Driving.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {sep},
number = {10},
pages = {100502},
publisher = {American Physical Society},
title = {{Shortcuts to Adiabaticity by Counterdiabatic Driving}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.100502},
volume = {111},
year = {2013}
}
@article{Nimmrichter,
abstract = {We propose an experimentally accessible, objective measure for the macroscopicity of superposition states in mechanical quantum systems. Based on the observable consequences of a minimal, macrorealist extension of quantum mechanics, it allows one to quantify the degree of macroscopicity achieved in different experiments.},
author = {Nimmrichter, Stefan and Hornberger, Klaus},
doi = {10.1103/PhysRevLett.110.160403},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Nimmrichter, Hornberger - Unknown - Macroscopicity of Mechanical Quantum Superposition States.pdf:pdf},
title = {{Macroscopicity of Mechanical Quantum Superposition States}}
}
@article{Jones2010,
abstract = {The Mandelstam-Tamm and Margolus-Levitin inequalities play an important role in the study of quantum-mechanical processes in nature since they provide general limits on the speed of dynamical evolution. However, to date there has been only one derivation of the Margolus-Levitin inequality. In this paper, alternative geometric derivations for both inequalities are obtained from the statistical distance between quantum states. The inequalities are shown to hold for unitary evolution of pure and mixed states, and a counterexample to the inequalities is given for evolution described by completely positive trace-preserving maps. The counterexample shows that there is no quantum speed limit for nonunitary evolution.},
author = {Jones, Philip J. and Kok, Pieter},
doi = {10.1103/PhysRevA.82.022107},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Jones, Kok - 2010 - Geometric derivation of the quantum speed limit(3).pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Jones, Kok - 2010 - Geometric derivation of the quantum speed limit(2).pdf:pdf},
isbn = {1094-1622},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {aug},
number = {2},
pages = {022107},
publisher = {American Physical Society},
title = {{Geometric derivation of the quantum speed limit}},
url = {https://journals.aps.org/pra/pdf/10.1103/PhysRevA.82.022107},
volume = {82},
year = {2010}
}
@article{Gardas,
abstract = {The Carnot statement of the second law of thermodynamics poses an upper limit on the efficiency of all heat engines. Recently, it has been studied whether generic quantum features such as coherence and quantum entanglement could allow for quantum devices with efficiencies larger than the Carnot efficiency. The present study shows that this is not permitted by the laws of thermodynamics—independent of the model. We will show that rather the definition of heat has to be modified to account for the thermodynamic cost of maintaining non-Gibbsian equilibrium states. Our theoretical findings are illustrated for two experimentally relevant examples.},
author = {Gardas, Bart{\l}omiej and Deffner, Sebastian},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gardas, Deffner - Unknown - Thermodynamic universality of quantum Carnot engines.pdf:pdf},
journal = {Pysical Rev. E},
title = {{Thermodynamic universality of quantum Carnot engines}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.92.042126},
year = {2015}
}
@inproceedings{Deterding2011,
address = {New York, New York, USA},
author = {Deterding, Sebastian and Sicart, Miguel and Nacke, Lennart and O'Hara, Kenton and Dixon, Dan},
booktitle = {Proc. 2011 Annu. Conf. Ext. Abstr. Hum. factors Comput. Syst. - CHI EA '11},
doi = {10.1145/1979742.1979575},
isbn = {9781450302685},
keywords = {design patterns,funology,game design,games with a purpose,gamification,motivational affordances,persuasive technology},
pages = {2425},
publisher = {ACM Press},
title = {{Gamification. using game-design elements in non-gaming contexts}},
url = {http://portal.acm.org/citation.cfm?doid=1979742.1979575},
year = {2011}
}
@article{Study1905,
author = {Study, Edurard},
journal = {Math. Ann.},
pages = {321--378},
title = {{K{\"{u}}rzeste Wege im komplexen Gebiet}},
volume = {60},
year = {1905}
}
@article{Petersen2010,
author = {Petersen, I.R. and Dong, D.},
doi = {10.1049/iet-cta.2009.0508},
issn = {1751-8644},
journal = {IET Control Theory Appl.},
month = {dec},
number = {12},
pages = {2651--2671},
title = {{Quantum control theory and applications: a survey}},
url = {http://digital-library.theiet.org/content/journals/10.1049/iet-cta.2009.0508},
volume = {4},
year = {2010}
}
@article{Frommer2010,
abstract = {We present methods to compute verified square roots of a square matrix A. Given an approximation X to the square root, obtained by a classical floating point algorithm, we use interval arithmetic to find an interval matrix which is guaranteed to contain the error of X. Our approach is based on the Krawczyk method, which we modify in two different ways in such a manner that the computational complexity for an {\$}n\backslashtimes n{\$} matrix is reduced to {\$}n{\^{}}3{\$}. The methods are based on the spectral decomposition or, in the case that the eigenvector matrix is ill conditioned, on a similarity transformation to block diagonal form. Numerical experiments prove that our methods are computationally efficient and that they yield narrow enclosures provided X is a good approximation. This is particularly true for symmetric matrices, since their eigenvector matrix is perfectly conditioned.},
author = {Frommer, Andreas and Hashemi, Behnam},
doi = {10.1137/090757058},
issn = {0895-4798},
journal = {SIAM J. Matrix Anal. Appl.},
keywords = {65F30,65F60,65G20,Brouwer's fixed point theorem,Krawczyk's method,Kronecker structures,circular arithmetic,interval analysis,matrix square root},
month = {jan},
number = {3},
pages = {1279--1302},
publisher = {Society for Industrial and Applied Mathematics},
title = {{Verified Computation of Square Roots of a Matrix}},
url = {http://epubs.siam.org/doi/10.1137/090757058},
volume = {31},
year = {2010}
}
@article{Gibilisco2007,
archivePrefix = {arXiv},
arxivId = {0712.1208},
author = {Gibilisco, Paolo and Hiai, Fumio and Petz, Denes},
eprint = {0712.1208},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Gibilisco, Hiai, Petz - 2007 - Quantum covariance, quantum Fisher information and the uncertainty principle.pdf:pdf},
title = {{Quantum covariance, quantum Fisher information and the uncertainty principle}},
url = {https://arxiv.org/abs/0712.1208},
year = {2007}
}
@article{Bravyi2012,
author = {Bravyi, Sergey and Haah, Jeongwan},
doi = {10.1103/PhysRevA.86.052329},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {nov},
number = {5},
pages = {052329},
publisher = {American Physical Society},
title = {{Magic-state distillation with low overhead}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.86.052329},
volume = {86},
year = {2012}
}
@article{An2016,
abstract = {The application of adiabatic protocols in quantum technologies is limited due to the detrimental action of decoherence. Here the authors demonstrate a shortcut to adiabaticity via counterdiabatic driving in a trapped ion system.},
author = {An, Shuoming and Lv, Dingshun and del Campo, Adolfo and Kim, Kihwan},
doi = {10.1038/ncomms12999},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/An et al. - 2016 - Shortcuts to adiabaticity by counterdiabatic driving for trapped-ion displacement in phase space.pdf:pdf},
issn = {2041-1723},
journal = {Nat. Commun.},
keywords = {Atomic and molecular interactions with photons,Quantum mechanics,Quantum optics},
month = {sep},
pages = {12999},
publisher = {Nature Publishing Group},
title = {{Shortcuts to adiabaticity by counterdiabatic driving for trapped-ion displacement in phase space}},
url = {http://www.nature.com/doifinder/10.1038/ncomms12999},
volume = {7},
year = {2016}
}
@article{Girolami2014,
author = {Girolami, Davide},
doi = {10.1103/PhysRevLett.113.170401},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Girolami - 2014 - Observable Measure of Quantum Coherence in Finite Dimensional Systems.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {oct},
number = {17},
pages = {170401},
publisher = {American Physical Society},
title = {{Observable Measure of Quantum Coherence in Finite Dimensional Systems}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.113.170401},
volume = {113},
year = {2014}
}
@article{Doherty1999,
author = {Doherty, A. C. and Jacobs, K.},
doi = {10.1103/PhysRevA.60.2700},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {oct},
number = {4},
pages = {2700--2711},
publisher = {American Physical Society},
title = {{Feedback control of quantum systems using continuous state estimation}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.60.2700},
volume = {60},
year = {1999}
}
@article{Sabin2008,
author = {Sab{\'{i}}n, C. and Garc{\'{i}}a-Alcaine, G.},
doi = {10.1140/epjd/e2008-00112-5},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Sab{\'{i}}n, Garc{\'{i}}a-Alcaine - 2008 - A classification of entanglement in three-qubit systems.pdf:pdf},
issn = {1434-6060},
journal = {Eur. Phys. J. D},
month = {jul},
number = {3},
pages = {435--442},
publisher = {EDP Sciences},
title = {{A classification of entanglement in three-qubit systems}},
url = {http://www.springerlink.com/index/10.1140/epjd/e2008-00112-5},
volume = {48},
year = {2008}
}
@article{Miszczak2008,
abstract = {We derive several bounds on fidelity between quantum states. In particular we show that fidelity is bounded from above by a simple to compute quantity we call super--fidelity. It is analogous to another quantity called sub--fidelity. For any two states of a two--dimensional quantum system (N=2) all three quantities coincide. We demonstrate that sub-- and super--fidelity are concave functions. We also show that super--fidelity is super--multiplicative while sub--fidelity is sub--multiplicative and design feasible schemes to measure these quantities in an experiment. Super--fidelity can be used to define a distance between quantum states. With respect to this metric the set of quantum states forms a part of a {\$}N{\^{}}2-1{\$} dimensional hypersphere.},
archivePrefix = {arXiv},
arxivId = {0805.2037},
author = {Miszczak, J. A. and Pucha{\l}a, Z. and Horodecki, P. and Uhlmann, A. and {\.{Z}}yczkowski, K.},
eprint = {0805.2037},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Miszczak et al. - 2008 - Sub-- and super--fidelity as bounds for quantum fidelity.pdf:pdf},
journal = {Quantum Inf. Comput.},
month = {may},
number = {1{\&}2},
title = {{Sub-- and super--fidelity as bounds for quantum fidelity}},
url = {http://arxiv.org/abs/0805.2037},
volume = {9},
year = {2009}
}
@article{Murphy2010,
abstract = {Spin chains have long been considered as candidates for quantum channels to facilitate quantum communication. We consider the transfer of a single excitation along a spin-1/2 chain governed by Heisenberg-type interactions. We build on the work of Balachandran and Gong [1], and show that by applying optimal control to an external parabolic magnetic field, one can drastically increase the propagation rate by two orders of magnitude. In particular, we show that the theoretical maximum propagation rate can be reached, where the propagation of the excitation takes the form of a dispersed wave. We conclude that optimal control is not only a useful tool for experimental application, but also for theoretical enquiry into the physical limits and dynamics of many-body quantum systems.},
author = {Murphy, Michael and Montangero, Simone and Giovannetti, Vittorio and Calarco, Tommaso},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Murphy et al. - 2010 - Communication at the quantum speed limit along a spin chain(2).pdf:pdf},
issn = {10502947},
journal = {Phys. Rev. A},
number = {2},
pages = {022318},
title = {{Communication at the quantum speed limit along a spin chain}},
url = {https://doi.org/10.1103/PhysRevA.82.022318},
volume = {82},
year = {2010}
}
@article{Goyal2016,
author = {Goyal, Sandeep K and Simon, B Neethi and Singh, Rajeev and Simon, Sudhavathani},
doi = {10.1088/1751-8113/49/16/165203},
file = {::},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {apr},
number = {16},
pages = {165203},
publisher = {IOP Publishing},
title = {{Geometry of the generalized Bloch sphere for qutrits}},
url = {http://stacks.iop.org/1751-8121/49/i=16/a=165203?key=crossref.d6f8ffb63e7fcf01daadd48d1c0d6823},
volume = {49},
year = {2016}
}
@article{Bennett1992,
author = {Bennett, Charles H. and Bessette, Francois and Brassard, Gilles and Salvail, Louis and Smolin, John},
doi = {10.1007/BF00191318},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Bennett et al. - 1992 - Experimental quantum cryptography.pdf:pdf},
issn = {0933-2790},
journal = {J. Cryptol.},
number = {1},
pages = {3--28},
publisher = {Springer-Verlag},
title = {{Experimental quantum cryptography}},
url = {http://link.springer.com/10.1007/BF00191318},
volume = {5},
year = {1992}
}
@article{Schrodinger1935,
author = {Schr{\"{o}}dinger, E. and Born, M. and Podolsky, B. and Rosen, N.},
doi = {10.1017/S0305004100013554},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Schr{\"{o}}dinger et al. - 1935 - Discussion of Probability Relations between Separated Systems.pdf:pdf},
issn = {0305-0041},
journal = {Math. Proc. Cambridge Philos. Soc.},
number = {04},
pages = {555},
publisher = {Cambridge University Press},
title = {{Discussion of Probability Relations between Separated Systems}},
url = {http://www.journals.cambridge.org/abstract{\_}S0305004100013554},
volume = {31},
year = {1935}
}
@article{Schirmer2010,
author = {Schirmer, S. G. and Wang, Xiaoting},
doi = {10.1103/PhysRevA.81.062306},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Schirmer, Wang - 2010 - Stabilizing open quantum systems by Markovian reservoir engineering.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {jun},
number = {6},
pages = {062306},
publisher = {American Physical Society},
title = {{Stabilizing open quantum systems by Markovian reservoir engineering}},
url = {https://link.aps.org/doi/10.1103/PhysRevA.81.062306},
volume = {81},
year = {2010}
}
@article{Ollivier2001,
author = {Ollivier, Harold and Zurek, Wojciech H.},
doi = {10.1103/PhysRevLett.88.017901},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Ollivier, Zurek - 2001 - Quantum Discord A Measure of the Quantumness of Correlations.pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {dec},
number = {1},
pages = {017901},
publisher = {American Physical Society},
title = {{Quantum Discord: A Measure of the Quantumness of Correlations}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.88.017901},
volume = {88},
year = {2001}
}
@article{Ilichev2003,
author = {Il'ichev, E. and Oukhanski, N. and Izmalkov, A. and Wagner, Th. and Grajcar, M. and Meyer, H.-G. and Smirnov, A. Yu. and {Maassen van den Brink}, Alec and Amin, M. H. S. and Zagoskin, A. M.},
doi = {10.1103/PhysRevLett.91.097906},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {aug},
number = {9},
pages = {097906},
publisher = {American Physical Society},
title = {{Continuous Monitoring of Rabi Oscillations in a Josephson Flux Qubit}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.097906},
volume = {91},
year = {2003}
}
@article{Dunjko2018,
author = {Dunjko, Vedran and Briegel, Hans J},
doi = {10.1088/1361-6633/aab406},
issn = {0034-4885},
journal = {Reports Prog. Phys.},
month = {jul},
number = {7},
pages = {074001},
publisher = {IOP Publishing},
title = {{Machine learning {\&} artificial intelligence in the quantum domain: a review of recent progress}},
url = {http://stacks.iop.org/0034-4885/81/i=7/a=074001?key=crossref.484b39e1cdde454de1cbc5aba8d6de34},
volume = {81},
year = {2018}
}
@article{Uffink1993,
author = {Uffink, Jos},
doi = {10.1119/1.17368},
issn = {00029505},
journal = {Am. J. Phys.},
keywords = {ENERGY,HALF−LIFE,PROJECTION OPERATORS,QUANTUM MECHANICS,TIME DEPENDENCE,UNCERTAINTY PRINCIPLE,WAVE FUNCTIONS},
month = {oct},
number = {10},
pages = {935},
publisher = {American Association of Physics Teachers},
title = {{The rate of evolution of a quantum state}},
url = {http://aapt.scitation.org/doi/10.1119/1.17368 http://link.aip.org/link/?AJP/61/935/1{\&}Agg=doi},
volume = {61},
year = {1993}
}
@article{Bruschweiler1996,
abstract = {The imaginary part of the magnetic dipole–dipole cross correlation spectral density in spin 1/2 systems generates a novel type of three‐spin Hamiltonian with terms I iz I jz I kz , I iz I jx I kx , and I iz I jy I ky and permutations in the spin labels i, j, k. These terms cause asymmetric positions of the spin multiplet components, which could not be explained by scalar J‐coupling and chemical shift terms.},
author = {Brüschweiler, R.},
doi = {10.1063/1.472475},
issn = {00219606},
journal = {J. Chem. Phys.},
number = {15},
pages = {6164},
publisher = {AIP Publishing},
title = {{Three-spin interaction in liquid state nuclear magnetic resonance}},
url = {http://scitation.aip.org/content/aip/journal/jcp/105/15/10.1063/1.472475},
volume = {105},
year = {1996}
}
@article{Binder2015,
author = {Binder, Felix C and Vinjanampathy, Sai and Modi, Kavan and Goold, John},
doi = {10.1088/1367-2630/17/7/075015},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Binder et al. - 2015 - Quantacell powerful charging of quantum batteries.pdf:pdf},
issn = {1367-2630},
journal = {New J. Phys.},
number = {7},
pages = {075015},
publisher = {IOP Publishing},
title = {{Quantacell: powerful charging of quantum batteries}},
url = {http://stacks.iop.org/1367-2630/17/i=7/a=075015?key=crossref.f48460736c353d5a2ed1ba5437285c6e},
volume = {17},
year = {2015}
}
@article{Francica2017,
abstract = {We investigate how the presence of quantum correlations can influence work extraction in closed quantum systems, establishing a new link between the field of quantum non-equilibrium thermodynamics and the one of quantum information theory. We consider a bipartite quantum system and we show that it is possible to optimize the process of work extraction, thanks to the correlations between the two parts of the system, by using an appropriate feedback protocol based on the concept of ergotropy. We prove that the maximum gain in the extracted work is related to the existence of quantum correlations between the two parts, quantified by either quantum discord or, for pure states, entanglement. We then illustrate our general findings on a simple physical situation consisting of a qubit system.},
author = {Francica, Gianluca and Goold, John and Plastina, Francesco and Paternostro, Mauro},
doi = {10.1038/s41534-017-0012-8},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Francica et al. - 2017 - Daemonic ergotropy enhanced work extraction from quantum correlations.pdf:pdf},
issn = {2056-6387},
journal = {npj Quantum Inf.},
keywords = {Quantum information,Theoretical physics},
month = {dec},
number = {1},
pages = {12},
publisher = {Nature Publishing Group},
title = {{Daemonic ergotropy: enhanced work extraction from quantum correlations}},
url = {http://www.nature.com/articles/s41534-017-0012-8},
volume = {3},
year = {2017}
}
@article{Zahedinejad2019,
abstract = {Signed graphs serve as a primary tool for modelling social networks. They can represent relationships between individuals (i.e., nodes) with the use of signed edges. Finding communities in a signed graph is of great importance in many areas, for example, targeted advertisement. We propose an algorithm to detect multiple communities in a signed graph. Our method reduces the multi-community detection problem to a quadratic binary unconstrained optimization problem and uses state-of-the-art quantum or classical optimizers to find an optimal assignment of each individual to a specific community.},
archivePrefix = {arXiv},
arxivId = {1901.04873},
author = {Zahedinejad, Ehsan and Crawford, Daniel and Adolphs, Clemens and Oberoi, Jaspreet S.},
eprint = {1901.04873},
file = {::},
month = {jan},
title = {{Multi-Community Detection in Signed Graphs Using Quantum Hardware}},
url = {http://arxiv.org/abs/1901.04873},
year = {2019}
}
@article{Borras2008,
author = {Borras, A. and Zander, C. and Plastino, A. R. and Casas, M. and Plastino, A.},
doi = {10.1209/0295-5075/81/30007},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Borras et al. - 2008 - Entanglement and the quantum brachistochrone problem.pdf:pdf},
issn = {0295-5075},
journal = {EPL},
month = {feb},
number = {3},
pages = {30007},
publisher = {IOP Publishing},
title = {{Entanglement and the quantum brachistochrone problem}},
url = {http://stacks.iop.org/0295-5075/81/i=3/a=30007?key=crossref.26a4121fc247b6748d695aebcc993501},
volume = {81},
year = {2008}
}
@article{You2005,
author = {You, J. Q. and Hu, Xuedong and Nori, Franco},
doi = {10.1103/PhysRevB.72.144529},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/You, Hu, Nori - 2005 - Correlation-induced suppression of decoherence in capacitively coupled Cooper-pair boxes.pdf:pdf},
issn = {1098-0121},
journal = {Phys. Rev. B},
month = {oct},
number = {14},
pages = {144529},
publisher = {American Physical Society},
title = {{Correlation-induced suppression of decoherence in capacitively coupled Cooper-pair boxes}},
url = {https://link.aps.org/doi/10.1103/PhysRevB.72.144529},
volume = {72},
year = {2005}
}
@article{Uzdin2012,
author = {Uzdin, Raam and G{\"{u}}nther, Uwe and Rahav, Saar and Moiseyev, Nimrod},
doi = {10.1088/1751-8113/45/41/415304},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Uzdin et al. - 2012 - Time-dependent Hamiltonians with 100{\%} evolution speed efficiency.pdf:pdf},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {oct},
number = {41},
pages = {415304},
publisher = {IOP Publishing},
title = {{Time-dependent Hamiltonians with 100{\%} evolution speed efficiency}},
url = {http://stacks.iop.org/1751-8121/45/i=41/a=415304?key=crossref.cf78bbe82541f4d253bf9e63f5a1da36},
volume = {45},
year = {2012}
}
@article{Wheeler1957,
author = {Wheeler, John A.},
doi = {10.1103/RevModPhys.29.463},
issn = {0034-6861},
journal = {Rev. Mod. Phys.},
month = {jul},
number = {3},
pages = {463--465},
publisher = {American Physical Society},
title = {{Assessment of Everett's "Relative State" Formulation of Quantum Theory}},
url = {https://link.aps.org/doi/10.1103/RevModPhys.29.463},
volume = {29},
year = {1957}
}
@article{Machnes2015,
abstract = {We argue that quantum optimal control can and should be done with analytic control functions, in the vast majority of applications. First, we show that discretizing continuous control functions as piecewise-constant functions prevents high accuracy optimization at reasonable computational costs. Second, we argue that the number of control parameters required is on-par with the dimension of the object manipulated, and therefore one may choose parametrization by other considerations, e.g. experimental suitability and the potential for physical insight into the optimized pulse. Third, we note that optimal control algorithms which make use of the gradient of the goal function with respect to control parameters are generally faster and reach higher final accuracies than non gradient-based methods. Thus, if the gradient can be efficiently computed, it should be used. Fourth, we present a novel way of computing the gradient based on an equation of motion for the gradient, which we evolve in time by the Taylor expansion of the propagator. This allows one to calculate any physically relevant analytic controls to arbitrarily high precision. The combination of the above techniques is GOAT (Gradient Optimization of Analytic conTrols) - gradient-based optimal control for analytic control functions, utilizing exact evolution in time of the derivative of the propagator with respect to arbitrary control parameters.},
archivePrefix = {arXiv},
arxivId = {1507.04261},
author = {Machnes, Shai and Tannor, David J. and Wilhelm, Frank K. and Ass{\'{e}}mat, Elie},
eprint = {1507.04261},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Machnes et al. - 2015 - Gradient optimization of analytic controls the route to high accuracy quantum optimal control.pdf:pdf},
month = {jul},
title = {{Gradient optimization of analytic controls: the route to high accuracy quantum optimal control}},
url = {http://arxiv.org/abs/1507.04261},
year = {2015}
}
@article{Giovannetti2004,
abstract = {How fast can a quantum system evolve? In this paper we study the relation between entanglement and the time it takes for a composite system to perform a given evolution. In particular, we analyse how the order of the interactions shapes the dynamics.},
author = {Giovannetti, Vittorio and Lloyd, Seth and Maccone, Lorenzo},
doi = {10.1088/1464-4266/6/8/028},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Giovannetti, Lloyd, Maccone - 2004 - The speed limit of quantum unitary evolution.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Giovannetti, Lloyd, Maccone - 2004 - The speed limit of quantum unitary evolution(2).pdf:pdf},
issn = {1464-4266},
journal = {J. Opt. B Quantum Semiclassical Opt.},
keywords = {dynamical evolution,entanglement,speed limit,time–energy uncertainty principle},
month = {aug},
number = {8},
pages = {S807--S810},
publisher = {IOP Publishing},
title = {{The speed limit of quantum unitary evolution}},
url = {http://stacks.iop.org/1464-4266/6/i=8/a=028?key=crossref.99d5f38f392f5a361a8822eaad6c5b4c http://iopscience.iop.org/1464-4266/6/8/028},
volume = {6},
year = {2004}
}
@article{Santos2018,
author = {Santos, Alan C and Sarandy, Marcelo S},
doi = {10.1088/1751-8121/aa96f1},
file = {::},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {jan},
number = {2},
pages = {025301},
publisher = {IOP Publishing},
title = {{Generalized shortcuts to adiabaticity and enhanced robustness against decoherence}},
url = {http://stacks.iop.org/1751-8121/51/i=2/a=025301?key=crossref.ec66674c4a132430bef6ed9d5ada69ca},
volume = {51},
year = {2018}
}
@article{Eigler1990,
author = {Eigler, D. M. and Schweizer, E. K.},
doi = {10.1038/344524a0},
issn = {0028-0836},
journal = {Nature},
pages = {524--526},
publisher = {Nature Publishing Group},
title = {{Positioning single atoms with a scanning tunnelling microscope}},
url = {http://www.nature.com/doifinder/10.1038/344524a0},
volume = {344},
year = {1990}
}
@article{Okuyama2018,
abstract = {The quantum speed limit (QSL), or the energy-time uncertainty relation, describes the fundamental maximum rate for quantum time evolution and has been regarded as being unique in quantum mechanics. In this study, we obtain a classical speed limit corresponding to the QSL using the Hilbert space for the classical Liouville equation. Thus, classical mechanics has a fundamental speed limit, and QSL is not a purely quantum phenomenon but a universal dynamical property of the Hilbert space. Furthermore, we obtain similar speed limits for the imaginary-time Schroedinger equations such as the master equation.},
author = {Okuyama, Manaka and Ohzeki, Masayuki},
doi = {10.1103/PhysRevLett.120.070402},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Okuyama, Ohzeki - 2018 - Quantum Speed Limit is Not Quantum.pdf:pdf;:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Okuyama, Ohzeki - 2017 - Quantum Speed Limit is Not Quantum(2).pdf:pdf},
issn = {0031-9007},
journal = {Phys. Rev. Lett.},
month = {feb},
number = {7},
pages = {070402},
publisher = {American Physical Society},
title = {{Quantum Speed Limit is Not Quantum}},
url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.070402},
volume = {120},
year = {2018}
}
@article{Deffner2013,
author = {Deffner, Sebastian and Lutz, Eric},
doi = {10.1088/1751-8113/46/33/335302},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Deffner, Lutz - 2013 - Energy–time uncertainty relation for driven quantum systems.pdf:pdf},
issn = {1751-8113},
journal = {J. Phys. A Math. Theor.},
month = {aug},
number = {33},
pages = {335302},
publisher = {IOP Publishing},
title = {{Energy–time uncertainty relation for driven quantum systems}},
volume = {46},
year = {2013}
}
@article{Winter2016,
author = {Winter, Andreas},
doi = {10.1007/s00220-016-2609-8},
file = {::},
issn = {0010-3616},
journal = {Commun. Math. Phys.},
month = {oct},
number = {1},
pages = {291--313},
publisher = {Springer Berlin Heidelberg},
title = {{Tight Uniform Continuity Bounds for Quantum Entropies: Conditional Entropy, Relative Entropy Distance and Energy Constraints}},
url = {http://link.springer.com/10.1007/s00220-016-2609-8},
volume = {347},
year = {2016}
}
@article{Pashkin2003a,
abstract = {Quantum oscillations in two coupled charge qubits},
author = {Pashkin, Yu. A. and Yamamoto, T. and Astafiev, O. and Nakamura, Y. and Averin, D. V. and Tsai, J. S.},
doi = {10.1038/nature01365},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pashkin et al. - 2003 - Quantum oscillations in two coupled charge qubits(2).pdf:pdf},
issn = {0028-0836},
journal = {Nature},
month = {feb},
number = {6925},
pages = {823--826},
publisher = {Nature Publishing Group},
title = {{Quantum oscillations in two coupled charge qubits}},
url = {http://www.nature.com/doifinder/10.1038/nature01365 http://www.nature.com/articles/nature01365},
volume = {421},
year = {2003}
}
@inproceedings{Xie2012,
author = {Xie, Jingming},
booktitle = {2012 7th Int. Conf. Comput. Sci. Educ.},
doi = {10.1109/ICCSE.2012.6295169},
isbn = {978-1-4673-0242-5},
month = {jul},
pages = {695--699},
publisher = {IEEE},
title = {{Research on key technologies base Unity3D game engine}},
url = {http://ieeexplore.ieee.org/document/6295169/},
year = {2012}
}
@article{Macchiavello2002,
author = {Macchiavello, Chiara and Palma, G. Massimo},
doi = {10.1103/PhysRevA.65.050301},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Macchiavello, Palma - 2002 - Entanglement-enhanced information transmission over a quantum channel with correlated noise.pdf:pdf},
issn = {1050-2947},
journal = {Phys. Rev. A},
month = {apr},
number = {5},
pages = {050301},
publisher = {American Physical Society},
title = {{Entanglement-enhanced information transmission over a quantum channel with correlated noise}},
url = {http://link.aps.org/doi/10.1103/PhysRevA.65.050301},
volume = {65},
year = {2002}
}
@article{Pati1993,
author = {Pati, A. K and Joshi, A},
doi = {10.1209/0295-5075/21/7/002},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Pati, Joshi - 1993 - A Geometric Meaning to the Probabilities of Two-State Quantum Systems.pdf:pdf},
issn = {0295-5075},
journal = {Europhys. Lett.},
month = {mar},
number = {7},
pages = {723--728},
publisher = {IOP Publishing},
title = {{A Geometric Meaning to the Probabilities of Two-State Quantum Systems}},
url = {http://stacks.iop.org/0295-5075/21/i=7/a=002?key=crossref.67aefb0f0055df8cfe4053aab4181aa7},
volume = {21},
year = {1993}
}
@article{Brunner2014,
author = {Brunner, Nicolas and Huber, Marcus and Linden, Noah and Popescu, Sandu and Silva, Ralph and Skrzypczyk, Paul},
doi = {10.1103/PhysRevE.89.032115},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Brunner et al. - 2014 - Entanglement enhances cooling in microscopic quantum refrigerators.pdf:pdf},
issn = {1539-3755},
journal = {Phys. Rev. E},
month = {mar},
number = {3},
pages = {032115},
publisher = {American Physical Society},
title = {{Entanglement enhances cooling in microscopic quantum refrigerators}},
url = {http://link.aps.org/doi/10.1103/PhysRevE.89.032115},
volume = {89},
year = {2014}
}
@article{Andai2007,
abstract = {In this paper we prove a nontrivial lower bound for the determinant of the covariance matrix of quantum mechanical observables, which was conjectured by Gibilisco, Isola and Imparato. The lower bound is given in terms of the commutator of the state and the observables and their scalar product, which is generated by an arbitrary symmetric operator monotone function.},
archivePrefix = {arXiv},
arxivId = {0707.1147},
author = {Andai, Attila},
doi = {10.1063/1.2830429},
eprint = {0707.1147},
file = {:Users/fcam0004/Library/Application Support/Mendeley Desktop/Downloaded/Andai - 2007 - Uncertainty principle with quantum Fisher information.pdf:pdf},
month = {jul},
title = {{Uncertainty principle with quantum Fisher information}},
url = {http://arxiv.org/abs/0707.1147 http://dx.doi.org/10.1063/1.2830429},
year = {2007}
}


==> overlay.tex <==
% --- Overlay with Tikz
\tikz[remember picture,overlay] \node[opacity=1,inner sep=0pt] at (current page.center){\includegraphics[width=\paperwidth,height=\paperheight]{back.png}};
\begin{tikzpicture}[remember picture, overlay]
    \node[inner sep=0pt] at (current page.center) {%
        \includegraphics[width=\paperwidth,height=\paperheight]{yourpic.png}%
    };%
\end{tikzpicture}
